Mix-and-Conquer: Beamforming Design with Interconnected RIS for Multi-User Networks

We propose a new reconfigurable intelligent surface (RIS) structure, referred to as interconnected RIS (I-RIS), which allows the RIS elements to be interconnected and share the incident signals using simple binary radio frequency (RF) switches and mix them into the reflecting signals. This structure enables multi-user scaling and requires fewer elements (i.e., a compact structure) compared to standard RIS (S-RIS), which assumes no interconnection between the elements. The I-RIS compact design makes it practical for deployment on space-limited nodes, e.g., unmanned aerial vehicles (UAVs). Hence, in this work, we propose a beamforming design based on I-RIS in a multi-user network, where we use binary RF switches as RIS elements. We show that our switch-based I-RIS offers a higher gain compared to an S-RIS using phase shifters. Finally, we introduce two optimization methods, sigmoid filled function (SFF) and semi-definite binary optimization (SBO), to optimize the RIS elements and evaluate their performance in terms of sum-rate and complexity.

==> Sections/Abstract.tex <==
We propose a new reconfigurable intelligent surface (RIS) structure, referred to as interconnected RIS (I-RIS), which allows the RIS elements to be interconnected and share the incident signals using simple binary radio frequency (RF) switches and mix them into the reflecting signals. This structure enables multi-user scaling and requires fewer elements (i.e., a compact structure) compared to standard RIS (S-RIS), which assumes no interconnection between the elements. The I-RIS compact design makes it practical for deployment on space-limited nodes, e.g., unmanned aerial vehicles (UAVs). Hence, in this work, we propose a beamforming design based on I-RIS in a multi-user network, where we use binary RF switches as RIS elements. We show that our switch-based I-RIS offers a higher gain compared to an S-RIS using phase shifters. Finally, we introduce two optimization methods, sigmoid filled function (SFF) and semi-definite binary optimization (SBO), to optimize the RIS elements and evaluate their performance in terms of sum-rate and complexity.

==> Sections/Abstract_USV_v0.tex <==
This paper focuses on beamforming with reconfigurable intelligent surfaces (RISs) installed on an unmanned surface vessel (USV) to assist maritime communications. To address the limited space issue on USVs, we propose a compact RIS architecture, referred to as generalized RIS. This architecture allows the RIS elements to share their received signals with each other, unlike previous studies that assumed the RIS elements do not connect to each other (referred to as standard RIS). Moreover, we use binary switches as RIS elements due to practical issues with phase shifters (PSs), such as the problems in controlling the amplitude and phase of a PS simultaneously and the difficulties of using PSs at high frequencies. Our simulation results show that the generalized RIS outperforms the standard RIS and thus requires fewer elements (i.e., compact RIS) to achieve a desired performance. Finally, we introduce two optimization methods, sigmoid filled function (SFF) and semi-definite binary optimization (SBO), to obtain the optimal RIS configuration. The findings reveal that the SFF method offers a higher gain than the SBO method.  


==> Sections/Abstract_USV_v1.tex <==
{\color{blue}We propose a compact structure for reconfigurable intelligent surface (RIS), referred to as generalized RIS, which allows the RIS elements to be interconnected to share the incident signals using simple binary radio frequency (RF) switches and mix them into the reflecting signals. This structure enables multi-user scaling and spectrum-efficient communications. In this paper, we focus on maritime networks and evaluate the performance of the generalized RIS by comparing it to the standard RIS, which assumes that the RIS elements do not connect to each other. Our results show that the generalized RIS requires fewer elements than the standard RIS to achieve the desired performance, and therefore is suitable to install on resource-limited nodes, e.g., unmanned surface vessels (USVs), to assist maritime networks. Moreover, we use binary RF switches} as RIS elements due to practical issues with phase shifters (PSs), such as the problems in controlling the amplitude and phase of a PS simultaneously and the difficulties of using PSs at high frequencies. Finally, we introduce two optimization methods, sigmoid filled function (SFF) and semi-definite binary optimization (SBO), to obtain the optimal RIS configuration. The findings reveal that the SFF method offers a higher gain than the SBO method.  


==> Sections/Sect1_Introduction.tex <==
With the ever-increasing demand for wireless networks, the next generation of wireless networks must improve key performance metrics such as coverage, data rate, and spectrum/energy efficiency compared to the existing networks. Reconfigurable intelligent surface (RIS) has recently emerged as a promising technique, offering a range of advantages, including the capability to bypass obstacles to improve coverage and enhance data rate and spectral efficiency, all achieved in a cost-effective and power-efficient manner~\cite{zhang2020capacity,yu2019miso,bjornson2020reconfigurable}. RIS, an artificial surface comprising electromagnetic material, contains a substantial number of reflecting elements that are low-cost and (nearly-)passive, capable of independently adjusting the phase and/or amplitude of incident signals. By intelligently configuring the RIS elements, it becomes possible to combine reflected signals constructively at the intended receiver and destructively at undesired receivers.  



Due to the high path loss in the transmitter-RIS-receiver link and the passive nature of RIS, the existing RISs require many elements to assist the network. In this work, we refer to the existing RIS structure as standard RIS (S-RIS), where each RIS element acts individually, and there is no interconnection between RIS elements. However, having a large-size RIS is not always feasible, especially in space-limited nodes, e.g., unmanned aerial vehicles (UAVs), where space plays a crucial role and affects the weight, power consumption, and cost of the vehicle. By minimizing the size of components and using space efficiently, UAVs can carry more payload/fuel, be more agile and responsive, and have longer flight times~\cite{ramasamy2014avionics,azarov2019composite}.  


As discussed above, small-size (i.e., compact) RIS is more desired in space-limited nodes. Thus, in this paper, we propose a new RIS structure, referred to as interconnected RIS (I-RIS), where RIS elements have interconnection with each other. In I-RIS, we divide the elements into different cells and define the elements in each cell as {\it neighbors}. Moreover, each I-RIS element involves: (i) sharing its incident signal with its neighbors and (ii) reflecting a combination of the incident signals from its neighbors toward the receivers. We show that I-RIS improves user-scaling and requires fewer elements compared to S-RIS. %For example, our findings demonstrate that I-RIS, with $64$ elements, provides a $68 \%$ higher sum-rate than S-RIS with the same number of elements. Further, I-RIS needs $16$ elements to achieve a sum-rate of $6$, while S-RIS requires $64$ elements to get the same performance. The smaller size of I-RIS is feasible due to what we call the degrees-of-control (DoC), which captures the number of tunable parameters in RIS and determines the gain from incorporating an RIS into the system. Thanks to the interconnected design, to attain the same DoC, I-RIS requires fewer elements compared to prior designs.
For example, our findings demonstrate that in a single-input single-output (SISO) network serving four users, an I-RIS with $64$ elements and $16$ cells provides a $68 \%$ higher sum-rate than an S-RIS with the same number of elements. Additionally, I-RIS requires four times fewer elements to match the same sum-rate achieved by S-RIS. The smaller size of I-RIS is feasible due to what we call the degrees-of-control (DoC), which captures the number of tunable parameters in RIS and intuitively determines the gain from incorporating an RIS into the system. Thanks to the interconnected design, I-RIS requires fewer elements to attain the same DoC than prior designs.




% Additionally, we show that with the same DoC, the complexity of finding the optimal solution with I-RIS and S-RIS is almost identical. 

%In particular, each receiver estimates its incoming channels from all transmitters using the pilot signals and then informs the others, while the estimated CSI is different from the actual CSI due to different reasons such as noise, hardware impairments, and unfavorable environments. 


Beyond the issue of interconnected elements, previous works usually used phase shifters (PSs) as RIS elements. However, simultaneously controlling the amplitude and phase of PSs is challenging, and PSs are lossy at high frequencies. Motivated by these,~\cite{mendez2016hybrid,nassirpour2022power} proposed beamforming techniques using radio frequency (RF) switches to enhance performance. Consequently, we consider RF switches as RIS elements in this work and show that our switch-based I-RIS outperforms an S-RIS using low-bit PSs.
On the other hand, the use of RF switches introduces a non-convex optimization problem. To address this problem, we propose two optimization methods: the sigmoid filled function (SFF) method and the semi-definite binary optimization (SBO) method, where the former is a heuristic approach, and the latter utilizes the successive convex approximation (SCA) method. We compare the performance of these two optimization methods with the successive-refinement (SR) method~\cite{wu2019beamforming} in terms of sum-rate and complexity. Our findings reveal: (i) the SFF method provides a higher sum-rate than the others; (ii) the complexity of the SFF method is lower than the SBO method and higher than the SR method.


The rest of this paper is organized as follows:
Section~\ref{Section:Problem} demonstrates problem setting and RIS structure. Section~\ref{Section:Beam_design} presents our beamforming
design, Section~\ref{Section:Num_results} includes numerical analysis, and Section~\ref{Section:conclusion} concludes the paper.

\textbf{Notations:} We utilize italic, bold-face lowercase, and bold-face uppercase letters to represent scalars, vectors, and matrices, respectively. We use $\mathbb{C}^{a\times b}$ to denote the space of an $a\times b$ dimensional complex-valued matrix. In this work, $\mathrm{diag}\{\textbf{a}\}$ shows a diagonal matrix using $\textbf{a}$, $\textbf{Y} \succeq \mathbf{0}$ denotes $\textbf{Y}$ is a positive semi-definite matrix, $\mathrm{blkdiag}\{\mathbf{A}, \mathbf{B}\}$ represents a block diagonal matrix with $\mathbf{A}$ and $\mathbf{B}$ on its main diagonal, and $\mathrm{Diag}(\textbf{A})$ is a vector of diagonal elements in $\textbf{A}$. Here, $|a|$ is the modulus of $a$, and $||\textbf{a}||$ denotes Euclidean norm of $\textbf{a}$. Further, we use $\log(.)$, $\lfloor . \rfloor$,  $\mathrm{tr}\left(.\right)$, $\textbf{B}^{\top}$, and $\textbf{B}^H$ to indicate the logarithmic function in base 2, the floor function, the trace function, the transpose of $\textbf{B}$, and the conjugate transpose of $\textbf{B}$, respectively. We also denote sets using calligraphic font style, and for a set $\mathcal{M}$, $|\mathcal{M}|$ is its cardinality.
\vspace{-0.3mm}

==> Sections/Sect1_Introduction_USV.tex <==
The demands for reliable and efficient maritime communications have increased significantly due to their vital role in various areas, such as near-shore activities and military operations. Traditionally, maritime networks utilize very-high-frequency (VHF) and satellite communications; however, VHF suffers from low data rates due to its limited bandwidth, and satellite communication is expensive and poses significant delays. To tackle these issues and extend coverage, the literature investigates multi-hop networks assisted by unmanned surface vessels (USVs)~\cite{wang2022unmanned}. \avc{the following sentence is weak and also shares too much information. 1) Why does SISO matter at this point? 2) beamforming for what?} Hence, in this paper, we focus on a single-input single-output (SISO) USV-assisted maritime network with distributed transmitter-receiver pairs and propose a beamforming design to assist the network. 

Most USV-assisted studies assume a USV that acts as a relay to improve the network performance~\cite{zeng2022mimo}. To fully utilize the benefits of a relay, it should operate in full-duplex mode, which increases the signal processing complexity and power consumption, while USVs are resource-limited nodes~\cite{lu2015stochastic}. On the other hand, recently, the research community has shown significant interest in reconfigurable intelligent surfaces (RISs) to enhance coverage and 
spectral efficiency in a power-efficient manner~\cite{choi2021joint,jiang2022intelligent}. An RIS comprises 
small and passive elements, each capable of reflecting the incident signals. By smartly configuring the RIS elements, one could combine the reflected signals constructively at the desired receiver and destructively at undesired receivers. 
\avc{1) this basically repeat what came at the end of the previous paragraph, 2) at this point it seems you are not doing anything new, RIS and USV assisted network, that's it.}
As a result, in this work, we consider a SISO USV-assisted maritime network in which the USV is equipped with an RIS to assist the network. We propose a beamforming design for the RIS to highlight the gain coming purely from passive RIS.

As RIS elements are passive, \avc{do not use ``we'', you can say the existing designs} we require a large-size RIS to compensate for product-path loss through the transmitter-RIS-receiver link~\cite{wu2019beamforming}. However, installing a large-size RIS on USV is not always feasible due to space limitations. The past studies typically assumed no interconnection between RIS elements where each element acts individually. We refer to this as standard RIS (S-RIS). Here, the interesting question is what would happen if the RIS elements were interconnected and could share their incident signals with each other? To answer this question, we propose a new RIS structure, interconnected RIS (\newwRIS), where the RIS elements are interconnected and share the incident signals. We show that \newRIS enhances multi-user scaling and requires fewer elements than S-RIS to achieve a given performance, thus enabling a compact RIS structure.


The smaller size of \newRIS is feasible due to what we refer to as the degrees-of-control (DoC), which captures the number of tunable parameters in the RIS design and determines the gain from incorporating an RIS into the system. Thanks to the interconnected design, to attain the same DoC, \newRIS requires fewer elements compared to prior designs.


Beyond the issue of interconnected elements, in RIS-aided networks, past works usually used phase shifters (PSs) as RIS elements, but it is hard to control the amplitude and phase of PSs simultaneously, and PSs do not operate at high frequencies. Motivated by these,~\cite{mendez2016hybrid,nassirpour2022power,johnny2021low} propose switch-based beamforming techniques to improve the network performance. Thus, we assume a switch-based RIS in this study where transmitters have imperfect channel state information (CSI). 
In particular, each receiver estimates its incoming channels from all transmitters using the pilot signals and then informs the others, while the estimated CSI is different from the actual CSI due to different reasons such as noise, hardware impairments, and unfavorable environments. Using binary switches leads to a non-convex optimization problem. To optimize this problem, we propose two optimization methods: the sigmoid filled function (SFF) method and the semi-definite binary
optimization (SBO) method, where the former is a heuristic method, and the latter operates based on the successive convex approximation (SCA) method. We compare the performance of these two optimization methods in terms of complexity and sum-rate, and our results show that the SFF method outperforms the SBO method. 

 


The rest of this paper is organized as follows:
Section~\ref{Section:Problem} demonstrates the problem setting and two RIS structures. Section~\ref{Section:Beam_design} presents the beamforming
design to maximize sum-rate, Section~\ref{Section:Num_results} includes the numerical analysis, and Section~\ref{Section:conclusion} concludes the paper.


\textbf{Notations:} We utilize italic, bold-face lowercase, and bold-face uppercase letters to represent scalars, vectors, and matrices, respectively. We use $\mathbb{C}^{a\times b}$ to denote the space of an $a\times b$ dimensional complex-valued matrix. In this work, $\mathrm{diag}\{\textbf{a}\}$ shows a diagonal matrix using vector $\textbf{a}$, $\mathrm{blkdiag}\{\mathbf{A}, \mathbf{B}\}$ represents a block diagonal matrix with $\mathbf{A}$ and $\mathbf{B}$ on its main diagonal, and $\mathrm{Diag}(\textbf{A})$ is a vector of diagonal elements in $\textbf{A}$. $|a|$ is the modulus of $a$, and $||\textbf{a}||$ denote Euclidean norm of $\textbf{a}$. Further, we use $\log(.)$, $\lfloor . \rfloor$,  $\mathrm{tr}\left(.\right)$, $\textbf{B}^{\top}$, and $\textbf{B}^H$ to indicate the logarithmic function in base 2, the floor function, the trace function, the transpose of $\textbf{B}$, and the conjugate transpose of $\textbf{B}$, respectively. We also denote sets using calligraphic font style, and for a set $\mathcal{M}$, $|\mathcal{M}|$ describes its cardinality.


==> Sections/Sect1_Introduction_USV_v0.tex <==
The blue economy's rapid expansion has brought great demands for reliable and efficient maritime wireless communications. Traditionally, maritime networks utilize very-high-frequency (VHF) and satellite communications; however, VHF suffers from low data rates due to its limited bandwidth, and satellite communication is expensive and poses significant delays and overhead. To tackle these issues, relay-aided maritime networks have been proposed in past works~\cite{zeng2022mimo,ai2021joint,wang2022unmanned}, where unmanned surface vessels (USVs), which have extensive military applications, e.g., intercepting enemies and detecting intelligence, act as relays to enhance communication performance. To fully utilize the benefits of a relay, it should operate in full-duplex mode, which generates loop-back self-interference at the relay and thus increases the signal processing complexity and power consumption, while USVs are limited-resource nodes~\cite{lu2015stochastic}. 

Recently, the research community has shown significant interest in reconfigurable intelligent surfaces (RISs) due to their potential to enhance spectral efficiency in a power-efficient manner~\cite{choi2021joint,jiang2022intelligent}. An RIS comprises a large number of small, passive, and cost-effective elements, each capable of reflecting an incident signal independently. By smartly configuring the RIS elements, the reflected signals can be combined constructively at the desired receiver and destructively at undesired receivers. As RIS elements reflect the incident signals without utilizing radio frequency (RF) chains, they could potentially offer a low-complexity and power-efficient solution to improve the performance of maritime networks.

As a result, in this paper, we use USV acting as RIS to assist a maritime network with distributed transmitters and receivers. Specifically, we focus on a single-input single-output (SISO) RIS-assisted maritime network and study pure RIS gain coming from passive beamforming at RIS. Due to the passive nature of RIS elements, a large-size RIS is necessary to compensate for product-path loss through the transmitter-RIS-receiver link~\cite{wu2019beamforming}. However, due to limited space, installing a large-size RIS on a USV may not be practical. The literature on RIS-assisted networks typically assumed no connection between RIS elements, and each element acts individually. We refer to this as standard RIS. Here, the interesting question is, what would happen if the RIS elements were inter-connected? To answer this, we propose a new RIS architecture, referred to as generalized RIS, where the RIS elements are inter-connected, and each element can share its received signal with other RIS elements. We show that the generalized RIS requires a fewer number of elements (i.e., smaller size) than the standard RIS to achieve a specific sum-rate, enabling a compact RIS architecture suitable for USVs.

Moreover, past works usually use phase shifters (PSs) as RIS elements, but PSs deal with two practical challenges. First, it is hard to control the amplitude and phase of PSs simultaneously; second, it is impossible to operate PSs at high frequencies. Motivated by these,~\cite{mendez2016hybrid,nassirpour2022power} propose switch-based beamforming techniques to improve the network performance. Therefore, in this work, we assume a switch-based RIS, where each RIS element can either reflect or block its incident signal. Notice that a beamforming design with switch-based RIS leads to a non-convex optimization problem. To optimize this problem, we propose two optimization methods as the sigmoid filled function (SFF) method and the semi-definite binary
optimization (SBO) method, where the former is a heuristic method, and the latter operates based on successive convex approximation (SCA) method. We compare the performance of these two optimization methods in terms of complexity and sum-rate, and our findings reveal that the SFF method outperforms the SBO method.

%Furthermore, to include a real-world maritime network, in this manuscript, we assume that imperfect channel state information (CSI) is available globally. In particular, each receiver estimates its incoming channels from all transmitters using the pilot signals and then informs the other nodes, while the estimated CSI is different from the actual CSI due to hardware impairments. 


The rest of this paper is organized as follows:
Section~\ref{Section:Problem} demonstrates the problem setting and two RIS architectures. Section~\ref{Section:Beam_design} presents the beamforming
design to maximize sum-rate, Section~\ref{Section:Num_results} includes the numerical analysis, and Section~\ref{Section:conclusion} concludes the paper.


\textbf{Notations:} In this paper, we utilize bold-face lowercase, bold-face uppercase, and italic letters to represent vectors, matrices, and scalars, respectively. We use the notation $\mathbb{C}^{I\times J}$ to denote the space of complex-valued matrices with dimensions $I\times J$. The diagonal matrix that utilizes vector $\textbf{x}$ is denoted by $\mathrm{diag}\{\textbf{x}\}$, while $\mathrm{blkdiag}\{\mathbf{X}, \mathbf{Y}\}$ represents a block diagonal matrix with matrices $\mathbf{X}$ and $\mathbf{Y}$ on its main diagonal, and $\mathrm{Diag}(\textbf{X})$ shows a vector of diagonal elements in $\textbf{X}$. In this study, $|\textbf{x}|$ and $||\textbf{x}||$ show the absolute value and Euclidean norm of a complex-valued vector $\textbf{x}$, respectively. Additionally, we use $\log(.)$, $\lfloor . \rfloor$,  $\mathrm{tr}\left(.\right)$, $\textbf{B}^{\top}$, and $\textbf{B}^H$ to indicate the logarithmic function in base 2, the floor function, the trace function, the transpose of $\textbf{B}$, and the conjugate transpose of $\textbf{B}$, respectively. We also denote sets using calligraphic font styles, and for a set $\mathcal{M}$, $|\mathcal{M}|$ describes its cardinality.


==> Sections/Sect1_Introduction_USV_v1.tex <==
{\color{blue}Recently, the research community has shown significant interest in reconfigurable intelligent surfaces (RISs) due to their potential to enhance spectral efficiency in a power-efficient manner~\cite{choi2021joint,jiang2022intelligent}. An RIS comprises a large number of small, passive, and cost-effective elements, each capable of reflecting an incident signal independently. By smartly configuring the RIS elements, the reflected signals can be combined constructively at the desired receiver and destructively at undesired receivers. Due to the passive nature of RIS elements, a large-size RIS is necessary to compensate for product-path loss through the transmitter-RIS-receiver link~\cite{wu2019beamforming}. However, installing a large-size RIS is not always feasible, especially on limited-space nodes, such as unmanned surface vessels (USVs) and unmanned aerial vehicles (UAVs). The past studies typically assumed no interconnection between RIS elements where each element acts individually. We refer to this as standard RIS (S-RIS). Here, the interesting question is, what would happen if the RIS elements were interconnected? To answer this, we propose a new RIS structure, referred to as generalized RIS (G-RIS), where the RIS elements are interconnected, and each element shares the incident signal with other elements. We show that the G-RIS not only enhances the multi-user scaling but also requires fewer elements than the S-RIS to achieve a given performance, enabling a compact RIS structure.


On the other hand, the blue economy's rapid expansion has brought great demands for reliable and efficient maritime wireless communications. Traditionally, maritime networks utilize very-high-frequency (VHF) and satellite communications; however, VHF suffers from low data rates due to its limited bandwidth, and satellite communication is expensive and poses significant delays and overhead. To tackle these issues, the literature proposes relay-aided maritime networks~\cite{zeng2022mimo,ai2021joint,wang2022unmanned}, where USVs, which have extensive military applications, e.g., intercepting enemies and detecting intelligence, act as relays to enhance communication performance. To fully utilize the benefits of a relay, it should operate in full-duplex mode, which generates loop-back self-interference at the relay and thus increases the signal processing complexity and power consumption, while USVs are resource-limited nodes~\cite{lu2015stochastic}. As a result, in this paper, we focus on a USV-assisted maritime network with distributed transmitters and receivers where the USV is equipped with a G-RIS to assist the network. We study a single-input single-output (SISO) network to highlight pure RIS gain coming from passive beamforming at RIS. 

Furthermore, to include a real-world maritime network, in this manuscript, we assume that imperfect channel state information (CSI) is available globally. In particular, each receiver estimates its incoming channels from all transmitters using the pilot signals and then informs the other nodes, while the estimated CSI is different from the actual CSI due to hardware impairments.}

Moreover, past works usually used phase shifters (PSs) as RIS elements, but PSs deal with two practical challenges. First, it is hard to control the amplitude and phase of PSs simultaneously; second, it is impossible to operate PSs at high frequencies. Motivated by these,~\cite{mendez2016hybrid,nassirpour2022power} propose switch-based beamforming techniques to improve the network performance. Therefore, in this work, we assume a switch-based RIS, where each RIS element can either reflect or block its incident signal. Notice that a beamforming design with switch-based RIS leads to a non-convex optimization problem. To optimize this problem, we propose two optimization methods as the sigmoid filled function (SFF) method and the semi-definite binary
optimization (SBO) method, where the former is a heuristic method, and the latter operates based on successive convex approximation (SCA) method. We compare the performance of these two optimization methods in terms of complexity and sum-rate, and our findings reveal that the SFF method outperforms the SBO method.

 


The rest of this paper is organized as follows:
Section~\ref{Section:Problem} demonstrates the problem setting and two RIS structures. Section~\ref{Section:Beam_design} presents the beamforming
design to maximize sum-rate, Section~\ref{Section:Num_results} includes the numerical analysis, and Section~\ref{Section:conclusion} concludes the paper.


\textbf{Notations:} In this paper, we utilize bold-face lowercase, bold-face uppercase, and italic letters to represent vectors, matrices, and scalars, respectively. We use the notation $\mathbb{C}^{I\times J}$ to denote the space of complex-valued matrices with dimensions $I\times J$. The diagonal matrix that utilizes vector $\textbf{x}$ is denoted by $\mathrm{diag}\{\textbf{x}\}$, while $\mathrm{blkdiag}\{\mathbf{X}, \mathbf{Y}\}$ represents a block diagonal matrix with matrices $\mathbf{X}$ and $\mathbf{Y}$ on its main diagonal, and $\mathrm{Diag}(\textbf{X})$ shows a vector of diagonal elements in $\textbf{X}$. In this study, $|\textbf{x}|$ and $||\textbf{x}||$ show the absolute value and Euclidean norm of a complex-valued vector $\textbf{x}$, respectively. Additionally, we use $\log(.)$, $\lfloor . \rfloor$,  $\mathrm{tr}\left(.\right)$, $\textbf{B}^{\top}$, and $\textbf{B}^H$ to indicate the logarithmic function in base 2, the floor function, the trace function, the transpose of $\textbf{B}$, and the conjugate transpose of $\textbf{B}$, respectively. We also denote sets using calligraphic font styles, and for a set $\mathcal{M}$, $|\mathcal{M}|$ describes its cardinality.


==> Sections/Sect1_Introduction_USV_v2.tex <==
Recently, the research community has shown significant interest in reconfigurable intelligent surfaces (RISs) to enhance coverage and %\avc{coverage and}
spectral efficiency in a power-efficient manner~\cite{choi2021joint,jiang2022intelligent}. An RIS comprises %a \avc{do you need to say large?} large number of 
small and passive elements, each capable of reflecting the incident signals. By smartly configuring the RIS elements, one could %\sout{we} \avc{one could}
combine the reflected signals constructively at the desired receiver and destructively at undesired receivers. As RIS elements are passive, we require a large-size RIS to compensate for product-path loss through the transmitter-RIS-receiver link~\cite{wu2019beamforming}. However, having a large-size RIS is not always feasible, especially in space-limited nodes, e.g., unmanned aerial vehicles (UAVs), where space plays a crucial role and affects the weight, power consumption, and cost of the vehicle. By minimizing the size of components and using space efficiently, UAVs can carry more payload/fuel, be more agile and responsive, and have longer flight times~\cite{ramasamy2014avionics,azarov2019composite}.
%\avc{my text is just a suggestion, you need to find reference(s) and say what these purposes could be.}
% \avc{where the available space is of great value and can be used for various other critical purposes}. \avc{new paragraph} 

The past studies typically assumed no interconnection between RIS elements where each element acts individually. We refer to this as standard RIS (S-RIS). Here, the interesting question is %\sout{,} \avc{no ``,'' needed} 
what would happen if the RIS elements were interconnected and could share their incident signals with each other?
% \avc{and could share their incident signals with each other}?
To answer this question, we propose a new RIS structure, interconnected RIS (\newwRIS), where the RIS elements are interconnected and share the incident signals. We show that \newRIS enhances multi-user scaling and requires fewer elements than S-RIS to achieve a given performance, thus enabling a compact RIS structure. The smaller size of \newRIS is feasible due to what we refer to as the degrees-of-control (DoC), which captures the number of tunable parameters in the RIS design and determines the gain from incorporating an RIS into the system. Thanks to the interconnected design, to attain the same DoC, \newRIS requires fewer elements compared to prior designs.


%\avc{I am having trouble understanding the point of the following paragraph in the introduction. At least the discussion on VHf etc.}
On the other hand, the blue economy's rapid expansion has brought great demands for reliable and efficient maritime communications. Traditionally, maritime networks utilize satellite communications; however, it is expensive and poses significant delays. To tackle this issue, the literature proposes relay-aided maritime networks~\cite{zeng2022mimo,wang2022unmanned}, where USVs act as relays to enhance communication performance. In addition, to fully utilize the benefits of a relay, it should operate in full-duplex mode, which increases the signal processing complexity and power consumption, while USVs are resource-limited nodes~\cite{lu2015stochastic}. 



As a result, in this paper, we focus on a maritime network with distributed transmitter-receiver pairs where there exists a USV equipped with an \newRIS to assist the network. We study a single-input single-output (SISO) network to highlight the gain coming purely from passive \newwRIS. Furthermore, to include a real-world scenario, we assume that transmitters have imperfect channel state information (CSI). 
%\sout{is available globally}. 
In particular, each receiver estimates its incoming channels from all transmitters using the pilot signals and then informs the others, while the estimated CSI is different from the actual CSI due to different reasons such as noise, hardware impairments, and unfavorable environments. % \avc{due to different reasons such as noise, hardware impairments, and unfavorable environments}.
%\avc{Beyond the issue of interconnected elements,}
%\avc{the text is weak, in this past paragraph, you do not say anything about your achievements or let alone exciting. You say what you consider, but what do you achieve? We need to discuss this in person.}

Beyond the issue of interconnected elements, in RIS-aided networks, past works usually used phase shifters (PSs) as RIS elements, but it is hard to control the amplitude and phase of PSs simultaneously, and PSs do not operate at high frequencies. Motivated by these,~\cite{mendez2016hybrid,nassirpour2022power,johnny2021low} %\avc{add my binary paper with Johnny here}
propose switch-based beamforming techniques to improve the network performance. Thus, we assume a switch-based RIS in this study, which leads to a non-convex optimization problem. %\avc{the next sentence negates the sharing part you have talked about so far!} %where each RIS element can either reflect or block its incident signal. A beamforming design with switch-based RIS leads to a non-convex optimization problem.
To optimize this problem, we propose two optimization methods: the sigmoid filled function (SFF) method and the semi-definite binary
optimization (SBO) method, where the former is a heuristic method, and the latter operates based on the successive convex approximation (SCA) method. We compare the performance of these two optimization methods in terms of complexity and sum-rate, and our results show that the SFF method outperforms the SBO method.

 


The rest of this paper is organized as follows:
Section~\ref{Section:Problem} demonstrates the problem setting and two RIS structures. Section~\ref{Section:Beam_design} presents the beamforming
design to maximize sum-rate, Section~\ref{Section:Num_results} includes the numerical analysis, and Section~\ref{Section:conclusion} concludes the paper.


\textbf{Notations:} We utilize italic, bold-face lowercase, and bold-face uppercase letters to represent scalars, vectors, and matrices, respectively. We use $\mathbb{C}^{a\times b}$ to denote the space of an $a\times b$ dimensional complex-valued matrix. In this work, $\mathrm{diag}\{\textbf{a}\}$ shows a diagonal matrix using vector $\textbf{a}$, $\mathrm{blkdiag}\{\mathbf{A}, \mathbf{B}\}$ represents a block diagonal matrix with $\mathbf{A}$ and $\mathbf{B}$ on its main diagonal, and $\mathrm{Diag}(\textbf{A})$ is a vector of diagonal elements in $\textbf{A}$. $|a|$ is the modulus of $a$, and $||\textbf{a}||$ denote Euclidean norm of $\textbf{a}$. Further, we use $\log(.)$, $\lfloor . \rfloor$,  $\mathrm{tr}\left(.\right)$, $\textbf{B}^{\top}$, and $\textbf{B}^H$ to indicate the logarithmic function in base 2, the floor function, the trace function, the transpose of $\textbf{B}$, and the conjugate transpose of $\textbf{B}$, respectively. We also denote sets using calligraphic font style, and for a set $\mathcal{M}$, $|\mathcal{M}|$ describes its cardinality.


==> Sections/Sect1_Introduction_v1.tex <==
With the ever-increasing demand for wireless networks, the next generation of wireless networks must improve key performance metrics such as coverage, data rate, and spectrum/energy efficiency compared to the existing networks. Reconfigurable intelligent surface (RIS) has recently emerged as a promising technique, offering a range of advantages, including the capability to bypass obstacles to improve coverage and enhance data rate and spectral efficiency, all achieved in a cost-effective and power-efficient manner~\cite{zhang2020capacity,yu2019miso,bjornson2020reconfigurable}. RIS, an artificial surface comprising electromagnetic material, contains a substantial number of reflecting elements that are low-cost and (nearly-)passive, capable of independently adjusting the phase and/or amplitude of incident signals. By intelligently configuring the RIS elements, it becomes possible to combine reflected signals constructively at the intended receiver and destructively at undesired receivers.  



Due to the high path loss in the transmitter-RIS-receiver link and the passive nature of RIS, existing RISs require many elements to assist the network. In this work, we refer to the existing RIS structure as standard RIS (S-RIS), where each RIS element acts individually, and there is no interconnection between RIS elements. However, having a large-size RIS is not always feasible, especially in space-limited nodes, e.g., unmanned aerial vehicles (UAVs), where space plays a crucial role and affects the weight, power consumption, and cost of the vehicle. By minimizing the size of components and using space efficiently, UAVs can carry more payload/fuel, be more agile and responsive, and have longer flight times~\cite{ramasamy2014avionics,azarov2019composite}.  


As discussed above, small-size (i.e., compact) RIS is more desired in space-limited nodes. Thus, in this paper, we propose a new RIS structure, referred to as interconnected RIS (I-RIS), where RIS elements have interconnection with each other. In I-RIS, we divide the elements into different cells and define the elements in each cell as {\it neighbors}. Moreover, each I-RIS element involves: (i) sharing its incident signal with its neighbors and (ii) reflecting a combination of the incident signals from its neighbors toward the receivers. We show that I-RIS improves user-scaling and requires fewer elements compared to S-RIS. %For example, our findings demonstrate that I-RIS, with $64$ elements, provides a $68 \%$ higher sum-rate than S-RIS with the same number of elements. Further, I-RIS needs $16$ elements to achieve a sum-rate of $6$, while S-RIS requires $64$ elements to get the same performance. The smaller size of I-RIS is feasible due to what we call the degrees-of-control (DoC), which captures the number of tunable parameters in RIS and determines the gain from incorporating an RIS into the system. Thanks to the interconnected design, to attain the same DoC, I-RIS requires fewer elements compared to prior designs.
For example, our findings demonstrate that in a single-input single-output (SISO) network serving four users, an I-RIS with $64$ elements and $16$ cells provides an $81 \%$ higher sum-rate than an S-RIS with the same number of elements. Additionally, I-RIS requires four times fewer elements to match the same sum-rate achieved by S-RIS. The smaller size of I-RIS is feasible due to what we call the degrees-of-control (DoC), which captures the number of tunable parameters in RIS and intuitively determines the gain from incorporating an RIS into the system. Thanks to the interconnected design, I-RIS requires fewer elements to attain the same DoC than prior designs.




% Additionally, we show that with the same DoC, the complexity of finding the optimal solution with I-RIS and S-RIS is almost identical. 

%In particular, each receiver estimates its incoming channels from all transmitters using the pilot signals and then informs the others, while the estimated CSI is different from the actual CSI due to different reasons such as noise, hardware impairments, and unfavorable environments. 

Beyond the issue of interconnected elements, previous works usually used phase shifters (PSs) as RIS elements. However, simultaneously controlling the amplitude and phase of PSs is challenging. %, and PSs are lossy at high frequencies. 
Motivated by this,~\cite{mendez2016hybrid,nassirpour2022power} proposed beamforming techniques using radio frequency (RF) switches to enhance performance. Consequently, we consider RF switches as RIS elements in this work and show that our switch-based I-RIS outperforms an S-RIS using low-bit PSs.
On the other hand, the use of RF switches introduces a non-convex optimization problem. To address this problem, we propose two optimization methods: the sigmoid filled function (SFF) method and the semi-definite binary optimization (SBO) method, where the former is a heuristic approach, and the latter utilizes the successive convex approximation (SCA) method. We compare the performance of these two optimization methods with the successive-refinement (SR) method~\cite{wu2019beamforming} in terms of sum-rate and complexity. Our findings reveal: (i) the SFF method provides a higher sum-rate than the others; (ii) the complexity of the SFF method is lower than the SBO method and higher than the SR method.


The rest of this paper is organized as follows:
Section~\ref{Section:Problem} demonstrates problem setting and RIS structure. Section~\ref{Section:Beam_design} presents our beamforming
design, Section~\ref{Section:Num_results} includes numerical analysis, and Section~\ref{Section:conclusion} concludes the paper.

\textbf{Notations:} We utilize italic, bold-face lowercase, and bold-face uppercase letters to represent scalars, vectors, and matrices, respectively. We use $\mathbb{C}^{a\times b}$ to denote the space of an $a\times b$ dimensional complex-valued matrix. $\mathrm{diag}\{\textbf{a}\}$ shows a diagonal matrix using $\textbf{a}$, $\textbf{Y} \succeq \mathbf{0}$ denotes $\textbf{Y}$ is a positive semi-definite matrix, $\mathrm{blkdiag}\{\mathbf{A}, \mathbf{B}\}$ is a block diagonal matrix with $\mathbf{A}$ and $\mathbf{B}$ on its main diagonal, and $\mathrm{Diag}(\textbf{A})$ is a vector of diagonal elements in $\textbf{A}$. Here, $||\textbf{A}||_{\mathrm{F}}$ denotes the Frobenius norm of $\textbf{A}$, $A_{i,j}$ is the element in the $i^{\mathrm{th}}$ row and $j^{\mathrm{th}}$ column of $\textbf{A}$, $|a|$ is the modulus of $a$, and $||\textbf{a}||$ denotes Euclidean norm of $\textbf{a}$. Further, we use $\log(.)$, $\lfloor . \rfloor$,  $\mathrm{tr}\left(.\right)$, $\textbf{B}^{\top}$, and $\textbf{B}^H$ to indicate the logarithmic function in base 2, the floor function, the trace function, the transpose of $\textbf{B}$, and the conjugate transpose of $\textbf{B}$, respectively. We also denote sets using calligraphic font style, and for a set $\mathcal{M}$, $|\mathcal{M}|$ is its cardinality.



==> Sections/Sect1_Introduction_v2.tex <==
With the ever-increasing demand for wireless networks, the next generation of wireless networks must improve key performance metrics such as coverage, data rate, and spectrum/energy efficiency compared to the existing networks. Reconfigurable intelligent surface (RIS) has recently emerged as a promising technique, offering a range of advantages, including the capability to bypass obstacles to improve coverage and enhance data rate and spectral efficiency, all achieved in a cost-effective and power-efficient manner~\cite{zhang2020capacity,yu2019miso,bjornson2020reconfigurable}. RIS, an artificial surface comprising electromagnetic material, contains a substantial number of reflecting elements that are low-cost and (nearly-)passive, capable of independently adjusting the phase and/or amplitude of incident signals. By intelligently configuring the RIS elements, it becomes possible to combine reflected signals constructively at the intended receiver and destructively at undesired receivers.  



Due to the high path loss in the transmitter-RIS-receiver link and the passive nature of RIS, existing RISs require many elements to assist the network. In this work, we refer to the existing RIS structure as standard RIS (S-RIS), where each RIS element acts individually, and there is no interconnection between RIS elements. However, having a large-size RIS is not always feasible, especially in space-limited nodes, e.g., unmanned aerial vehicles (UAVs), where space plays a crucial role and affects the weight, power consumption, and cost of the vehicle. By minimizing the size of components and using space efficiently, UAVs can carry more payload/fuel, be more agile and responsive, and have longer flight times~\cite{ramasamy2014avionics,azarov2019composite}.  


As discussed above, small-size (i.e., compact) RIS is more desired in space-limited nodes. Thus, in this paper, we propose a new RIS structure, referred to as interconnected RIS (I-RIS), where RIS elements have interconnection with each other. In I-RIS, we divide the elements into different cells and define the elements in each cell as {\it neighbors}. Recently,~\cite{li2022reconfigurable} studied an I-RIS, where each I-RIS element receives the incident signal and reflects it either via itself or via only one of the other elements. However, in our work, each I-RIS element involves: (i) sharing its incident signal with multiple of its neighbors and (ii) reflecting a combination of the incident signals from its neighbors toward the receivers. We show that I-RIS improves user-scaling and requires fewer elements compared to S-RIS. %For example, our findings demonstrate that I-RIS, with $64$ elements, provides a $68 \%$ higher sum-rate than S-RIS with the same number of elements. Further, I-RIS needs $16$ elements to achieve a sum-rate of $6$, while S-RIS requires $64$ elements to get the same performance. The smaller size of I-RIS is feasible due to what we call the degrees-of-control (DoC), which captures the number of tunable parameters in RIS and determines the gain from incorporating an RIS into the system. Thanks to the interconnected design, to attain the same DoC, I-RIS requires fewer elements compared to prior designs.
For example, our findings demonstrate that in a single-input single-output (SISO) network serving four users, an I-RIS with $64$ elements and $16$ cells provides an $81 \%$ higher sum-rate than an S-RIS with the same number of elements. Additionally, I-RIS requires four times fewer elements to match the same sum-rate achieved by S-RIS. The smaller size of I-RIS is feasible due to what we call the degrees-of-control (DoC), which captures the number of tunable parameters in RIS and intuitively determines the gain from incorporating an RIS into the system. Thanks to the interconnected design, I-RIS needs fewer elements to get the same DoC than prior designs.




% Additionally, we show that with the same DoC, the complexity of finding the optimal solution with I-RIS and S-RIS is almost identical. 

%In particular, each receiver estimates its incoming channels from all transmitters using the pilot signals and then informs the others, while the estimated CSI is different from the actual CSI due to different reasons such as noise, hardware impairments, and unfavorable environments. 

Beyond the issue of interconnected elements, previous works usually used phase shifters (PSs) as RIS elements. However, simultaneously controlling the amplitude and phase of PSs is challenging. %, and PSs are lossy at high frequencies. 
Motivated by this,~\cite{mendez2016hybrid,nassirpour2022power} proposed beamforming techniques using radio frequency (RF) switches to enhance performance. Consequently, we consider RF switches as RIS elements in this work and show that our switch-based I-RIS outperforms an S-RIS using low-bit PSs.
On the other hand, the use of RF switches introduces a non-convex integer programming problem. To address this problem, we propose two optimization methods: the sigmoid filled function (SFF) method and the semi-definite binary optimization (SBO) method, where the former is a heuristic approach, and the latter utilizes the successive convex approximation (SCA) method. We compare the performance of these two optimization methods with the successive-refinement (SR) method~\cite{wu2019beamforming} in terms of sum-rate and complexity. Our findings reveal: (i) the SFF method provides a higher sum-rate than the others; (ii) the complexity of the SFF method is lower than the SBO method and higher than the SR method.


The rest of this paper is organized as follows:
Section~\ref{Section:Problem} demonstrates problem setting and RIS structure. Section~\ref{Section:Beam_design} presents our beamforming
design, Section~\ref{Section:Num_results} includes numerical analysis, and Section~\ref{Section:conclusion} concludes the paper.

\textbf{Notation:} We utilize italic, bold-face lowercase, and bold-face uppercase letters to represent scalars, vectors, and matrices, respectively. We use $\mathbb{C}^{a\times b}$ to denote the space of an $a\times b$ dimensional complex-valued matrix. $\mathrm{diag}\{\textbf{a}\}$ shows a diagonal matrix using $\textbf{a}$, $\textbf{Y} \succeq \mathbf{0}$ denotes $\textbf{Y}$ is a positive semi-definite matrix, $\mathrm{blkdiag}\{\mathbf{A}, \mathbf{B}\}$ is a block diagonal matrix with $\mathbf{A}$ and $\mathbf{B}$ on its main diagonal, and $\mathrm{Diag}(\textbf{A})$ is a vector of diagonal elements in $\textbf{A}$. Here, $||\textbf{A}||_{\mathrm{F}}$ denotes the Frobenius norm of $\textbf{A}$, $A_{i,j}$ is the element in the $i^{\mathrm{th}}$ row and $j^{\mathrm{th}}$ column of $\textbf{A}$, $|a|$ is the modulus of $a$, and $||\textbf{a}||$ denotes Euclidean norm of $\textbf{a}$. Further, we use $\log(.)$, $\lfloor . \rfloor$,  $\mathrm{tr}\left(.\right)$, $\textbf{B}^{\top}$, and $\textbf{B}^H$ to indicate the logarithmic function in base 2, the floor function, the trace function, the transpose of $\textbf{B}$, and the conjugate transpose of $\textbf{B}$, respectively. We also denote sets using calligraphic font style, and for a set $\mathcal{M}$, $|\mathcal{M}|$ is its cardinality.



==> Sections/Sect1_Introduction_v3.tex <==
% With the ever-increasing demand for wireless networks, the next generation of wireless networks must improve key performance metrics such as coverage, data rate, and spectrum/energy efficiency compared to the existing networks. Reconfigurable intelligent surface (RIS) has recently emerged as a promising technique, offering a range of advantages, including the capability to bypass obstacles to improve coverage and enhance data rate and spectral efficiency, all achieved in a cost-effective and power-efficient manner~\cite{zhang2020capacity,yu2019miso,bjornson2020reconfigurable}. RIS, an artificial surface comprising electromagnetic material, contains a substantial number of reflecting elements that are low-cost and (nearly-)passive, capable of independently adjusting the phase and/or amplitude of incident signals. By intelligently configuring the RIS elements, it becomes possible to combine reflected signals constructively at the intended receiver and destructively at undesired receivers.  

With the ever-increasing demand for wireless networks, the next generation must enhance key performance metrics such as coverage, data rate, and spectrum/energy efficiency compared to current networks. Reconfigurable intelligent surface (RIS) has recently emerged as a promising technique, offering advantages, including bypassing obstacles to improve coverage and enhance data rate and spectral efficiency in a cost-effective and power-efficient manner~\cite{zhang2020capacity,yu2019miso,bjornson2020reconfigurable}. RIS, an artificial surface with electromagnetic material, contains numerous reflecting elements that are low-cost and (nearly-)passive, capable of independently adjusting the phase and/or amplitude of incident signals. Intelligently configuring RIS elements allows combining reflected signals constructively at the intended receiver and destructively at undesired receivers.



% Due to the high path loss in the transmitter-RIS-receiver link and the passive nature of RIS, existing RISs require many elements to assist the network. In this work, we refer to the existing RIS structure as standard RIS (S-RIS), where each RIS element acts individually, and there is no interconnection between RIS elements, leading to a diagonal RIS matrix. However, having a large-size RIS is not always feasible, especially in space-limited nodes, e.g., unmanned aerial vehicles (UAVs), where space plays a crucial role and affects the weight, power consumption, and cost of the vehicle. By minimizing the size of components and using space efficiently, UAVs can carry more payload/fuel, be more agile and responsive, and have longer flight times~\cite{ramasamy2014avionics,azarov2019composite}.


Due to high path loss in the transmitter-RIS-receiver link and the passive nature of RIS, existing RISs, referred to as standard RIS (S-RIS), rely on many elements for network assistance; each S-RIS element acts individually, with no interconnection between elements, leading to a diagonal RIS matrix. However, achieving a large-size RIS is often impractical, especially in space-limited nodes, e.g., unmanned aerial vehicles (UAVs), where space significantly influences weight, power consumption, and vehicle cost. Minimizing component size and using space efficiently allows UAVs to enhance payload/fuel capacity, agility, and extend flight times~\cite{ramasamy2014avionics}.


As discussed above, small-size (i.e., compact) RIS is more desired in space-limited nodes. Thus, in this paper, we propose a new RIS structure, referred to as interconnected RIS (I-RIS), where RIS elements have interconnection with each other, resulting in a non-diagonal I-RIS matrix. A recent study by~\cite{an2023stacked} proposed a stacked version of reconfigurable intelligent surfaces positioned at both the transmitter and receiver sides in holographic multiple-input multiple-output (HMIMO) communications. This configuration also generates a non-diagonal matrix, enhancing spatial gain. However, the findings in~\cite{an2023stacked} are confined to a single-user scenario and are ineffective when direct links between the transmitter and receiver are obstructed. Consequently, our focus in this paper is on a multi-user scenario where these direct links are blocked. In I-RIS, we divide the elements into different cells and define the elements in each cell as {\it neighbors}. Recently,~\cite{li2022reconfigurable} studied an I-RIS, where each I-RIS element receives the incident signal and reflects it either via itself or via only one of the other elements. However, in our work, each I-RIS element involves: (i) sharing its incident signal with multiple of its neighbors and (ii) reflecting a combination of the incident signals from its neighbors toward the receivers. We show that I-RIS improves user-scaling and requires fewer elements compared to S-RIS. For example, our findings reveal that in a single-input single-output (SISO) network serving four users, an I-RIS with $64$ elements and $16$ cells provides an $81 \%$ higher sum-rate than an S-RIS with an identical element count. Moreover, I-RIS achieves the same sum-rate as S-RIS with only one-fourth of the elements. This is feasible due to what we call the degrees-of-control (DoC), which captures the number of tunable parameters in RIS and intuitively determines the gain from incorporating an RIS into the system. Thanks to the interconnected design, I-RIS needs fewer elements to get the same DoC as prior designs.



% For example, our findings reveal that in a single-input single-output (SISO) network with four users, an I-RIS with $64$ elements and $16$ cells yields an $81 \%$ higher sum-rate than an S-RIS with an identical element count. Moreover, I-RIS achieves the same sum-rate as S-RIS with only one-fourth of the elements, attributed to the degrees-of-control (DoC) concept. DoC, reflecting the tunable parameters in the RIS, determines the efficiency of incorporating an RIS into the system, and I-RIS achieves a comparable DoC with fewer elements due to its interconnected design.



% Additionally, we show that with the same DoC, the complexity of finding the optimal solution with I-RIS and S-RIS is almost identical. 

%In particular, each receiver estimates its incoming channels from all transmitters using the pilot signals and then informs the others, while the estimated CSI is different from the actual CSI due to different reasons such as noise, hardware impairments, and unfavorable environments. 

Beyond the issue of interconnected elements, prior works usually used phase shifters (PSs) as RIS elements. However, simultaneously controlling the amplitude and phase of PSs is challenging. %, and PSs are lossy at high frequencies. 
Motivated by this,~\cite{mendez2016hybrid,nassirpour2022power} proposed beamforming techniques using radio frequency (RF) switches to enhance performance. Thus, we adopt RF switches as RIS elements in this work and show that our switch-based I-RIS outperforms an S-RIS using low-bit PSs.
On the other hand, the use of RF switches poses a non-convex integer programming problem. To address this, we propose two optimization methods: the sigmoid filled function (SFF) method and the semi-definite binary optimization (SBO) method, where the former is a heuristic approach, and the latter utilizes the successive convex approximation (SCA) method. We compare these two optimization methods with the successive-refinement (SR) method~\cite{wu2019beamforming} in terms of sum-rate and complexity. Our findings reveal: (i) the SFF method provides a higher sum-rate than the others; (ii) the complexity of the SFF method is lower than the SBO method and higher than the SR method.


The rest of this paper is organized as follows:
Section~\ref{Section:Problem} demonstrates problem setting and RIS structure. Section~\ref{Section:Beam_design} presents our beamforming
design, Section~\ref{Section:Num_results} includes numerical analysis, and Section~\ref{Section:conclusion} concludes the paper.

\textbf{Notation:} We use italic, bold-face lowercase, and bold-face uppercase letters to denote scalars, vectors, and matrices, respectively. $\mathbb{C}^{a\times b}$ represents the space of an $a\times b$ dimensional complex-valued matrix. $\mathrm{diag}\{\textbf{a}\}$ is a diagonal matrix using $\textbf{a}$, $\textbf{Y} \succeq \mathbf{0}$ denotes $\textbf{Y}$ is a positive semi-definite matrix, $\mathrm{blkdiag}\{\mathbf{A}, \mathbf{B}\}$ is a block diagonal matrix with $\mathbf{A}$ and $\mathbf{B}$ on its main diagonal, and $\mathrm{Diag}(\textbf{A})$ is a vector of diagonal elements in $\textbf{A}$. $||\textbf{A}||_{\mathrm{F}}$ is the Frobenius norm of $\textbf{A}$, $A_{i,j}$ is the element in the $i^{\mathrm{th}}$ row and $j^{\mathrm{th}}$ column of $\textbf{A}$, $|a|$ is the modulus of $a$, and $||\textbf{a}||$ denotes Euclidean norm of $\textbf{a}$. We use $\log(.)$, $\lfloor . \rfloor$,  $\mathrm{tr}\left(.\right)$, $\textbf{B}^{\top}$, and $\textbf{B}^H$ to indicate the logarithmic function in base 2, the floor function, the trace function, the transpose of $\textbf{B}$, and the conjugate transpose of $\textbf{B}$, respectively. We denote sets using calligraphic font style, and for a set $\mathcal{M}$, $|\mathcal{M}|$ is its cardinality.




==> Sections/Sect2_Problem_setting_RIS_structure.tex <==
In this paper, we examine an RIS-assisted network with distributed transmitter-receiver pairs where each transmitter aims to communicate with only one desired receiver, as shown in Fig.~\ref{Fig:channel_model_standard_RIS}. Further, we focus on a SISO scenario to highlight the pure RIS gain in the network.
\begin{figure}[ht]
\vspace{-3mm}
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=6, width=0.82\linewidth, draft=false]{images/channel_model_IRIS.png}
  \vspace{-2mm}
  \caption{A SISO network with an RIS assisting multi-user communications.%\avc{Remove the controller from the figure, it is weird that the RIS is controlled by the BS rather than a big host ship. Maybe add a UAV too. Watch: https://www.youtube.com/watch?v=P2tSwngihp0}
}\label{Fig:channel_model_standard_RIS}
  %\vspace{-7mm}
\end{figure}
\subsection{Channel model}
We represent the channels between ${\sf Tx}_j$ and RIS and the channels between RIS and ${\sf Rx}_{k}$ at time $t$ as $\textbf{h}^{[j]}(t) \in \mathbb{C}^{M\times 1}$ and $\textbf{g}^{[k]}(t) \in \mathbb{C}^{1\times M}$, respectively, where $j,k \in \{1,2,\ldots,K\}$, $K$ is the number of transmitter-receiver pairs, and $M$ denotes the number of RIS elements. We use Rician fading to model $\textbf{h}^{[j]}(t)$ and express $h_m^{[j]}(t)$, the $m^{\mathrm{th}}$ element of $\textbf{h}^{[j]}(t), 1 \leq m \leq M$, as follows:
\begin{align}
    \label{eq:Rician_fading}
    h_m^{[j]}(t)=\sqrt{\frac{1}{1+\kappa}}h_m^{[j],NLoS}(t)+\sqrt{\frac{\kappa}{1+\kappa}}h_m^{[j],LoS},
\end{align}
where $\kappa$ is the Rician factor, $h_m^{[j],NLoS}(t) \thicksim \mathcal{CN}(0,C_0d_{1,j}^{-\alpha_1})$ represents the non-line-of-sight (NLoS) component of $h_m^{[j]}(t)$, and $h_m^{[j],LoS}=\sqrt{C_0d_{1,j}^{-\alpha_1}}e^{-j\frac{2 \pi }{\lambda}d_{1,j}}$ shows the line-of-sight (LoS) part of $h_m^{[j]}(t)$, where $d_{1,j}$ denotes the distance between ${\sf Tx}_j$ and RIS, $\alpha_1$ is the path loss exponent between them, and $\lambda$ is the wavelength of the transmitted signal. We use $C_0$ to capture the signal loss at a reference distance, e.g., $1\mathrm{m}$. Here, $\textbf{g}^{[k]}(t)$ follows Rayleigh fading whose elements are modeled as a complex Gaussian distribution with zero mean and variance $C_0d_{2,k}^{-\alpha_2}$, where $d_{2,k}$ and $\alpha_2$ denote the distance and path loss exponent between RIS and ${\sf Rx}_k$, respectively. 

In this work, we assume that the direct path between transmitters and receivers is blocked. We also suppose that the channels are independent due to the spacing of the RIS elements being at least $\lambda/2$ apart. Similar to~\cite{fu2021reconfigurable,wu2019intelligent}, we assume that channel state information (CSI) is available globally, and beyond that, there is no data exchange between transmitters or receivers. We note that all operations occur within a single coherence time; hence, we omit the time notation throughout the rest of this paper.

\begin{comment}
\textbf{CSI resolution:} In this work, we assume that each receiver estimates its incoming channels from all transmitters using the pilot signals and then informs the others, while the estimated CSI is different from the actual CSI due to different reasons such as noise, hardware impairments, and unfavorable environments. Thus, we have: 
\begin{align}
    &\hat{\textbf{h}}^{[j]}(t) = \textbf{h}^{[j]}(t) + \mathbf{e}^{[j]}_h(t),~~1 \leq j \leq K,\\ \nonumber
    &\hat{\textbf{g}}^{[k]}(t) = \textbf{g}^{[k]}(t) + \mathbf{e}^{[k]}_g(t),~~1 \leq k \leq K,
\end{align}
where $\mathbf{e}^{[j]}_h(t)\in \mathbb{C}^{M\times 1}$ and $\mathbf{e}^{[k]}_g(t)\in \mathbb{C}^{1\times M}$ are the estimation errors whose elements are distributed based on $\mathcal{CN}(0,1/p)$, and $p$ denotes the signal-to-noise ratio (SNR) during the estimation process.
\end{comment}

\begin{figure*}[ht]
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=9, width=0.99\linewidth, draft=false]{images/std_general_RIS_models_3.png}
  \vspace{-3mm}
  \caption{(a) A $32$-element S-RIS, where the $m^{\mathrm{th}}$ RIS element uses an RF switch to either reflect or block its incident signal; (b) An I-RIS with $32$ elements and eight cells of size $(2,2)$; (c) The $m^{\mathrm{th}}$ arrival element uses $c\times d$ RF switches and a power splitter to share its incident signal; (d) The reflected signal from the $m^{\mathrm{th}}$ departure element includes a combination of the incident signals at all arrival elements.}\label{Fig:channel_model_new_RIS}
  %\vspace{-5mm}
\end{figure*}
%\vspace{10mm}
\subsection{Existing vs. the proposed RIS design}
In this subsection, we delve into the details of two RIS structures using RF switches. Here, each RIS element has an arrival part that receives the incident signals from transmitters and a departure part that reflects the signals toward receivers.% We place a controller between a control unit, e.g., a shore control center, and the RIS to exchange CSI and control RIS elements over a separate communication link.

\textbf{S-RIS:} In this RIS, there is no interconnection between the elements. The $m^{\mathrm{th}}$ RIS element, $1 \leq m \leq M$, receives the incident signal and then uses its binary RF switch, $s_{m}\in \{0,1\}$ between its arrival and departure parts, to either reflect or block its incident signal as shown in Fig.~\ref{Fig:channel_model_new_RIS}(a). We define $\mathbf{T}^{\mathrm{s}}$ as the S-RIS configuration, which is given by:
\begin{align}
    \mathbf{T}^{\mathrm{s}}=\mathrm{diag}\left\{\boldsymbol{\tau}^{\mathrm{s}}\right\},~~~\boldsymbol{\tau}^{\mathrm{s}}=\left[s_{1},s_{2},\ldots,s_{M}\right]^{\top}.
\end{align}

\textbf{I-RIS:} In this case, we first divide RIS into $M/cd$ different cells{\footnote{Without loss of generality, we suppose $M$ is divisible by $cd.$}}, where $c$ and $d$ denote the cell size. (e.g., Fig.~\ref{Fig:channel_model_new_RIS}(b) shows a $32$-element I-RIS with eight cells of size $(2, 2)$.) Next, each element within a given cell shares its incident signal with its neighbors in that cell, as depicted in Fig.~\ref{Fig:channel_model_new_RIS}(c). We use $\mathcal{M}^{[m]}$ to denote the cell that includes the $m^{\mathrm{th}}$ element. Thereafter, the $m^{\mathrm{th}}$ RIS element uses $cd$ binary RF switches to determine  $\bar{\mathcal{M}}^{[m]}\subseteq \mathcal{M}^{[m]}$, which contains the elements in the cell obtaining the incident signal received by the $m^{\mathrm{th}}$ arrival element. The $m^{\mathrm{th}}$ arrival element utilizes a power splitter to distribute the incident signal power uniformly across all members of $\bar{\mathcal{M}}^{[m]}$. Then, to indicate how the $m^{\mathrm{th}}$ arrival element connects to the $\ell^{\mathrm{th}}$ departure element, $1\leq \ell,M\leq M$, we define $\tau^{\mathrm{i}}_{\ell m}$ as below:
\begin{align}
\tau^{\mathrm{i}}_{\ell m}=\left\{ \begin{array}{ll} \frac{1}{\sqrt{\left|\bar{\mathcal{M}}^{[m]}\right|}}s_{\ell m}, & \ell\in \bar{\mathcal{M}}^{[m]}, \\
0, & \ell\notin \bar{\mathcal{M}}^{[m]},
\end{array} \right.
\end{align}
where $s_{\ell m}\in \{0,1\}$ is a binary RF switch between the $m^{\mathrm{th}}$ arrival element and the $\ell^{\mathrm{th}}$ departure element, and $\frac{1}{\sqrt{\left|\bar{\mathcal{M}}^{[m]}\right|}}$ guarantees $\sum_{\ell=1}^M |\tau^{\mathrm{i}}_{\ell m}|^2=1$, i.e., RIS elements are passive. We note that I-RIS is nearly-passive as it requires control signals to activate or deactivate its RF switches. %\avc{1. ``.'' then i.e., does not work, 2. the sentence after i.e. is not well written, it simply means sharing is useless, you want to say the I-RIS elements are passive} (i.e., there is no gain from power sharing at the $m^{\mathrm{th}}$ arrival element.)
Then, we use $\mathbf{T}^{\mathrm{i}}$ to denote the I-RIS configuration as:
\begin{align}
    \mathbf{T}^{\mathrm{i}}=\mathrm{blkdiag}\left\{\boldsymbol{\tau}^{\mathrm{i}[1]},\boldsymbol{\tau}^{\mathrm{i}[2]}, \ldots, \boldsymbol{\tau}^{\mathrm{i}[\frac{M}{cd}]}\right\},
\end{align}
where $\boldsymbol{\tau}^{\mathrm{i}[u]}, 1\leq u \leq \frac{M}{cd}$ follows \eqref{eq:tau_general_vector} (at the top of the next page).
\begin{figure*}
\begin{align}
\label{eq:tau_general_vector}
    \boldsymbol{\tau}^{\mathrm{i}[u]}= \begin{bmatrix}
\tau^{\mathrm{i}}_{[(u-1)cd+1][(u-1)cd+1]} & \tau^{\mathrm{i}}_{[(u-1)cd+1][(u-1)cd+2]} & \ldots & \tau^{\mathrm{i}}_{[(u-1)cd+1][ucd]}\\
\vdots & \vdots & \ldots & \vdots
\\
\tau^{\mathrm{i}}_{[ucd][(u-1)cd+1]} & \tau^{\mathrm{i}}_{[ucd][(u-1)cd+2]} & \ldots & \tau^{\mathrm{i}}_{[ucd][ucd]}
\end{bmatrix}, & ~1\leq u \leq \frac{M}{cd}.
\end{align}
\hrule
\end{figure*}
Finally, based on Fig.~\ref{Fig:channel_model_new_RIS}(d), the $m^{\mathrm{th}}$ departure element mixes the incident signals of all elements in $\mathcal{M}^{[m]}$ and then reflects a combination of them toward the receivers.

\textbf{Received signal:} ${\sf Rx}_{k}$ receives the reflected signals from the RIS, which is given by:
\begin{align}
\label{eq_ch5:received_sig_a_RIS}
    y_{k}=\sum_{j=1}^K \Big[\textbf{g}^{[k]}\mathbf{T}\textbf{h}^{[j]}\Big]x_j+n_{k},
\end{align}
where $\mathbf{T} \in \left\{\mathbf{T}^{\mathrm{s}}, \mathbf{T}^{\mathrm{i}}\right\}$, $x_j$ is the transmitted signal from ${\sf Tx}_j$, and $n_{k} \thicksim \mathcal{CN}(0,\sigma^2)$ denotes noise at ${\sf Rx}_{k}$. Here, $\mathbb{E}\left\{\textbf{x}\textbf{x}^{H}\right\}=\mathrm{diag}([P_1, P_2,\ldots,P_K])$, where $\textbf{x}=[x_1,x_2,\ldots,x_K] \in \mathbb{C}^{1\times K}$, and $P_j$ is the transmit power from ${\sf Tx}_j$.  Then, we use \eqref{eq_ch5:received_sig_a_RIS} to express the signal-to-interference-plus-noise ratio (SINR) at ${\sf Rx}_{k}$ as follows:
\begin{align}
\label{eq_ch5:SINR_update_a_RIS}
    \text{SINR}_{k}=\frac{P_{k}\Big|\textbf{g}^{[k]}\mathbf{T}\textbf{h}^{[k]}\Big|^2}{\sigma^2+\sum_{j=1, j\neq k}^{K }P_j\Big|\textbf{g}^{[k]}\mathbf{T}\textbf{h}^{[j]}\Big|^2}.
\end{align} 


==> Sections/Sect2_Problem_setting_RIS_structure_USV.tex <==
In this paper, we examine a SISO maritime network with distributed transmitter-receiver pairs where each transmitter aims to communicate with one desired receiver, as shown in Fig.~\ref{Fig:channel_model_standard_RIS}. Further, we incorporate a USV with an \newwRIS, which fits limited-size USVs to assist the network.

\subsection{Channel model}
We represent the channels between ${\sf Tx}_j$ and RIS and the channels between RIS and ${\sf Rx}_i$ at time $t$ as $\textbf{h}^{[j]}(t) \in \mathbb{C}^{M\times 1}$ and $\textbf{g}^{[i]}(t) \in \mathbb{C}^{1\times M}$, respectively, where $i,j \in \{1,2,\ldots,K\}$, $K$ is the number of transmitter-receiver pairs, and $M$ denotes the number of RIS elements. We use Rician fading to model $\textbf{h}^{[j]}(t)$ and express $h_m^{[j]}(t)$, the $m^{\mathrm{th}}$ element of $\textbf{h}^{[j]}(t), 1 \leq m \leq M$, as follows:
\begin{align}
    \label{eq:Rician_fading}
    h_m^{[j]}(t)=\sqrt{\frac{1}{1+\kappa}}h_m^{[j],NLoS}(t)+\sqrt{\frac{\kappa}{1+\kappa}}h_m^{[j],LoS},
\end{align}
where $\kappa$ is the Rician factor, $h_m^{[j],NLoS}(t) \thicksim \mathcal{CN}(0,C_0d_{1,j}^{-\alpha_1})$ represents the non-line-of-sight (NLoS) component of $h_m^{[j]}(t)$, and $h_m^{[j],LoS}=\sqrt{C_0d_{1,j}^{-\alpha_1}}e^{-j\frac{2 \pi }{\lambda}d_{1,j}}$ shows the line-of-sight (LoS) part of $h_m^{[j]}(t)$, where $d_{1,j}$ denotes the distance between ${\sf Tx}_j$ and RIS, $\alpha_1$ is the path loss exponent between them, and $\lambda$ is the wavelength of the transmitted signal. We use $C_0$ to capture the signal loss at a reference distance, e.g., $1\mathrm{m}$. We assume that $\textbf{g}^{[i]}(t)$ follows Rayleigh fading whose elements are modeled as a complex Gaussian distribution with zero mean and variance $C_0d_{2,i}^{-\alpha_2}$, where $d_{2,i}$ and $\alpha_2$ denote the distance and path loss exponent between RIS and ${\sf Rx}_i$, respectively.


We consider that the maritime network includes obstructions, such as islands, that block the direct path between transmitters and receivers. We also assume that $\textbf{h}^{[j]}(t)$ and $\textbf{g}^{[i]}(t)$ are independent over time and users due to the spacing of the RIS elements being at least $\lambda/2$ apart. Similar to~\cite{fu2021reconfigurable,wu2019intelligent}, we assume that CSI is available globally and beyond that there is no data exchange between transmitters or receivers.
\begin{figure}[htb]
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=9, width=0.99\linewidth, draft=false]{images/system_model_USV_5.png}
  \vspace{-5mm}
  \caption{\it A SISO maritime network with an RIS installed on a USV assisting multi-user communications.%\avc{Remove the controller from the figure, it is weird that the RIS is controlled by the BS rather than a big host ship. Maybe add a UAV too. Watch: https://www.youtube.com/watch?v=P2tSwngihp0}
  }\label{Fig:channel_model_standard_RIS}
  %\vspace{-7mm}
\end{figure}

\begin{figure*}[ht]
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=9, width=0.99\linewidth, draft=false]{images/std_general_RIS_models_2.png}
  \vspace{-3mm}
  \caption{\it (a) A $32$-element S-RIS, where the $m^{\mathrm{th}}$ element uses a switch to either reflect or block its incident signal; (b) An \newRIS with $32$ elements, which is partitioned into $8$ cells where $c=d=2$; (c) The $m^{\mathrm{th}}$ arrival element uses $cd$ switches and a power splitter to share its incident signal; (d) The reflected signal from the $m^{\mathrm{th}}$ departure element includes a combination of the incident signals at all arrival elements.}\label{Fig:channel_model_new_RIS}
  %\vspace{-5mm}
\end{figure*}

\textbf{CSI resolution:} Due to hardware impairments, ${\sf Rx}_i$ estimates its incoming channels with errors. Thus, we have:
\begin{align}
    &\hat{\textbf{h}}^{[j]}(t) = \textbf{h}^{[j]}(t) + \mathbf{e}^{[j]}_h(t),~~1 \leq j \leq K,\\ \nonumber
    &\hat{\textbf{g}}^{[i]}(t) = \textbf{g}^{[i]}(t) + \mathbf{e}^{[i]}_g(t),~~1 \leq i \leq K,
\end{align}
where $\mathbf{e}^{[j]}_h(t)\in \mathbb{C}^{M\times 1}$ and $\mathbf{e}^{[i]}_g(t)\in \mathbb{C}^{1\times M}$ are the estimation errors whose elements are distributed based on $\mathcal{CN}(0,1/p)$, and $p$ denotes the signal-to-noise ratio (SNR) during the estimation process.

\subsection{RIS structures}
In this section, we explain two structures of switch-based RIS. Each RIS element has an arrival part to receive the incident signals from transmitters and a departure part to reflect the signals towards receivers. We place a controller between a control unit, e.g., a shore control center, and the RIS to exchange CSI and control RIS elements over a separate communication link.

\textbf{S-RIS:} In this RIS, there is no interconnection between the elements. The $m^{\mathrm{th}}$ RIS element, $1 \leq m \leq M$, receives the incident signal and then uses its binary RF switch, $s_{m}(t)\in \{0,1\}$ between its arrival and departure parts, to either reflect or block its received signal at time $t$ as Fig.~\ref{Fig:channel_model_new_RIS}(a). We define $\mathbf{T}^{s}(t)$ as the S-RIS configuration, which is given by:
\begin{align}
    \mathbf{T}^{s}(t)=\mathrm{diag}\left\{\boldsymbol{\tau}^{s}(t)\right\},
\end{align}
where
\begin{align}
    \boldsymbol{\tau}^{s}(t)=\left[s_{1}(t),s_{2}(t),\ldots,s_{M}(t)\right]^{\top}.
\end{align}

\textbf{\newwRIS:} In this case, we first partition the RIS into $M/cd$ different cells{\footnote{Without loss of generality, we suppose $M$ is divisible by $cd.$}}, where $c$ and $d$ show the cell dimensions. (e.g., Fig.~\ref{Fig:channel_model_new_RIS}(b) shows a $32$-element \newRIS with $8$ cells.) Next, each element in a given cell shares its received signal with others in that cell as depicted in Fig.~\ref{Fig:channel_model_new_RIS}(c). We use $\mathcal{M}^{[m]}$ to denote the cell that includes the $m^{\mathrm{th}}$ element, where
\begin{align}
    &\mathcal{M}^{[m]} = \\ \nonumber
    &\left\{ \begin{array}{ll} \big\{\lfloor \frac{m}{cd} \rfloor cd+1,\lfloor \frac{m}{cd} \rfloor cd+2,\ldots,\lfloor \frac{m}{cd} \rfloor cd+cd \big\}, & \lfloor \frac{m}{cd} \rfloor\neq \frac{m}{cd}, \\
\big\{m-cd+1,m-cd+2,\ldots,m \big\}, & \lfloor \frac{m}{cd} \rfloor = \frac{m}{cd}.
\end{array} \right.
\end{align}

Thereafter, the $m^{\mathrm{th}}$ RIS element uses $cd$ binary RF switches to determine  $\bar{\mathcal{M}}^{[m]}\subseteq \mathcal{M}^{[m]}$, which contains the elements in the cell obtaining the incident signal received by the $m^{\mathrm{th}}$ arrival element. 
The $m^{\mathrm{th}}$ arrival elements utilizes a power splitter to distribute the received signal power uniformly across all members of $\bar{\mathcal{M}}^{[m]}$. Then, to indicate how the $m^{\mathrm{th}}$ arrival element connects to the $\ell^{\mathrm{th}}$ departure element at time $t$, we define $\tau^{i}_{\ell m}(t)$ as below:
\begin{align}
    \tau^i_{\ell m}(t)=\left\{ \begin{array}{ll} \frac{1}{\sqrt{\big|\bar{\mathcal{M}}^{[m]}\big|}}s_{\ell m}(t), & \ell\in \bar{\mathcal{M}}^{[m]}, \\
0, & \ell\notin \bar{\mathcal{M}}^{[m]},
\end{array} \right.
\end{align}
where $s_{\ell m}(t)\in \{0,1\}$ is a binary RF switch between the $m^{\mathrm{th}}$ arrival element and the $\ell^{\mathrm{th}}$ departure element, and $\frac{1}{\sqrt{\big|\bar{\mathcal{M}}^{[m]}\big|}}$ guarantees that $\sum_{\ell=1}^M |\tau^i_{\ell m}(t)|^2=1$. (i.e., there is no gain from power sharing at the $m^{\mathrm{th}}$ arrival element.) Then, we use $\mathbf{T}^i(t) \in \mathbb{C}^{M \times M}$ to denote the \newRIS configuration as:
\begin{align}
    \mathbf{T}^i(t)=\mathrm{blkdiag}\left\{\boldsymbol{\tau}^{i[1]}(t),\boldsymbol{\tau}^{i[2]}(t), \ldots, \boldsymbol{\tau}^{i[\frac{M}{cd}]}(t)\right\},
\end{align}
where $\boldsymbol{\tau}^{i[u]}(t)$ follows \eqref{eq:tau_general_vector} on top of the next page.
\begin{figure*}
\begin{align}
\label{eq:tau_general_vector}
    \boldsymbol{\tau}^{i[u]}(t)= \begin{bmatrix}
\tau^i_{[(u-1)cd+1][(u-1)cd+1]}(t) & \tau^i_{[(u-1)cd+1][(u-1)cd+2]}(t) & \ldots & \tau^i_{[(u-1)cd+1][ucd]}(t)\\
\vdots & \vdots & \ldots & \vdots
\\
\tau^i_{[ucd][(u-1)cd+1]}(t) & \tau^i_{[ucd][(u-1)cd+2]}(t) & \ldots & \tau^i_{[ucd][ucd]}(t)
\end{bmatrix}, & \quad 1\leq u \leq \frac{M}{cd}.
\end{align}
\hrule
\end{figure*}
Finally, based on Fig.~\ref{Fig:channel_model_new_RIS}(d), the $m^{\mathrm{th}}$ departure element mixes the received signals at all elements in $\mathcal{M}^{[m]}$ and then reflects a combination of them toward the receivers.

\textbf{Received signal:} The received signal at ${\sf Rx}_i$ is the reflected signal from the RIS, which is given by:
\begin{align}
\label{eq:received_sig_a_RIS}
    y_i(t)=\sum_{j=1}^K \Big[\textbf{g}^{[i]}(t)\mathbf{T}(t)\textbf{h}^{[j]}(t)\Big]x_j(t)+n_i(t),
\end{align}
where $\mathbf{T}(t) \in \{\mathbf{T}^{s}(t), \mathbf{T}^i(t)\}$, $x_j(t)$ represents the transmitted signal from ${\sf Tx}_j$, and $n_i(t) \thicksim \mathcal{CN}(0,\sigma^2)$ denotes noise at ${\sf Rx}_i$. Here, $\mathbb{E}\left\{\textbf{x}(t)\textbf{x}^{H}(t)\right\}=\mathrm{diag}([P_1, P_2,\ldots,P_K])$, where $\textbf{x}(t)=[x_1(t),x_2(t),\ldots,x_K(t)] \in \mathbb{C}^{1\times K}$, and $P_j, j\in \{1,2,\ldots K\}$ is the transmit power from ${\sf Tx}_j$. We note that all operations occur within a single coherence time; hence, we omit the time notation throughout the rest of this work. Then, we use \eqref{eq:received_sig_a_RIS} to express the signal-to-interference-plus-noise ratio (SINR) at ${\sf Rx}_i$ as follows:
\begin{align}
\label{eq:SINR_update_a_RIS}
    \text{SINR}_i=\frac{P_i\Big|\textbf{g}^{[i]}\mathbf{T}\textbf{h}^{[i]}\Big|^2}{\sigma^2+\sum_{j=1, j\neq i}^{K }P_j\Big|\textbf{g}^{[i]}\mathbf{T}\textbf{h}^{[j]}\Big|^2}.
\end{align} 


==> Sections/Sect2_Problem_setting_RIS_structure_USV_v0.tex <==
We consider a SISO maritime network with $K$-pair distributed transmitters and receivers as Fig.~\ref{Fig:channel_model_standard_RIS}, where each transmitter and receiver has a single antenna. We use a USV, which is equipped with an $M$-element RIS to assist the network. 

\subsection{Channel model}
We use $\textbf{h}^{[j]}(t) \in \mathbb{C}^{M\times 1}$ and $\textbf{g}^{[i]}(t) \in \mathbb{C}^{1\times M}$ to denote the channels between ${\sf Tx}_j$ and the RIS and the channels between the RIS and ${\sf Rx}_i$, respectively, at time $t$, where $i,j \in \{1,2,\ldots,K\}$. To specify the channels, we will discuss the small-scale fading and large-scale fading later in this section. Notice that channels $\textbf{h}^{[j]}(t)$ and $\textbf{g}^{[i]}(t)$
are independent across time and users since we assume RIS elements are spaced at least $\lambda/2$
apart from each other where $\lambda$ is the wavelength of the transmitted signal. In this network, we assume there are obstacles (e.g., island), which block the direct path between transmitters and receivers.

\textbf{Available CSI at transmitters:} Similar to~\cite{wu2019beamforming,wu2019intelligent,fu2021reconfigurable,bafghi2022degrees}, we assume that the global CSI is available at the transmitters and rather than that no further data is exchanged between the transmitters.
\begin{figure}[htb]
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=9, width=0.99\linewidth, draft=false]{images/system_model_USV_2.png}
  \vspace{-3mm}
  \caption{\it 
  (a) A $K$-user SISO interference channel with an RIS where the RIS is equipped with $M$ reconfigurable
elements; (b) We use an attenuator and a phase shifter to change the amplitude and phase between the $m^{\mathrm{th}}$ arrival port and the $m^{\mathrm{th}}$ departure port using the standard RIS at time $t$.}\label{Fig:channel_model_standard_RIS}
  %\vspace{-7mm}
\end{figure}

\textbf{Available CSI at receivers:} We presume that the global CSI is available at each receiver since the CSI is required to determine the RIS configuration and afterwards decode the desired message at each receiver. There is also no further data exchange between the receivers other than CSI.


\begin{figure*}[ht]
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=9, width=0.99\linewidth, draft=false]{images/std_general_RIS_models.png}
  \vspace{-3mm}
  \caption{\it 
  (a) A $32$-element RIS, which is partitioned into $8$ cells where $c=d=2$; (b) In the general RIS case, the received signal at the $\ell^{\mathrm{th}}$ arrival port in a given cell can be divided between the other elements in that cell; (c) The reflected signal from the $m^{\mathrm{th}}$ departure port in a certain cell includes a combination of the incident signals at all arrival ports in that cell.}\label{Fig:channel_model_new_RIS}
  %\vspace{-7mm}
\end{figure*}
To make the global CSI available at each node, we assume each receiver estimates its incoming channels from all transmitters perfectly and then informs the others about these channels through two cases: (1) The noiseless links, which represent that other network nodes learn the channels as the receivers; (2) The noisy links, which means that the information provided to the transmitters is noisy. We refer this to as ``noisy-$p$'' channels if  other nodes attain the channels at SNR $=p$ dB.  

To characterize the above communication channels, we consider the small-scale fading and large-scale fading as below:

\textbf{Small-scale fading:} In practice, the RIS is usually positioned with knowledge of the BS's location. However, having a pure LoS signal between the BS and the RIS is not always feasible, especially in urban areas. As a result, we consider $\textbf{h}^{[j]}(t)$ is distributed based on Rician fading distribution. Here, we write $h_m^{[j]}(t)$, the $m^{\mathrm{th}}$ element of $\textbf{h}^{[j]}(t)$, as
\begin{align}
    \label{eq:Rician_fading}
    h_m^{[j]}(t)=\sqrt{\frac{1}{1+\kappa}}h_m^{[j],NLoS}(t)+\sqrt{\frac{\kappa}{1+\kappa}}h_m^{[j],LoS},
\end{align}
where $\kappa$ describes Rician factor, $h_m^{[j],NLoS}(t) \thicksim \mathcal{CN}(0,\Tilde{\sigma}_h^2)$, and $h_m^{[j],LoS}=e^{-j\frac{2 \pi }{\lambda}d^{\prime}_{j}}$ where $d^{\prime}_{j}$ shows the distance between ${\sf Tx}_j$ and the RIS. In this case, we say $h_m^{[j]}(t)$ is distributed based on a random distribution with mean $m^{[j]}_{h}$ and variance $\sigma_h^2$ where
\begin{align}
m^{[j]}_h=\sqrt{\frac{\kappa}{1+\kappa}}e^{-j\frac{2 \pi }{\lambda}d^{\prime}_{j}}, \quad \quad
\sigma_h^2=\frac{1}{1+\kappa}\Tilde{\sigma}_h^2.
\end{align}

On the contrary, due to the user’s mobility and the
complex propagation environment, having LoS channel for $\textbf{g}^{[i]}(t)$ is impossible in practice; thus, we assume $\textbf{g}^{[i]}(t)$ is distributed based on Rayleigh fading, which means that each element of $\textbf{g}^{[i]}(t)$ is distributed based on $\mathcal{CN}(0,\sigma_g^2)$ where $\sigma_g^2$ shows the variance. 

\textbf{Large-scale fading:} We use $C_0 d^{-\alpha}$ as the path loss profile where $C_0$ describes the signal loss at a reference distance (e.g., $1m$), $d$ is the distance between a pair of nodes (e.g., ${\sf Tx}_j$ and RIS) and $\alpha$ represents the corresponding path loss component.

For simplicity, in the rest of the paper, we use $m^{[j]}_h$, $\sigma_h^2$, and $\sigma_g^2$ to denote the mean of $h_m^{[j]}(t)$, the variance of $h_m^{[j]}(t)$, and the variance of each element of $\textbf{g}^{[i]}(t)$, respectively, which include the impact of both small-scale fading and large-scale fading. 

\textbf{RIS configuration:}In particular, we propose two  in two ways: (1) a standard RIS where each RIS element varies the phase and amplitude of its incident signals from the transmitters and then reflects them toward the receivers; and (2) a general RIS in which the RIS elements are partitioned into different cells and each RIS element in a certain cell can share its incident signals with other elements in that cell and then reflects a combination of the incident signals toward the receivers. In this paper, we assume a %{\color{red} remove smart for controller everywhere in the text}
controller between one of the transmitters (e.g., ${\sf Tx}_1$ in Fig.~\ref{Fig:channel_model_standard_RIS}(a)) and the RIS to exchange CSI and control the RIS elements over a separate communication link. Moreover, we only consider the first reflected signal from the RIS due to the significant path loss and ignore the hardware imperfection features (e.g, non-linearity) at the RIS. We suppose that each RIS element has two ports: arrival port and departure port, where the former is the place where it receives the incident signals from transmitters and the latter is the location where it reflects the signals toward the receivers. Therefore, in this paper, we focus on two RIS-based instances as follows.

{$\bullet$ \textbf{Case I (standard RIS)}}

In this case, the $m^{\mathrm{th}}$ element of the RIS uses amplitude $\beta_{mm}(t)$ and phase $\theta_{mm}(t)$ to adjust the amplitude and phase of the incident signals received at the $m^{\mathrm{th}}$ arrival port and then reflects them via the $m^{\mathrm{th}}$ departure port at time $t$ as Fig.~\ref{Fig:channel_model_standard_RIS}(b). %In the rest of this manuscript, we use tuple $(\beta_{mm}(t),\theta_{mm}(t))$ to denote the amplitude and phase change between the $m^{\mathrm{th}}$ arrival port and the $m^{\mathrm{th}}$ departure port at time $t$.
Suppose $s_m(t)$ is the incident signal, received by the $m^{\mathrm{th}}$ RIS element at time $t$, and $\tau^{st}_{mm}(t)$ represents the amplitude and phase change between the $m^{\mathrm{th}}$ arrival port and the $m^{\mathrm{th}}$ departure port. Then, we have the reflected signal from the $m^{\mathrm{th}}$ element of the RIS at time $t$ as
\begin{align}
    r_m(t)=s_m(t) \tau^{st}_{mm}(t)=s_m(t)\left[\beta_{mm}(t)e^{j\theta_{mm}(t)}\right], \quad 1\leq m \leq M, 
\end{align}
where $\beta_{mm}(t) \in[0,1]$ and $\theta_{mm}(t) \in [0,2\pi)$. Recently, \cite{nayeri2018reflectarray,wu2019towards,wu2019intelligent} have shown that it is hard to control $\beta_{mm}(t)$ and $\theta_{mm}(t)$ separately in the real-world scenarios; therefore, we consider $\beta_{mm}(t)=1$ (i.e., perfect reflectors). 
We also assume that each RIS element has a $b$-bit PS, which results in $N=2^b$ quantized levels for each RIS element. For simplicity, we assume these $N$ levels are distributed uniformly in $[0,2\pi)$. We define $\phi_N$, the set of quantized values of $\theta_{mm}(t)$, as
\begin{align}
\label{eq:phi_N}
    \phi_N=\left\{0,\frac{2\pi}{N},\frac{4\pi}{N},\ldots,\frac{2\pi(N-1)}{N}\right\}.
\end{align}

Moreover, we define $\mathbf{T}^{st}(t)$ as the standard RIS configuration, which is given by
\begin{align}
    \mathbf{T}^{st}(t)=\mathrm{diag}\{\boldsymbol{\tau}^{st}(t)\},
\end{align}
where
\begin{align}
    \boldsymbol{\tau}^{st}(t)=\left[\tau^{st}_{11}(t),\tau^{st}_{22}(t),\ldots,\tau^{st}_{MM}(t)\right]=\left[e^{j\theta_{11}(t)},e^{j\theta_{22}(t)},\ldots,e^{j\theta_{MM}(t)}\right].
\end{align}

{$\bullet$ \textbf{Case II (general RIS)}} 

%{\color{red} Sajjad, the entire report I wanted is this part. Please make it accurate and bullet proof. Next round I want it to be in great shape.}

In this case, we partition the RIS into $M/cd$ different cells, where $c$ and $d$ show the cell dimensions.{\footnote{Without loss of generality, we suppose $M$ is divisible by $cd.$}}(e.g., Fig.~\ref{Fig:channel_model_new_RIS}(a) depicts a $32$-element RIS, which is partitioned into $8$ cells.) Then, we assume that each RIS element in a given cell can share its received signal with others in that cell as depicted in Fig.~\ref{Fig:channel_model_new_RIS}(b). In particular, we divide the received signal at the $\ell^{\mathrm{th}}, 1\leq \ell \leq M$ arrival port between all members of %$\mathcal{T}^{[\ell]}(t)\subseteq 
$\mathcal{M}^{[\ell]}$ where
\begin{align}
    \mathcal{M}^{[\ell]}\subseteq\left\{ \begin{array}{ll} \big\{\lfloor \frac{\ell}{cd} \rfloor cd+1,\lfloor \frac{\ell}{cd} \rfloor cd+2,\ldots,\lfloor \frac{\ell}{cd} \rfloor cd+cd \big\}, & \lfloor \frac{\ell}{cd} \rfloor\neq \frac{\ell}{cd}, \\
\big\{\ell-cd+1,\ell-cd+2,\ldots,\ell \big\}, & \lfloor \frac{\ell}{cd} \rfloor = \frac{\ell}{cd}.
\end{array} \right.
\end{align}

For simplicity, we consider a simple power splitter at the $\ell^{\mathrm{th}}$ arrival port, which distributes the power of the received signal uniformly across all members of $\mathcal{M}^{[\ell]}$. As a result, we define $\tau^{g}_{m\ell}(t)$ %{\color{red} multiple things: (1) what happened to the time index? (2) what is $g$ and why is it needed here? (3) why can't you just use $m$ and $\ell$ or something like that? prime is more confusing.} 
to indicate the amplitude and phase change between the $\ell^{\mathrm{th}}$ arrival port and the $m^{\mathrm{th}}$ departure port at time $t$, which is obtained as
\begin{align}
    \tau^g_{m\ell}(t)=\left\{ \begin{array}{ll} \frac{1}{\sqrt{\big|\mathcal{M}^{[\ell]}\big|}}\beta_{m\ell}(t)e^{j\theta_{m\ell}(t)}, & m\in \mathcal{M}^{[\ell]}, \\
0, & m\notin \mathcal{M}^{[\ell]},
\end{array} \right.
\end{align}
where $\beta_{m\ell}(t) \in[0,1]$, $\theta_{m\ell}(t) \in [0,2\pi)$, and $\frac{1}{\sqrt{\big|\mathcal{M}^{[\ell]}\big|}}$ is formed by the power splitter, which guarantees that $\sum_{m=1}^M |\tau^g_{m\ell}(t)|^2=1$ (i.e., there is no gain from power sharing at the $\ell^{\mathrm{th}}$ arrival port). Similar to the previous case, we assume $\beta_{m\ell}(t)=1$ %{\color{red} power constraint? this is why we need the problem formulation first before simulations. Once again, I am not sure I can trust the simulation results.} 
and exploit a $b$-bit PS to realize phase $\theta_{m\ell}(t)$.
Then, we use $\mathbf{T}^g(t) \in \mathbb{C}^{M \times M}$ to denote the general RIS configuration as follows.
\begin{align}
    \mathbf{T}^g(t)=\mathrm{blkdiag}\{\boldsymbol{\tau}^{g[1]}(t),\boldsymbol{\tau}^{g[2]}(t), \ldots, \boldsymbol{\tau}^{g[\frac{M}{cd}]}(t)\},
\end{align}
where
\begin{align}
    &\boldsymbol{\tau}^{g[u]}(t)= \\ \nonumber
    &\begin{bmatrix}
\tau^g_{[(u-1)cd+1][(u-1)cd+1]}(t) & \tau^g_{[(u-1)cd+1][(u-1)cd+2]}(t) & \ldots & \tau^g_{[(u-1)cd+1][ucd]}(t)\\
\vdots & \vdots & \ldots & \vdots
\\
\tau^g_{[ucd][(u-1)cd+1]}(t) & \tau^g_{[ucd][(u-1)cd+2]}(t) & \ldots & \tau^g_{[ucd][ucd]}(t)
\end{bmatrix}, & \quad 1\leq u \leq \frac{M}{cd}.
\end{align}

% \begin{align}
%     \mathbf{T}^g(t)=\begin{bmatrix}
% t_{11}(t) & t_{12}(t) & \ldots & t_{1M}(t)\\
% \vdots & \vdots & \ldots & \vdots
% \\
% t_{M1}(t) & t_{M2}(t) & \ldots & t_{MM}(t)
% \end{bmatrix}.
% \end{align}
In this case, if $s_{\ell}(t), 1\leq \ell \leq M$ is the incident signal, received by the $\ell^{\mathrm{th}}$ arrival port, at time $t$, according to Fig.~\ref{Fig:channel_model_new_RIS}(c), we obtain the reflected signal from the $m^{\mathrm{th}}$ departure port as
\begin{align}
    r_m(t)=\sum_{\ell=1}^Ms_{\ell}(t) \tau^g_{m\ell}(t), \quad 1\leq m \leq M. 
\end{align}

\textbf{Received signal:} The received signal at ${\sf Rx}_i$ is the reflected signal from the RIS, which is given by
\begin{align}
\label{eq:received_sig_a_RIS}
    y_i(t)=\sum_{j=1}^K \Big[\textbf{g}^{[i]}(t)\mathbf{T}(t)\textbf{h}^{[j]}(t)\Big]x_j(t)+n_i(t),
\end{align}
where $\mathbf{T}(t) \in \{\mathbf{T}^{st}(t), \mathbf{T}^g(t)\}$, $x_j(t)$ is the transmitted signal at ${\sf Tx}_j$, $n_i(t) \thicksim \mathcal{CN}(0,\sigma^2)$ is additive white Gaussian noise (AWGN) at ${\sf Rx}_i$, and $\mathbb{E}\{\textbf{x}(t)\textbf{x}^{H}(t)\}=\mathrm{diag}([P_1, P_2,\ldots,P_K])$ where $\textbf{x}(t)=[x_1(t),x_2(t),\ldots,$ $x_K(t)] \in \mathbb{C}^{1\times K}$ and $P_i, i\in \{1,2,\ldots K\}$ describes the transmit power from ${\sf Tx}_i$. As we describe later, all operations occur in a single coherence time; therefore, the time notation is removed throughout the rest of this work. Then, we use \eqref{eq:received_sig_a_RIS} and write the SINR at ${\sf Rx}_i$ as follows:
\begin{align}
\label{eq:SINR_update_a_RIS}
    \text{SINR}_i=\frac{P_i\Big|\textbf{g}^{[i]}\mathbf{T}\textbf{h}^{[i]}\Big|^2}{\sigma^2+\sum_{j=1, j\neq i}^{K }P_j\Big|\textbf{g}^{[i]}\mathbf{T}\textbf{h}^{[j]}\Big|^2}, \quad \mathbf{T} \in \{\mathbf{T}^{st}, \mathbf{T}^g\}.
\end{align} 



==> Sections/Sect2_Problem_setting_RIS_structure_USV_v1.tex <==
We examine a SISO maritime network consisting of $K$ pairs of distributed transmitters and receivers, as shown in Fig.~\ref{Fig:channel_model_standard_RIS}. Each transmitter aims to communicate with one receiver. Further, we incorporate a USV with an $M$-element RIS to assist the network. Finally, we propose G-RIS, a compact RIS structure, which fits limited-size USVs.

\subsection{Channel model}
We represent the channels between ${\sf Tx}_j$ and RIS and the channels between RIS and ${\sf Rx}_i$ at time $t$ as $\textbf{h}^{[j]}(t) \in \mathbb{C}^{M\times 1}$ and $\textbf{g}^{[i]}(t) \in \mathbb{C}^{1\times M}$, respectively, where $i,j \in \{1,2,\ldots,K\}$. The Rician fading distribution is used to model $\textbf{h}^{[j]}(t)$, and we express $h_m^{[j]}(t)$, the $m^{\mathrm{th}}$ element of $\textbf{h}^{[j]}(t)$, as follows:
\begin{align}
    \label{eq:Rician_fading}
    h_m^{[j]}(t)=\sqrt{\frac{1}{1+\kappa}}h_m^{[j],NLoS}(t)+\sqrt{\frac{\kappa}{1+\kappa}}h_m^{[j],LoS},
\end{align}
where $\kappa$ is Rician factor, $h_m^{[j],NLoS}(t) \thicksim \mathcal{CN}(0,C_0d_{1,j}^{-\alpha_1})$ represents the non-line-of-sight (NLoS) component of $h_m^{[j]}(t)$, and $h_m^{[j],LoS}=e^{-j\frac{2 \pi }{\lambda}d_{1,j}}$ shows the line-of-sight (LoS) part of $h_m^{[j]}(t)$, where $d_{1,j}$ denotes the distance between ${\sf Tx}_j$ and RIS, and $\alpha_1$ is the path loss exponent between them. The constant $C_0$ is used to capture the signal loss at a reference distance, such as $1m$. Additionally, we assume that $\textbf{g}^{[i]}(t)$ follows Rayleigh fading, where each element is modeled as a complex Gaussian distribution with zero mean and variance $C_0d_{2,i}^{-\alpha_2}$, where $d_{2,i}$ and $\alpha_2$ denote the distance and path loss exponent between RIS and ${\sf Rx}_i$, respectively.




We consider that the maritime network includes obstructions, such as islands, that block the direct path between transmitters and receivers. We also assume that $\textbf{h}^{[j]}(t)$ and $\textbf{g}^{[i]}(t)$ are independent over time and users due to the spacing of the RIS elements being at least $\lambda/2$ apart, where $\lambda$ is the wavelength of the transmitted signal. As in previous studies~\cite{fu2021reconfigurable,wu2019intelligent}, we assume that channel state information (CSI) is available globally and beyond that there is no data exchange between transmitters or receivers.
\begin{figure}[htb]
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=9, width=0.99\linewidth, draft=false]{images/system_model_USV_3.png}
  \vspace{-5mm}
  \caption{\it A SISO maritime network with an $M$-element RIS installed on a USV.%\avc{Remove the controller from the figure, it is weird that the RIS is controlled by the BS rather than a big host ship. Maybe add a UAV too. Watch: https://www.youtube.com/watch?v=P2tSwngihp0}
  }\label{Fig:channel_model_standard_RIS}
  %\vspace{-7mm}
\end{figure}

\begin{figure*}[ht]
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=9, width=0.99\linewidth, draft=false]{images/std_general_RIS_models.png}
  \vspace{-3mm}
  \caption{\it (a) A $32$-element S-RIS, where the $m^{\mathrm{th}}$ element uses a switch to either reflect or block its incident signal; (b) A G-RIS with $32$ elements, which is partitioned into $8$ cells where $c=d=2$; (c) The $m^{\mathrm{th}}$ arrival element uses $cd$ switches and a power splitter to share its incident signal; (d) The reflected signal from the $m^{\mathrm{th}}$ departure element includes a combination of the incident signals at all arrival elements.}\label{Fig:channel_model_new_RIS}
  %\vspace{-5mm}
\end{figure*}

{\color{blue}\textbf{CSI perfectness:} We assume that ${\sf Rx}_i$ estimates its incoming channels through ${\sf Tx}_j$-RIS-${\sf Rx}_i$ link with errors. Thus, we have:
\begin{align}
    &\hat{\textbf{h}}^{[j]}(t) = \textbf{h}^{[j]}(t) + \mathbf{e}^{[j]}_h(t),~~1 \leq j \leq K,\\ \nonumber
    &\hat{\textbf{g}}^{[i]}(t) = \textbf{g}^{[i]}(t) + \mathbf{e}^{[i]}_g(t),~~1 \leq i \leq K,
\end{align}
where $\mathbf{e}^{[j]}_h(t)\in \mathbb{C}^{M\times 1}$ and $\mathbf{e}^{[i]}_g(t)\in \mathbb{C}^{1\times M}$ are the estimation errors whose elements are distributed based on $\mathcal{CN}(0,1/p)$, and $p$ denotes the signal-to-noise-ratio (SNR) during the estimation process.}

\subsection{RIS structures}
In this section, we explain two structures of switch-based RIS. We assume that each RIS element has an arrival part that receives signals from transmitters and a departure part that reflects signals towards receivers. A controller is placed between a control unit, such as shore control center, and the RIS to facilitate the exchange of CSI and control RIS elements over a separate communication link.

\textbf{S-RIS:} In this RIS, there is no interconnection between the elements, and the $m^{\mathrm{th}}$ RIS element, $1 \leq m \leq M$, receives the incident signal and then uses its binary RF switch, $s_{m}(t)\in \{0,1\}$ that connects its arrival and departure parts, to either reflect or block its received signal at time $t$ as Fig.~\ref{Fig:channel_model_new_RIS}(a). Consequently, we define $\mathbf{T}^{s}(t)$ as the S-RIS configuration, which is given by:
\begin{align}
    \mathbf{T}^{s}(t)=\mathrm{diag}\left\{\boldsymbol{\tau}^{s}(t)\right\},
\end{align}
where
\begin{align}
    \boldsymbol{\tau}^{s}(t)=\left[s_{1}(t),s_{2}(t),\ldots,s_{M}(t)\right]^{\top}.
\end{align}

\textbf{G-RIS:} In this case, we partition RIS into $M/cd$ different cells{\footnote{Without loss of generality, we suppose $M$ is divisible by $cd.$}}, where $c$ and $d$ show the cell dimensions.(e.g., Fig.~\ref{Fig:channel_model_new_RIS}(b) shows a $32$-element G-RIS, which is partitioned into $8$ cells.) Next, we assume that each RIS element in a given cell can share its received signal with others in that cell as depicted in Fig.~\ref{Fig:channel_model_new_RIS}(c). Then, we use $\mathcal{M}^{[m]}$ to denote the cell that includes the $m^{\mathrm{th}}$ element, where
\begin{align}
    &\mathcal{M}^{[m]} = \\ \nonumber
    &\left\{ \begin{array}{ll} \big\{\lfloor \frac{m}{cd} \rfloor cd+1,\lfloor \frac{m}{cd} \rfloor cd+2,\ldots,\lfloor \frac{m}{cd} \rfloor cd+cd \big\}, & \lfloor \frac{m}{cd} \rfloor\neq \frac{m}{cd}, \\
\big\{m-cd+1,m-cd+2,\ldots,m \big\}, & \lfloor \frac{m}{cd} \rfloor = \frac{m}{cd}.
\end{array} \right.
\end{align}

Thereafter, the $m^{\mathrm{th}}$ element uses $cd$ binary RF switches to determine  $\bar{\mathcal{M}}^{[m]}\subseteq \mathcal{M}^{[m]}$, which contains the elements in the cell that obtain the signal received by the $m^{\mathrm{th}}$ arrival element. 
To share the power of the received signal, the $m^{\mathrm{th}}$ arrival elements utilizes a power splitter, which distributes the received power uniformly across all members of $\bar{\mathcal{M}}^{[m]}$. As a result, we define $\tau^{g}_{\ell m}(t)$ to indicate how the $m^{\mathrm{th}}$ arrival element is connected to the $\ell^{\mathrm{th}}$ departure element at time $t$, which is obtained as:
\begin{align}
    \tau^g_{\ell m}(t)=\left\{ \begin{array}{ll} \frac{1}{\sqrt{\big|\bar{\mathcal{M}}^{[m]}\big|}}s_{\ell m}(t), & \ell\in \bar{\mathcal{M}}^{[m]}, \\
0, & \ell\notin \bar{\mathcal{M}}^{[m]},
\end{array} \right.
\end{align}
where $\frac{1}{\sqrt{\big|\bar{\mathcal{M}}^{[m]}\big|}}$ is formed by the power splitter, which guarantees that $\sum_{\ell=1}^M |\tau^g_{\ell m}(t)|^2=1$ (i.e., there is no gain from power sharing at the $m^{\mathrm{th}}$ arrival element) and $s_{\ell m}(t)$ is a binary switch between the $m^{\mathrm{th}}$ arrival element and the $\ell^{\mathrm{th}}$ departure element. Then, we use $\mathbf{T}^g(t) \in \mathbb{C}^{M \times M}$ to denote the G-RIS configuration as below:
\begin{align}
    \mathbf{T}^g(t)=\mathrm{blkdiag}\left\{\boldsymbol{\tau}^{g[1]}(t),\boldsymbol{\tau}^{g[2]}(t), \ldots, \boldsymbol{\tau}^{g[\frac{M}{cd}]}(t)\right\},
\end{align}
where $\boldsymbol{\tau}^{g[u]}(t)$ follows \eqref{eq:tau_general_vector} on top of the next page.

Finally, based on Fig.~\ref{Fig:channel_model_new_RIS}(d), the $m^{\mathrm{th}}$ departure element collects the received signals at all elements in $\mathcal{M}^{[m]}$ and then reflects a combination of them toward the receivers.

\textbf{Received signal:} The received signal at ${\sf Rx}_i$ is the reflected signal from the RIS, which is given by:
\begin{align}
\label{eq:received_sig_a_RIS}
    y_i(t)=\sum_{j=1}^K \Big[\textbf{g}^{[i]}(t)\mathbf{T}(t)\textbf{h}^{[j]}(t)\Big]x_j(t)+n_i(t),
\end{align}
where $\mathbf{T}(t) \in \{\mathbf{T}^{s}(t), \mathbf{T}^g(t)\}$, $x_j(t)$ represents the transmitted signal at ${\sf Tx}_j$, and $n_i(t) \thicksim \mathcal{CN}(0,\sigma^2)$ denotes noise at ${\sf Rx}_i$. Here, $\mathbb{E}\left\{\textbf{x}(t)\textbf{x}^{H}(t)\right\}=\mathrm{diag}([P_1, P_2,\ldots,P_K])$, where $\textbf{x}(t)=[x_1(t),x_2(t),\ldots,x_K(t)] \in \mathbb{C}^{1\times K}$, and $P_i, i\in \{1,2,\ldots K\}$ denotes the transmit power from ${\sf Tx}_i$. We note that all operations occur within a single coherence time, and therefore the time notation is omitted throughout the rest of this work. Then, we use \eqref{eq:received_sig_a_RIS} to express the signal-to-interference-plus-noise ratio (SINR) at ${\sf Rx}_i$ as follows:
\begin{align}
\label{eq:SINR_update_a_RIS}
    \text{SINR}_i=\frac{P_i\Big|\textbf{g}^{[i]}\mathbf{T}\textbf{h}^{[i]}\Big|^2}{\sigma^2+\sum_{j=1, j\neq i}^{K }P_j\Big|\textbf{g}^{[i]}\mathbf{T}\textbf{h}^{[j]}\Big|^2}, \quad \mathbf{T} \in \{\mathbf{T}^{s}, \mathbf{T}^g\}.
\end{align} 
\begin{figure*}
\begin{align}
\label{eq:tau_general_vector}
    \boldsymbol{\tau}^{g[u]}(t)= \begin{bmatrix}
\tau^g_{[(u-1)cd+1][(u-1)cd+1]}(t) & \tau^g_{[(u-1)cd+1][(u-1)cd+2]}(t) & \ldots & \tau^g_{[(u-1)cd+1][ucd]}(t)\\
\vdots & \vdots & \ldots & \vdots
\\
\tau^g_{[ucd][(u-1)cd+1]}(t) & \tau^g_{[ucd][(u-1)cd+2]}(t) & \ldots & \tau^g_{[ucd][ucd]}(t)
\end{bmatrix}, & \quad 1\leq u \leq \frac{M}{cd}.
\end{align}
\hrule
\end{figure*}


==> Sections/Sect2_Problem_setting_RIS_structure_v1.tex <==
In this paper, we examine an RIS-assisted network with distributed transmitter-receiver pairs where each transmitter aims to communicate with only one desired receiver, as shown in Fig.~\ref{Fig:channel_model_standard_RIS}. Further, we focus on a SISO scenario to highlight the pure RIS gain in the network.

\subsection{Channel model} We represent the channels between ${\sf Tx}_j$ and RIS and the channels between RIS and ${\sf Rx}_{k}$ at time $t$ as $\textbf{h}^{[j]}(t) \in \mathbb{C}^{M\times 1}$ and $\textbf{g}^{[k]}(t) \in \mathbb{C}^{1\times M}$, respectively, where $j,k \in \{1,2,\ldots,K\}$, $K$ is the number of transmitter-receiver pairs, and $M$ denotes the number of RIS elements. We use Rician fading to model $\textbf{h}^{[j]}(t)$ and express $h_m^{[j]}(t)$, the $m^{\mathrm{th}}$ element of $\textbf{h}^{[j]}(t), 1 \leq m \leq M$, as follows:
\begin{align}
    \label{eq:Rician_fading}
    h_m^{[j]}(t)=\sqrt{\frac{1}{1+\kappa}}h_m^{[j],NLoS}(t)+\sqrt{\frac{\kappa}{1+\kappa}}h_m^{[j],LoS},
\end{align}
where $\kappa$ is the Rician factor, $h_m^{[j],NLoS}(t) \thicksim \mathcal{CN}(0,C_0d_{1,j}^{-\alpha_1})$ represents the non-line-of-sight (NLoS) component of $h_m^{[j]}(t)$, and $h_m^{[j],LoS}=\sqrt{C_0d_{1,j}^{-\alpha_1}}e^{-j\frac{2 \pi }{\lambda}d_{1,j}}$ shows the line-of-sight (LoS) part of $h_m^{[j]}(t)$, where $d_{1,j}$ denotes the distance between ${\sf Tx}_j$ and RIS, $\alpha_1$ is the path loss exponent between them, and $\lambda$ is the wavelength of the transmitted signal. We use $C_0$ to capture the signal loss at a reference distance, e.g., $1\mathrm{m}$. Here, $\textbf{g}^{[k]}(t)$ follows Rayleigh fading whose elements are modeled as a complex Gaussian distribution with zero mean and variance $C_0d_{2,k}^{-\alpha_2}$, where $d_{2,k}$ and $\alpha_2$ denote the distance and path loss exponent between RIS and ${\sf Rx}_k$, respectively. 

We assume that the direct path between transmitters and receivers is blocked. We also suppose that the channels are independent due to the spacing of the RIS elements being at least $\lambda/2$ apart. Similar to~\cite{fu2021reconfigurable,wu2019intelligent}, we assume that channel state information (CSI) is available globally, and beyond that, there is no data exchange between transmitters or receivers. We note that all operations occur within a single coherence time; hence, we omit the time notation in the rest of this paper.

\begin{comment}
\textbf{CSI resolution:} In this work, we assume that each receiver estimates its incoming channels from all transmitters using the pilot signals and then informs the others, while the estimated CSI is different from the actual CSI due to different reasons such as noise, hardware impairments, and unfavorable environments. Thus, we have: 
\begin{align}
    &\hat{\textbf{h}}^{[j]}(t) = \textbf{h}^{[j]}(t) + \mathbf{e}^{[j]}_h(t),~~1 \leq j \leq K,\\ \nonumber
    &\hat{\textbf{g}}^{[k]}(t) = \textbf{g}^{[k]}(t) + \mathbf{e}^{[k]}_g(t),~~1 \leq k \leq K,
\end{align}
where $\mathbf{e}^{[j]}_h(t)\in \mathbb{C}^{M\times 1}$ and $\mathbf{e}^{[k]}_g(t)\in \mathbb{C}^{1\times M}$ are the estimation errors whose elements are distributed based on $\mathcal{CN}(0,1/p)$, and $p$ denotes the signal-to-noise ratio (SNR) during the estimation process.
\end{comment}

\begin{figure}[ht]
%\vspace{-3mm}
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=7, width=0.75\linewidth, draft=false]{images/channel_model_IRIS.png}
  \vspace{-3mm}
  \caption{A SISO network with an RIS assisting multi-user communications.%\avc{Remove the controller from the figure, it is weird that the RIS is controlled by the BS rather than a big host ship. Maybe add a UAV too. Watch: https://www.youtube.com/watch?v=P2tSwngihp0}
}\label{Fig:channel_model_standard_RIS}
  \vspace{-5mm}
\end{figure}

\begin{figure*}[ht]
%\vspace{-3mm}
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=4, width=0.85\linewidth, draft=false]{images/std_general_RIS_models_5.png}
  \vspace{-3mm}
  \caption{(a) A $32$-element S-RIS, where the $m^{\mathrm{th}}$ RIS element uses an RF switch to either reflect or block its incident signal; (b) An I-RIS with $32$ elements and eight cells of size $(2,2)$; (c) The $m^{\mathrm{th}}$ arrival element uses $cd$ RF switches and a power splitter to share its incident signal; (d) The reflected signal from the $m^{\mathrm{th}}$ departure element includes a combination of the incident signals at all arrival elements.}\label{Fig:channel_model_new_RIS}
  \vspace{-2mm}
\end{figure*}
%\vspace{10mm}
\subsection{Existing vs. the proposed RIS design}
In this subsection, we delve into the details of two RIS structures using RF switches. Here, each RIS element has an arrival part that receives the incident signals from transmitters and a departure part that reflects the signals toward receivers.% We place a controller between a control unit, e.g., a shore control center, and the RIS to exchange CSI and control RIS elements over a separate communication link.

\textbf{S-RIS:} In this RIS, there is no interconnection between the elements. The $m^{\mathrm{th}}$ RIS element, $1 \leq m \leq M$, receives the incident signal and then uses its binary RF switch, $s_{m}\in \{0,1\}$ between its arrival and departure parts, to either reflect or block its incident signal as shown in Fig.~\ref{Fig:channel_model_new_RIS}(a). We define $\mathbf{T}^{\mathrm{s}}$ as the S-RIS configuration, which is given by:
\begin{align}
\mathbf{T}^{\mathrm{s}}=\mathrm{diag}\left\{\boldsymbol{\tau}^{\mathrm{s}}\right\},~~~\boldsymbol{\tau}^{\mathrm{s}}=\left[s_{1},s_{2},\ldots,s_{M}\right]^{\top}.
\end{align}

\textbf{I-RIS:} Here, we first divide RIS into $M/(c \times d)$ different cells, where $c$ and $d$ represent the cell size. (e.g., Fig.~\ref{Fig:channel_model_new_RIS}(b) shows a $32$-element I-RIS with eight cells of size $(2, 2)$.) Without loss of generality, we suppose $M$ is divisible by $c \times d$. In the rest of this work, we use $cd$ to denote $c \times d$. Next, each element within a given cell shares its incident signal with its neighbors in that cell, as depicted in Fig.~\ref{Fig:channel_model_new_RIS}(c). We define $\mathcal{M}^{[m]}$ as a cell that includes the $m^{\mathrm{th}}$ element. Then, the $m^{\mathrm{th}}$ RIS element uses $cd$ binary RF switches to determine  $\bar{\mathcal{M}}^{[m]}\subseteq \mathcal{M}^{[m]}$, which contains the active elements in the cell obtaining the incident signal received by the $m^{\mathrm{th}}$ arrival element. The $m^{\mathrm{th}}$ arrival element uses a power splitter to distribute the incident signal power uniformly across all members of $\bar{\mathcal{M}}^{[m]}$. Then, to indicate how the $m^{\mathrm{th}}$ arrival element connects to the $\ell^{\mathrm{th}}$ departure element, $1\leq \ell,M\leq M$, we define $\tau_{\ell, m}$ as:
% $\tau_{\ell, m}=\left(1/\sqrt{\left|\bar{\mathcal{M}}^{[m]}\right|}\right)s_{\ell, m}$ when $\ell\in \mathcal{M}^{[m]}$; conversely, $\tau_{\ell, m}=0$ if $\ell\notin \mathcal{M}^{[m]}$.
\begin{align}
\tau_{\ell, m}=\left\{ \begin{array}{ll} \left(1/\sqrt{\left|\bar{\mathcal{M}}^{[m]}\right|}\right)s_{\ell, m}, & \ell\in \mathcal{M}^{[m]}, \\
0, & \ell\notin \mathcal{M}^{[m]},
\end{array} \right.
\end{align}
where $s_{\ell, m}\in \{0,1\}$ is a binary RF switch between the $m^{\mathrm{th}}$ arrival element and the $\ell^{\mathrm{th}}$ departure element, and $1/\sqrt{\left|\bar{\mathcal{M}}^{[m]}\right|}$ guarantees $\sum_{\ell=1}^M |\tau_{\ell, m}|^2\leq1$, where the inequality holds true only if all switches from the $m^{\mathrm{th}}$ arrival element to its neighbors are zero. In this case $\sum_{\ell=1}^M |\tau_{\ell, m}|^2 =0 <1$. %, i.e., RIS elements are passive. We note that I-RIS is nearly-passive as it requires control signals to activate or deactivate its RF switches. %\avc{1. ``.'' then i.e., does not work, 2. the sentence after i.e. is not well written, it simply means sharing is useless, you want to say the I-RIS elements are passive} (i.e., there is no gain from power sharing at the $m^{\mathrm{th}}$ arrival element.)
Then, we use $\mathbf{T}^{\mathrm{i}}$ to denote the I-RIS configuration as:
\begin{align}
    \mathbf{T}^{\mathrm{i}}=\mathrm{blkdiag}\left\{\boldsymbol{\tau}^{\mathrm{i}[1]},\boldsymbol{\tau}^{\mathrm{i}[2]}, \ldots, \boldsymbol{\tau}^{\mathrm{i}[\frac{M}{cd}]}\right\},
\end{align}
where $\boldsymbol{\tau}^{\mathrm{i}[u]}, 1\leq u \leq \frac{M}{cd}$ follows \eqref{eq:tau_general_vector}.
\begin{figure*}
\begin{align}
\label{eq:tau_general_vector}
    \boldsymbol{\tau}^{\mathrm{i}[u]} = \begin{bmatrix}
\tau^{\mathrm{i}[u]}_{1,1} & \tau^{\mathrm{i}[u]}_{1,2} & \ldots & \tau^{\mathrm{i}[u]}_{1,cd}\\
\vdots & \vdots & \ldots & \vdots
\\
\tau^{\mathrm{i}[u]}_{cd,1} & \tau^{\mathrm{i}[u]}_{cd,2} & \ldots & \tau^{\mathrm{i}[u]}_{cd, cd}
\end{bmatrix} = \begin{bmatrix}
\tau_{(u-1)cd+1,(u-1)cd+1} & \tau_{(u-1)cd+1,(u-1)cd+2} & \ldots & \tau_{(u-1)cd+1,ucd}\\
\vdots & \vdots & \ldots & \vdots
\\
\tau_{ucd,(u-1)cd+1} & \tau_{ucd,(u-1)cd+2} & \ldots & \tau_{ucd,ucd}
\end{bmatrix}.
\end{align}
\hrule
\end{figure*}
We consider $\boldsymbol{\tau}^{\mathrm{i}[u]}=\hat{\boldsymbol{\tau}}^{\mathrm{i}[u]}+\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}$. For each $\tau^{\mathrm{i}[u]}_{u_1,u_2}, 1 \leq u_1, u_2 \leq cd$, if it is the only non-zero element in the $u_1^{\mathrm{th}}$ row and $u_2^{\mathrm{th}}$ column of $\boldsymbol{\tau}^{\mathrm{i}[u]}$, we include $\tau^{\mathrm{i}[u]}_{u_1,u_2}$ in $\hat{\boldsymbol{\tau}}^{\mathrm{i}[u]}$ by following~\eqref{eq:hat_tau}; otherwise, we save $\tau^{\mathrm{i}[u]}_{u_1,u_2}$ in $\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}$ as~\eqref{eq:tilde_tau}. We show \eqref{eq:tau_general_vector},~\eqref{eq:hat_tau}, and~\eqref{eq:tilde_tau} at the top of the next page.  
\begin{figure*}
\begin{minipage}[t]{0.50\linewidth}
\begin{equation}
\label{eq:hat_tau}
\hat{\tau}^{\mathrm{i}[u]}_{u_1,u_2}=\left\{ \begin{array}{ll} \tau^{\mathrm{i}[u]}_{u_1,u_2}, & \sum_{q=1}^{cd}\left(\tau^{\mathrm{i}[u]}_{u_1,q} + \tau^{\mathrm{i}[u]}_{q,u_2} \right) = 2\tau^{\mathrm{i}[u]}_{u_1,u_2}, \\
0, & \text{otherwise},
\end{array} \right.
\end{equation}
\end{minipage}
 % Adjust the spacing between equations
\begin{minipage}[t]{0.50\linewidth}
\begin{equation}
\label{eq:tilde_tau}
\tilde{\tau}^{\mathrm{i}[u]}_{u_1,u_2}=\left\{ \begin{array}{ll} \tau^{\mathrm{i}[u]}_{u_1,u_2}, & \sum_{q=1}^{cd}\left(\tau^{\mathrm{i}[u]}_{u_1,q} + \tau^{\mathrm{i}[u]}_{q,u_2}\right) \neq 2\tau^{\mathrm{i}[u]}_{u_1,u_2}, \\
0, & \text{otherwise},
\end{array} \right.
\end{equation}
\end{minipage}
\hrule
\end{figure*}Then, based on Fig.~\ref{Fig:channel_model_new_RIS}(d), to ensure I-RIS is passive, we normalize $\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}$, i.e., replace $\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}$ with $\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}/||\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}||_{\mathrm{F}}$. Finally, the $m^{\mathrm{th}}$ departure element mixes the incident signals of all elements in $\mathcal{M}^{[m]}$ and reflects a combination of them toward the receivers.

\textbf{Received signal:} ${\sf Rx}_{k}, 1\leq k \leq K,$ receives the reflected signals from the RIS, which is given by:
\begin{align}
\label{eq_ch5:received_sig_a_RIS}
    y_{k}=\sum_{j=1}^K \Big[\textbf{g}^{[k]}\mathbf{T}\textbf{h}^{[j]}\Big]x_j+n_{k},
\end{align}
where $\mathbf{T} \in \left\{\mathbf{T}^{\mathrm{s}}, \mathbf{T}^{\mathrm{i}}\right\}$, $x_j$ is the transmitted signal from ${\sf Tx}_j$, and $n_{k} \thicksim \mathcal{CN}(0,\sigma^2)$ denotes noise at ${\sf Rx}_{k}$. Here, $\mathbb{E}\left\{\textbf{x}\textbf{x}^{H}\right\}=\mathrm{diag}([P_1, P_2,\ldots,P_K])$, where $\textbf{x}=[x_1,x_2,\ldots,x_K] \in \mathbb{C}^{1\times K}$, and $P_j$ is the transmit power from ${\sf Tx}_j$.  Then, we use \eqref{eq_ch5:received_sig_a_RIS} to express the signal-to-interference-plus-noise ratio (SINR) at ${\sf Rx}_{k}$ as follows:
\begin{align}
\label{eq_ch5:SINR_update_a_RIS}
    \text{SINR}_{k}=\frac{P_{k}\Big|\textbf{g}^{[k]}\mathbf{T}\textbf{h}^{[k]}\Big|^2}{\sigma^2+\sum_{j=1, j\neq k}^{K }P_j\Big|\textbf{g}^{[k]}\mathbf{T}\textbf{h}^{[j]}\Big|^2}.
\end{align} 


==> Sections/Sect2_Problem_setting_RIS_structure_v2.tex <==
In this paper, we examine an RIS-assisted network with distributed transmitter-receiver pairs where each transmitter aims to communicate with only one desired receiver, as shown in Fig.~\ref{Fig:channel_model_standard_RIS}. Further, we focus on a SISO scenario to highlight the pure RIS gain in the network.

\subsection{Channel model} We represent the channels between ${\sf Tx}_j$ and RIS and the channels between RIS and ${\sf Rx}_{k}$ at time $t$ as $\textbf{h}^{[j]}(t) \in \mathbb{C}^{M\times 1}$ and $\textbf{g}^{[k]}(t) \in \mathbb{C}^{1\times M}$, respectively, where $j,k \in \{1,2,\ldots,K\}$, $K$ is the number of transmitter-receiver pairs, and $M$ denotes the number of RIS elements. We use Rician fading to model $\textbf{h}^{[j]}(t)$ and express $h_m^{[j]}(t)$, the $m^{\mathrm{th}}$ element of $\textbf{h}^{[j]}(t), 1 \leq m \leq M$, as follows:
\begin{align}
    \label{eq:Rician_fading}
    h_m^{[j]}(t)=\sqrt{\frac{1}{1+\kappa}}h_m^{[j],NLoS}(t)+\sqrt{\frac{\kappa}{1+\kappa}}h_m^{[j],LoS},
\end{align}
where $\kappa$ is the Rician factor, $h_m^{[j],NLoS}(t) \thicksim \mathcal{CN}(0,C_0d_{1,j}^{-\alpha_1})$ represents the non-line-of-sight (NLoS) component of $h_m^{[j]}(t)$, and $h_m^{[j],LoS}=\sqrt{C_0d_{1,j}^{-\alpha_1}}e^{-j\frac{2 \pi }{\lambda}d_{1,j}}$ shows the line-of-sight (LoS) part of $h_m^{[j]}(t)$, where $d_{1,j}$ denotes the distance between ${\sf Tx}_j$ and RIS, $\alpha_1$ is the path loss exponent between them, and $\lambda$ is the wavelength of the transmitted signal. We use $C_0$ to capture the signal loss at a reference distance, e.g., $1\mathrm{m}$. Here, $\textbf{g}^{[k]}(t)$ follows Rayleigh fading whose elements are modeled as a complex Gaussian distribution with zero mean and variance $C_0d_{2,k}^{-\alpha_2}$, where $d_{2,k}$ and $\alpha_2$ denote the distance and path loss exponent between RIS and ${\sf Rx}_k$, respectively. 

We assume that the direct path between transmitters and receivers is blocked. We also suppose that the channels are independent due to the spacing of the RIS elements being at least $\lambda/2$ apart. Similar to~\cite{fu2021reconfigurable,wu2019intelligent}, we assume that channel state information (CSI) is available globally, and beyond that, there is no data exchange between transmitters or receivers. We note that all operations occur within a single coherence time; hence, we omit the time notation in the rest of this paper.

\begin{comment}
\textbf{CSI resolution:} In this work, we assume that each receiver estimates its incoming channels from all transmitters using the pilot signals and then informs the others, while the estimated CSI is different from the actual CSI due to different reasons such as noise, hardware impairments, and unfavorable environments. Thus, we have: 
\begin{align}
    &\hat{\textbf{h}}^{[j]}(t) = \textbf{h}^{[j]}(t) + \mathbf{e}^{[j]}_h(t),~~1 \leq j \leq K,\\ \nonumber
    &\hat{\textbf{g}}^{[k]}(t) = \textbf{g}^{[k]}(t) + \mathbf{e}^{[k]}_g(t),~~1 \leq k \leq K,
\end{align}
where $\mathbf{e}^{[j]}_h(t)\in \mathbb{C}^{M\times 1}$ and $\mathbf{e}^{[k]}_g(t)\in \mathbb{C}^{1\times M}$ are the estimation errors whose elements are distributed based on $\mathcal{CN}(0,1/p)$, and $p$ denotes the signal-to-noise ratio (SNR) during the estimation process.
\end{comment}

\begin{figure}[ht]
\vspace{-3mm}
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=7, width=0.82\linewidth, draft=false]{images/channel_model_IRIS.png}
  \vspace{-4mm}
  \caption{A SISO network with an RIS assisting multi-user communications.%\avc{Remove the controller from the figure, it is weird that the RIS is controlled by the BS rather than a big host ship. Maybe add a UAV too. Watch: https://www.youtube.com/watch?v=P2tSwngihp0}
}\label{Fig:channel_model_standard_RIS}
  \vspace{-2mm}
\end{figure}

\begin{figure*}[ht]
%\vspace{-3mm}
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=4, width=0.9\linewidth, draft=false]{images/std_general_RIS_models_5.png}
  \vspace{-4mm}
  \caption{(a) A $32$-element S-RIS, where the $m^{\mathrm{th}}$ RIS element uses an RF switch to either reflect or block its incident signal; (b) An I-RIS with $32$ elements and eight cells of size $(2,2)$; (c) The $m^{\mathrm{th}}$ arrival element uses $cd$ RF switches and a power splitter to share its incident signal; (d) The reflected signal from the $m^{\mathrm{th}}$ departure element includes a combination of the incident signals at all arrival elements.}\label{Fig:channel_model_new_RIS}
  \vspace{-2mm}
\end{figure*}
%\vspace{10mm}
\subsection{Existing vs. the proposed RIS design}
In this subsection, we delve into the details of two RIS structures using RF switches. Here, each RIS element has an arrival part that receives the incident signals from transmitters and a departure part that reflects the signals toward receivers.% We place a controller between a control unit, e.g., a shore control center, and the RIS to exchange CSI and control RIS elements over a separate communication link.

\textbf{S-RIS:} In this RIS, there is no interconnection between the elements. The $m^{\mathrm{th}}$ RIS element, $1 \leq m \leq M$, receives the incident signal and then uses its binary RF switch, $s_{m}\in \{0,1\}$ between its arrival and departure parts, to either reflect or block its incident signal as shown in Fig.~\ref{Fig:channel_model_new_RIS}(a). We define $\mathbf{T}^{\mathrm{s}}$ as the S-RIS configuration, which is given by:
\begin{align}
\mathbf{T}^{\mathrm{s}}=\mathrm{diag}\left\{\boldsymbol{\tau}^{\mathrm{s}}\right\},~~~\boldsymbol{\tau}^{\mathrm{s}}=\left[s_{1},s_{2},\ldots,s_{M}\right]^{\top}.
\end{align}

\textbf{I-RIS:} Here, we first divide RIS into $M/(c \times d)$ different cells, where $c$ and $d$ represent the cell size. (e.g., Fig.~\ref{Fig:channel_model_new_RIS}(b) shows a $32$-element I-RIS with eight cells of size $(2, 2)$.) Without loss of generality, we suppose $M$ is divisible by $c \times d$. In the rest of this work, we use $cd$ to denote $c \times d$. Next, each element within a given cell shares its incident signal with its neighbors in that cell, as depicted in Fig.~\ref{Fig:channel_model_new_RIS}(c). We define $\mathcal{M}^{[m]}$ as a cell that includes the $m^{\mathrm{th}}$ element. Then, the $m^{\mathrm{th}}$ RIS element uses $cd$ binary RF switches to determine  $\bar{\mathcal{M}}^{[m]}\subseteq \mathcal{M}^{[m]}$, which contains the active elements in the cell obtaining the incident signal received by the $m^{\mathrm{th}}$ arrival element. The $m^{\mathrm{th}}$ arrival element uses a power splitter to distribute the incident signal power uniformly across all members of $\bar{\mathcal{M}}^{[m]}$. Then, to indicate how the $m^{\mathrm{th}}$ arrival element connects to the $\ell^{\mathrm{th}}$ departure element, $1\leq \ell,m\leq M$, we define $\tau_{\ell, m}$ as:
$\tau_{\ell, m}=\left(1/\sqrt{\left|\bar{\mathcal{M}}^{[m]}\right|}\right)s_{\ell, m}$ when $\ell\in \mathcal{M}^{[m]}$; conversely, $\tau_{\ell, m}=0$ if $\ell\notin \mathcal{M}^{[m]}$.
% \begin{align}
% \tau_{\ell, m}=\left\{ \begin{array}{ll} \left(1/\sqrt{\left|\bar{\mathcal{M}}^{[m]}\right|}\right)s_{\ell, m}, & \ell\in \mathcal{M}^{[m]}, \\
% 0, & \ell\notin \mathcal{M}^{[m]},
% \end{array} \right.
% \end{align}
Here, $s_{\ell, m}\in \{0,1\}$ is a binary RF switch between the $m^{\mathrm{th}}$ arrival element and the $\ell^{\mathrm{th}}$ departure element, and $1/\sqrt{\left|\bar{\mathcal{M}}^{[m]}\right|}$ guarantees $\sum_{\ell=1}^M |\tau_{\ell, m}|^2\leq1$, where the inequality holds true only if all switches from the $m^{\mathrm{th}}$ arrival element to its neighbors are zero. In this case $\sum_{\ell=1}^M |\tau_{\ell, m}|^2 =0 <1$. %, i.e., RIS elements are passive. We note that I-RIS is nearly-passive as it requires control signals to activate or deactivate its RF switches. %\avc{1. ``.'' then i.e., does not work, 2. the sentence after i.e. is not well written, it simply means sharing is useless, you want to say the I-RIS elements are passive} (i.e., there is no gain from power sharing at the $m^{\mathrm{th}}$ arrival element.)
Then, we use $\mathbf{T}^{\mathrm{i}}$ to denote the I-RIS configuration as:
\begin{align}
    \mathbf{T}^{\mathrm{i}}=\mathrm{blkdiag}\left\{\boldsymbol{\tau}^{\mathrm{i}[1]},\boldsymbol{\tau}^{\mathrm{i}[2]}, \ldots, \boldsymbol{\tau}^{\mathrm{i}[\frac{M}{cd}]}\right\},
\end{align}
where $\boldsymbol{\tau}^{\mathrm{i}[u]}, 1\leq u \leq \frac{M}{cd}$ follows \eqref{eq:tau_general_vector}.
\begin{figure*}
\begin{align}
\label{eq:tau_general_vector}
    \boldsymbol{\tau}^{\mathrm{i}[u]} = \begin{bmatrix}
\tau^{\mathrm{i}[u]}_{1,1} & \tau^{\mathrm{i}[u]}_{1,2} & \ldots & \tau^{\mathrm{i}[u]}_{1,cd}\\
\vdots & \vdots & \ldots & \vdots
\\
\tau^{\mathrm{i}[u]}_{cd,1} & \tau^{\mathrm{i}[u]}_{cd,2} & \ldots & \tau^{\mathrm{i}[u]}_{cd, cd}
\end{bmatrix} = \begin{bmatrix}
\tau_{(u-1)cd+1,(u-1)cd+1} & \tau_{(u-1)cd+1,(u-1)cd+2} & \ldots & \tau_{(u-1)cd+1,ucd}\\
\vdots & \vdots & \ldots & \vdots
\\
\tau_{ucd,(u-1)cd+1} & \tau_{ucd,(u-1)cd+2} & \ldots & \tau_{ucd,ucd}
\end{bmatrix}.
\end{align}
\hrule
\end{figure*}
We consider $\boldsymbol{\tau}^{\mathrm{i}[u]}=\hat{\boldsymbol{\tau}}^{\mathrm{i}[u]}+\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}$. For each $\tau^{\mathrm{i}[u]}_{u_1,u_2}, 1 \leq u_1, u_2 \leq cd$, if it is the only non-zero element in the $u_1^{\mathrm{th}}$ row and $u_2^{\mathrm{th}}$ column of $\boldsymbol{\tau}^{\mathrm{i}[u]}$, we include $\tau^{\mathrm{i}[u]}_{u_1,u_2}$ in $\hat{\boldsymbol{\tau}}^{\mathrm{i}[u]}$ by following~\eqref{eq:hat_tau}; otherwise, we save $\tau^{\mathrm{i}[u]}_{u_1,u_2}$ in $\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}$ as~\eqref{eq:tilde_tau}. We show \eqref{eq:tau_general_vector},~\eqref{eq:hat_tau}, and~\eqref{eq:tilde_tau} at the top of the next page.  
\begin{figure*}
\begin{minipage}[t]{0.50\linewidth}
\begin{equation}
\label{eq:hat_tau}
\hat{\tau}^{\mathrm{i}[u]}_{u_1,u_2}=\left\{ \begin{array}{ll} \tau^{\mathrm{i}[u]}_{u_1,u_2}, & \sum_{q=1}^{cd}\left(\tau^{\mathrm{i}[u]}_{u_1,q} + \tau^{\mathrm{i}[u]}_{q,u_2} \right) = 2\tau^{\mathrm{i}[u]}_{u_1,u_2}, \\
0, & \text{otherwise},
\end{array} \right.
\end{equation}
\end{minipage}
 % Adjust the spacing between equations
\begin{minipage}[t]{0.50\linewidth}
\begin{equation}
\label{eq:tilde_tau}
\tilde{\tau}^{\mathrm{i}[u]}_{u_1,u_2}=\left\{ \begin{array}{ll} \tau^{\mathrm{i}[u]}_{u_1,u_2}, & \sum_{q=1}^{cd}\left(\tau^{\mathrm{i}[u]}_{u_1,q} + \tau^{\mathrm{i}[u]}_{q,u_2}\right) \neq 2\tau^{\mathrm{i}[u]}_{u_1,u_2}, \\
0, & \text{otherwise},
\end{array} \right.
\end{equation}
\end{minipage}
\hrule
\end{figure*}Then, based on Fig.~\ref{Fig:channel_model_new_RIS}(d), to ensure I-RIS is passive, we normalize $\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}$, i.e., replace $\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}$ with $\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}/||\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}||_{\mathrm{F}}$. Finally, the $m^{\mathrm{th}}$ departure element mixes the incident signals of all elements in $\mathcal{M}^{[m]}$ and reflects a combination of them toward the receivers.

\textbf{Received signal:} ${\sf Rx}_{k}, 1\leq k \leq K,$ receives the reflected signals from the RIS, which is given by:
\begin{align}
\label{eq_ch5:received_sig_a_RIS}
    y_{k}=\sum_{j=1}^K \Big[\textbf{g}^{[k]}\mathbf{T}\textbf{h}^{[j]}\Big]x_j+n_{k},
\end{align}
where $\mathbf{T} \in \left\{\mathbf{T}^{\mathrm{s}}, \mathbf{T}^{\mathrm{i}}\right\}$, $x_j$ is the transmitted signal from ${\sf Tx}_j$, and $n_{k} \thicksim \mathcal{CN}(0,\sigma^2)$ denotes noise at ${\sf Rx}_{k}$. Here, $\mathbb{E}\left\{\textbf{x}^{H}\textbf{x}\right\}=\mathrm{diag}([P_1, P_2,\ldots,P_K])$, where $\textbf{x}=[x_1,x_2,\ldots,x_K] \in \mathbb{C}^{1\times K}$, and $P_j$ is the transmit power from ${\sf Tx}_j$.  Then, we use \eqref{eq_ch5:received_sig_a_RIS} to express the signal-to-interference-plus-noise ratio (SINR) at ${\sf Rx}_{k}$ as follows:
\begin{align}
\label{eq_ch5:SINR_update_a_RIS}
    \text{SINR}_{k}=\frac{P_{k}\Big|\textbf{g}^{[k]}\mathbf{T}\textbf{h}^{[k]}\Big|^2}{\sigma^2+\sum_{j=1, j\neq k}^{K }P_j\Big|\textbf{g}^{[k]}\mathbf{T}\textbf{h}^{[j]}\Big|^2}.
\end{align} 


==> Sections/Sect2_Problem_setting_RIS_structure_v2_two_authors.tex <==
In this paper, we examine an RIS-assisted network with distributed transmitter-receiver pairs where each transmitter aims to communicate with only one desired receiver, as shown in Fig.~\ref{Fig:channel_model_standard_RIS}. Further, we focus on a SISO scenario to highlight the pure RIS gain in the network.

\subsection{Channel model} We represent the channels between ${\sf Tx}_j$ and RIS and the channels between RIS and ${\sf Rx}_{k}$ at time $t$ as $\textbf{h}^{[j]}(t) \in \mathbb{C}^{M\times 1}$ and $\textbf{g}^{[k]}(t) \in \mathbb{C}^{1\times M}$, respectively, where $j,k \in \{1,2,\ldots,K\}$, $K$ is the number of transmitter-receiver pairs, and $M$ denotes the number of RIS elements. We use Rician fading to model $\textbf{h}^{[j]}(t)$ and express $h_m^{[j]}(t)$, the $m^{\mathrm{th}}$ element of $\textbf{h}^{[j]}(t), 1 \leq m \leq M$, as follows:
\begin{align}
    \label{eq:Rician_fading}
    h_m^{[j]}(t)=\sqrt{\frac{1}{1+\kappa}}h_m^{[j],NLoS}(t)+\sqrt{\frac{\kappa}{1+\kappa}}h_m^{[j],LoS},
\end{align}
where $\kappa$ is the Rician factor, $h_m^{[j],NLoS}(t) \thicksim \mathcal{CN}(0,C_0d_{1,j}^{-\alpha_1})$ represents the non-line-of-sight (NLoS) component of $h_m^{[j]}(t)$, and $h_m^{[j],LoS}=\sqrt{C_0d_{1,j}^{-\alpha_1}}e^{-j\frac{2 \pi }{\lambda}d_{1,j}}$ shows the line-of-sight (LoS) part of $h_m^{[j]}(t)$, where $d_{1,j}$ denotes the distance between ${\sf Tx}_j$ and RIS, $\alpha_1$ is the path loss exponent between them, and $\lambda$ is the wavelength of the transmitted signal. We use $C_0$ to capture the signal loss at a reference distance, e.g., $1\mathrm{m}$. Here, $\textbf{g}^{[k]}(t)$ follows Rayleigh fading whose elements are modeled as a complex Gaussian distribution with zero mean and variance $C_0d_{2,k}^{-\alpha_2}$, where $d_{2,k}$ and $\alpha_2$ denote the distance and path loss exponent between RIS and ${\sf Rx}_k$, respectively. 

We assume that the direct path between transmitters and receivers is blocked. We also suppose that the channels are independent due to the spacing of the RIS elements being at least $\lambda/2$ apart. Similar to~\cite{fu2021reconfigurable,wu2019intelligent}, we assume that channel state information (CSI) is available globally, and beyond that, there is no data exchange between transmitters or receivers. We note that all operations occur within a single coherence time; hence, we omit the time notation in the rest of this paper.

\begin{comment}
\textbf{CSI resolution:} In this work, we assume that each receiver estimates its incoming channels from all transmitters using the pilot signals and then informs the others, while the estimated CSI is different from the actual CSI due to different reasons such as noise, hardware impairments, and unfavorable environments. Thus, we have: 
\begin{align}
    &\hat{\textbf{h}}^{[j]}(t) = \textbf{h}^{[j]}(t) + \mathbf{e}^{[j]}_h(t),~~1 \leq j \leq K,\\ \nonumber
    &\hat{\textbf{g}}^{[k]}(t) = \textbf{g}^{[k]}(t) + \mathbf{e}^{[k]}_g(t),~~1 \leq k \leq K,
\end{align}
where $\mathbf{e}^{[j]}_h(t)\in \mathbb{C}^{M\times 1}$ and $\mathbf{e}^{[k]}_g(t)\in \mathbb{C}^{1\times M}$ are the estimation errors whose elements are distributed based on $\mathcal{CN}(0,1/p)$, and $p$ denotes the signal-to-noise ratio (SNR) during the estimation process.
\end{comment}

\begin{figure}[ht]
%\vspace{-3mm}
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=7, width=0.8\linewidth, draft=false]{images/channel_model_IRIS.png}
  \vspace{-4mm}
  \caption{A SISO network with an RIS assisting multi-user communications.%\avc{Remove the controller from the figure, it is weird that the RIS is controlled by the BS rather than a big host ship. Maybe add a UAV too. Watch: https://www.youtube.com/watch?v=P2tSwngihp0}
}\label{Fig:channel_model_standard_RIS}
  \vspace{-4mm}
\end{figure}

\begin{figure*}[ht]
%\vspace{-3mm}
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=4, width=0.9\linewidth, draft=false]{images/std_general_RIS_models_5.png}
  \vspace{-4mm}
  \caption{(a) A $32$-element S-RIS, where the $m^{\mathrm{th}}$ RIS element uses an RF switch to either reflect or block its incident signal; (b) An I-RIS with $32$ elements and eight cells of size $(2,2)$; (c) The $m^{\mathrm{th}}$ arrival element uses $cd$ RF switches and a power splitter to share its incident signal; (d) The reflected signal from the $m^{\mathrm{th}}$ departure element includes a combination of the incident signals at all arrival elements.}\label{Fig:channel_model_new_RIS}
  \vspace{-2mm}
\end{figure*}
%\vspace{10mm}
\subsection{Existing vs. the proposed RIS design}
In this subsection, we delve into the details of two RIS structures using RF switches. Here, each RIS element has an arrival part that receives the incident signals from transmitters and a departure part that reflects the signals toward receivers.% We place a controller between a control unit, e.g., a shore control center, and the RIS to exchange CSI and control RIS elements over a separate communication link.

\textbf{S-RIS:} In this RIS, there is no interconnection between the elements. The $m^{\mathrm{th}}$ RIS element, $1 \leq m \leq M$, receives the incident signal and then uses its binary RF switch, $s_{m}\in \{0,1\}$ between its arrival and departure parts, to either reflect or block its incident signal as shown in Fig.~\ref{Fig:channel_model_new_RIS}(a). We define $\mathbf{T}^{\mathrm{s}}$ as the S-RIS configuration, which is given by:
\begin{align}
\mathbf{T}^{\mathrm{s}}=\mathrm{diag}\left\{\boldsymbol{\tau}^{\mathrm{s}}\right\},~~~\boldsymbol{\tau}^{\mathrm{s}}=\left[s_{1},s_{2},\ldots,s_{M}\right]^{\top}.
\end{align}

\textbf{I-RIS:} Here, we first divide RIS into $M/(c \times d)$ different cells, where $c$ and $d$ represent the cell size. (e.g., Fig.~\ref{Fig:channel_model_new_RIS}(b) shows a $32$-element I-RIS with eight cells of size $(2, 2)$.) Without loss of generality, we suppose $M$ is divisible by $c \times d$. In the rest of this work, we use $cd$ to denote $c \times d$. Next, each element within a given cell shares its incident signal with its neighbors in that cell, as depicted in Fig.~\ref{Fig:channel_model_new_RIS}(c). We define $\mathcal{M}^{[m]}$ as a cell that includes the $m^{\mathrm{th}}$ element. Then, the $m^{\mathrm{th}}$ RIS element uses $cd$ binary RF switches to determine  $\bar{\mathcal{M}}^{[m]}\subseteq \mathcal{M}^{[m]}$, which contains the active elements in the cell obtaining the incident signal received by the $m^{\mathrm{th}}$ arrival element. The $m^{\mathrm{th}}$ arrival element uses a power splitter to distribute the incident signal power uniformly across all members of $\bar{\mathcal{M}}^{[m]}$. Then, to indicate how the $m^{\mathrm{th}}$ arrival element connects to the $\ell^{\mathrm{th}}$ departure element, $1\leq \ell,M\leq M$, we define $\tau_{\ell, m}$ as:
% $\tau_{\ell, m}=\left(1/\sqrt{\left|\bar{\mathcal{M}}^{[m]}\right|}\right)s_{\ell, m}$ when $\ell\in \mathcal{M}^{[m]}$; conversely, $\tau_{\ell, m}=0$ if $\ell\notin \mathcal{M}^{[m]}$.
\begin{align}
\tau_{\ell, m}=\left\{ \begin{array}{ll} \left(1/\sqrt{\left|\bar{\mathcal{M}}^{[m]}\right|}\right)s_{\ell, m}, & \ell\in \mathcal{M}^{[m]}, \\
0, & \ell\notin \mathcal{M}^{[m]},
\end{array} \right.
\end{align}
where $s_{\ell, m}\in \{0,1\}$ is a binary RF switch between the $m^{\mathrm{th}}$ arrival element and the $\ell^{\mathrm{th}}$ departure element, and $1/\sqrt{\left|\bar{\mathcal{M}}^{[m]}\right|}$ guarantees $\sum_{\ell=1}^M |\tau_{\ell, m}|^2\leq1$, where the inequality holds true only if all switches from the $m^{\mathrm{th}}$ arrival element to its neighbors are zero. In this case $\sum_{\ell=1}^M |\tau_{\ell, m}|^2 =0 <1$. %, i.e., RIS elements are passive. We note that I-RIS is nearly-passive as it requires control signals to activate or deactivate its RF switches. %\avc{1. ``.'' then i.e., does not work, 2. the sentence after i.e. is not well written, it simply means sharing is useless, you want to say the I-RIS elements are passive} (i.e., there is no gain from power sharing at the $m^{\mathrm{th}}$ arrival element.)
Then, we use $\mathbf{T}^{\mathrm{i}}$ to denote the I-RIS configuration as:
\begin{align}
    \mathbf{T}^{\mathrm{i}}=\mathrm{blkdiag}\left\{\boldsymbol{\tau}^{\mathrm{i}[1]},\boldsymbol{\tau}^{\mathrm{i}[2]}, \ldots, \boldsymbol{\tau}^{\mathrm{i}[\frac{M}{cd}]}\right\},
\end{align}
where $\boldsymbol{\tau}^{\mathrm{i}[u]}, 1\leq u \leq \frac{M}{cd}$ follows \eqref{eq:tau_general_vector}.
\begin{figure*}
\begin{align}
\label{eq:tau_general_vector}
    \boldsymbol{\tau}^{\mathrm{i}[u]} = \begin{bmatrix}
\tau^{\mathrm{i}[u]}_{1,1} & \tau^{\mathrm{i}[u]}_{1,2} & \ldots & \tau^{\mathrm{i}[u]}_{1,cd}\\
\vdots & \vdots & \ldots & \vdots
\\
\tau^{\mathrm{i}[u]}_{cd,1} & \tau^{\mathrm{i}[u]}_{cd,2} & \ldots & \tau^{\mathrm{i}[u]}_{cd, cd}
\end{bmatrix} = \begin{bmatrix}
\tau_{(u-1)cd+1,(u-1)cd+1} & \tau_{(u-1)cd+1,(u-1)cd+2} & \ldots & \tau_{(u-1)cd+1,ucd}\\
\vdots & \vdots & \ldots & \vdots
\\
\tau_{ucd,(u-1)cd+1} & \tau_{ucd,(u-1)cd+2} & \ldots & \tau_{ucd,ucd}
\end{bmatrix}.
\end{align}
\hrule
\end{figure*}
We consider $\boldsymbol{\tau}^{\mathrm{i}[u]}=\hat{\boldsymbol{\tau}}^{\mathrm{i}[u]}+\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}$. For each $\tau^{\mathrm{i}[u]}_{u_1,u_2}, 1 \leq u_1, u_2 \leq cd$, if it is the only non-zero element in the $u_1^{\mathrm{th}}$ row and $u_2^{\mathrm{th}}$ column of $\boldsymbol{\tau}^{\mathrm{i}[u]}$, we include $\tau^{\mathrm{i}[u]}_{u_1,u_2}$ in $\hat{\boldsymbol{\tau}}^{\mathrm{i}[u]}$ by following~\eqref{eq:hat_tau}; otherwise, we save $\tau^{\mathrm{i}[u]}_{u_1,u_2}$ in $\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}$ as~\eqref{eq:tilde_tau}. We show \eqref{eq:tau_general_vector},~\eqref{eq:hat_tau}, and~\eqref{eq:tilde_tau} at the top of the next page.  
\begin{figure*}
\begin{minipage}[t]{0.50\linewidth}
\begin{equation}
\label{eq:hat_tau}
\hat{\tau}^{\mathrm{i}[u]}_{u_1,u_2}=\left\{ \begin{array}{ll} \tau^{\mathrm{i}[u]}_{u_1,u_2}, & \sum_{q=1}^{cd}\left(\tau^{\mathrm{i}[u]}_{u_1,q} + \tau^{\mathrm{i}[u]}_{q,u_2} \right) = 2\tau^{\mathrm{i}[u]}_{u_1,u_2}, \\
0, & \text{otherwise},
\end{array} \right.
\end{equation}
\end{minipage}
 % Adjust the spacing between equations
\begin{minipage}[t]{0.50\linewidth}
\begin{equation}
\label{eq:tilde_tau}
\tilde{\tau}^{\mathrm{i}[u]}_{u_1,u_2}=\left\{ \begin{array}{ll} \tau^{\mathrm{i}[u]}_{u_1,u_2}, & \sum_{q=1}^{cd}\left(\tau^{\mathrm{i}[u]}_{u_1,q} + \tau^{\mathrm{i}[u]}_{q,u_2}\right) \neq 2\tau^{\mathrm{i}[u]}_{u_1,u_2}, \\
0, & \text{otherwise},
\end{array} \right.
\end{equation}
\end{minipage}
\hrule
\end{figure*}Then, based on Fig.~\ref{Fig:channel_model_new_RIS}(d), to ensure I-RIS is passive, we normalize $\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}$, i.e., replace $\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}$ with $\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}/||\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}||_{\mathrm{F}}$. Finally, the $m^{\mathrm{th}}$ departure element mixes the incident signals of all elements in $\mathcal{M}^{[m]}$ and reflects a combination of them toward the receivers.

\textbf{Received signal:} ${\sf Rx}_{k}, 1\leq k \leq K,$ receives the reflected signals from the RIS, which is given by:
\begin{align}
\label{eq_ch5:received_sig_a_RIS}
    y_{k}=\sum_{j=1}^K \Big[\textbf{g}^{[k]}\mathbf{T}\textbf{h}^{[j]}\Big]x_j+n_{k},
\end{align}
where $\mathbf{T} \in \left\{\mathbf{T}^{\mathrm{s}}, \mathbf{T}^{\mathrm{i}}\right\}$, $x_j$ is the transmitted signal from ${\sf Tx}_j$, and $n_{k} \thicksim \mathcal{CN}(0,\sigma^2)$ denotes noise at ${\sf Rx}_{k}$. Here, $\mathbb{E}\left\{\textbf{x}\textbf{x}^{H}\right\}=\mathrm{diag}([P_1, P_2,\ldots,P_K])$, where $\textbf{x}=[x_1,x_2,\ldots,x_K] \in \mathbb{C}^{1\times K}$, and $P_j$ is the transmit power from ${\sf Tx}_j$.  Then, we use \eqref{eq_ch5:received_sig_a_RIS} to express the signal-to-interference-plus-noise ratio (SINR) at ${\sf Rx}_{k}$ as follows:
\begin{align}
\label{eq_ch5:SINR_update_a_RIS}
    \text{SINR}_{k}=\frac{P_{k}\Big|\textbf{g}^{[k]}\mathbf{T}\textbf{h}^{[k]}\Big|^2}{\sigma^2+\sum_{j=1, j\neq k}^{K }P_j\Big|\textbf{g}^{[k]}\mathbf{T}\textbf{h}^{[j]}\Big|^2}.
\end{align} 


==> Sections/Sect2_Problem_setting_RIS_structure_v3.tex <==
In this paper, we examine an RIS-assisted network with distributed transmitter-receiver pairs where each transmitter aims to communicate with only one desired receiver, as shown in Fig.~\ref{Fig:channel_model_standard_RIS}. Further, we focus on a SISO scenario to highlight the pure RIS gain in the network.

\subsection{Channel Model} We denote the channels between ${\sf Tx}_j$ and RIS, and between RIS and ${\sf Rx}_{k}$ at time $t$ as $\textbf{h}^{j}(t) \in \mathbb{C}^{M\times 1}$ and $\textbf{g}^{k}(t) \in \mathbb{C}^{1\times M}$, respectively. Here, $j,k \in \{1,2,\ldots,K\}$, $K$ is the number of transmitter-receiver pairs, and $M$ is the number of RIS elements. We use Rician fading to model $\textbf{h}^{j}(t)$ and express $h_m^{j}(t)$, the $m^{\mathrm{th}}$ element of $\textbf{h}^{j}(t), 1 \leq m \leq M$, as follows:
\begin{align}
    \label{eq:Rician_fading}
    h_m^{j}(t)=\sqrt{\frac{1}{1+\kappa}}h_m^{j,NLoS}(t)+\sqrt{\frac{\kappa}{1+\kappa}}h_m^{j,LoS},
\end{align}
where $\kappa$ is the Rician factor, $h_m^{j,NLoS}(t) \thicksim \mathcal{CN}(0,C_0d_{1,j}^{-\alpha_1})$ represents the non-line-of-sight (NLoS) component of $h_m^{j}(t)$, and $h_m^{j,LoS}=\sqrt{C_0d_{1,j}^{-\alpha_1}}e^{-j\frac{2 \pi }{\lambda}d_{1,j}}$ shows the line-of-sight (LoS) part of $h_m^{j}(t)$, where $d_{1,j}$ denotes the distance between ${\sf Tx}_j$ and RIS, $\alpha_1$ is the path loss exponent between them, and $\lambda$ is the wavelength of the transmitted signal. We use $C_0$ to capture the signal loss at a reference distance, e.g., $1\mathrm{m}$. Here, $\textbf{g}^{k}(t)$ follows Rayleigh fading whose elements are modeled as a complex Gaussian distribution with zero mean and variance $C_0d_{2,k}^{-\alpha_2}$, where $d_{2,k}$ and $\alpha_2$ denote the distance and path loss exponent between RIS and ${\sf Rx}_k$, respectively. 

We assume that the direct path between transmitters and receivers is blocked, and the channels are independent due to the spacing of the RIS elements being at least $\lambda/2$ apart. Similar to~\cite{fu2021reconfigurable}, we assume that global channel state information (CSI) is available with no data exchange between transmitters or receivers. All operations occur within a single coherence time; hence, we omit the time notation in the rest of this paper.

\begin{comment}
\textbf{CSI resolution:} In this work, we assume that each receiver estimates its incoming channels from all transmitters using the pilot signals and then informs the others, while the estimated CSI is different from the actual CSI due to different reasons such as noise, hardware impairments, and unfavorable environments. Thus, we have: 
\begin{align}
    &\hat{\textbf{h}}^{j}(t) = \textbf{h}^{j}(t) + \mathbf{e}^{j}_h(t),~~1 \leq j \leq K,\\ \nonumber
    &\hat{\textbf{g}}^{k}(t) = \textbf{g}^{k}(t) + \mathbf{e}^{k}_g(t),~~1 \leq k \leq K,
\end{align}
where $\mathbf{e}^{j}_h(t)\in \mathbb{C}^{M\times 1}$ and $\mathbf{e}^{k}_g(t)\in \mathbb{C}^{1\times M}$ are the estimation errors whose elements are distributed based on $\mathcal{CN}(0,1/p)$, and $p$ denotes the signal-to-noise ratio (SNR) during the estimation process.
\end{comment}

\begin{figure}[ht]
\vspace{-3mm}
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=7, width=0.78\linewidth, draft=false]{images/channel_model_IRIS.png}
  \vspace{-4mm}
  \caption{A SISO network with an RIS assisting multi-user communications.%\avc{Remove the controller from the figure, it is weird that the RIS is controlled by the BS rather than a big host ship. Maybe add a UAV too. Watch: https://www.youtube.com/watch?v=P2tSwngihp0}
}\label{Fig:channel_model_standard_RIS}
  \vspace{-2mm}
\end{figure}

\begin{figure*}[ht]
%\vspace{-3mm}
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=4, width=0.9\linewidth, draft=false]{images/std_general_RIS_models_5.png}
  \vspace{-4mm}
  \caption{(a) A $32$-element S-RIS, where the $m^{\mathrm{th}}$ RIS element uses an RF switch to either reflect or block its incident signal; (b) An I-RIS with $32$ elements and eight cells of size $(2,2)$; (c) The $m^{\mathrm{th}}$ arrival element uses $cd$ RF switches and a power splitter to share its incident signal; (d) The reflected signal from the $m^{\mathrm{th}}$ departure element includes a combination of the incident signals at all arrival elements.}\label{Fig:channel_model_new_RIS}
  \vspace{-2mm}
\end{figure*}
%\vspace{10mm}
\subsection{Existing vs. The Proposed RIS Design}
In this subsection, we delve into the details of two RIS structures using RF switches. Here, each RIS element has an arrival part that receives the incident signals from transmitters and a departure part that reflects the signals toward receivers.% We place a controller between a control unit, e.g., a shore control center, and the RIS to exchange CSI and control RIS elements over a separate communication link.

\textbf{S-RIS:} In this RIS, there is no interconnection between the elements. The $m^{\mathrm{th}}$ RIS element, $1 \leq m \leq M$, receives the incident signal and then uses its binary RF switch, $s_{m}\in \{0,1\}$ between its arrival and departure parts, to either reflect or block its incident signal as shown in Fig.~\ref{Fig:channel_model_new_RIS}(a). We define $\mathbf{T}^{\mathrm{s}}$ as the S-RIS configuration, which is given by:
\begin{align}
\mathbf{T}^{\mathrm{s}}=\mathrm{diag}\left\{\boldsymbol{\tau}^{\mathrm{s}}\right\},~~~\boldsymbol{\tau}^{\mathrm{s}}=\left[s_{1},s_{2},\ldots,s_{M}\right]^{\top}.
\end{align}

\textbf{I-RIS:} Here, we first divide RIS into $M/(c \times d)$ different cells, where $c$ and $d$ represent the cell size. (e.g., Fig.~\ref{Fig:channel_model_new_RIS}(b) shows a $32$-element I-RIS with eight cells of size $(2, 2)$.) Without loss of generality, we suppose $M$ is divisible by $c \times d$. In the rest of this work, we use $cd$ to denote $c \times d$. Next, each element within a given cell shares its incident signal with its neighbors in that cell, as depicted in Fig.~\ref{Fig:channel_model_new_RIS}(c). We define $\mathcal{M}^{[m]}$ as a cell that includes the $m^{\mathrm{th}}$ element. Then, the $m^{\mathrm{th}}$ RIS element uses $cd$ binary RF switches to determine  $\bar{\mathcal{M}}^{[m]}\subseteq \mathcal{M}^{[m]}$, which contains the active elements in the cell obtaining the incident signal received by the $m^{\mathrm{th}}$ arrival element. The $m^{\mathrm{th}}$ arrival element uses a power splitter to distribute the incident signal power uniformly across all members of $\bar{\mathcal{M}}^{[m]}$. Then, to indicate how the $m^{\mathrm{th}}$ arrival element connects to the $\ell^{\mathrm{th}}$ departure element, $1\leq \ell,m\leq M$, we define $\tau_{\ell, m}$ as:
$\tau_{\ell, m}=\left(1/\sqrt{\left|\bar{\mathcal{M}}^{[m]}\right|}\right)s_{\ell, m}$ when $\ell\in \mathcal{M}^{[m]}$; conversely, $\tau_{\ell, m}=0$ if $\ell\notin \mathcal{M}^{[m]}$.
% \begin{align}
% \tau_{\ell, m}=\left\{ \begin{array}{ll} \left(1/\sqrt{\left|\bar{\mathcal{M}}^{[m]}\right|}\right)s_{\ell, m}, & \ell\in \mathcal{M}^{[m]}, \\
% 0, & \ell\notin \mathcal{M}^{[m]},
% \end{array} \right.
% \end{align}
Here, $s_{\ell, m}\in \{0,1\}$ is a binary RF switch between the $m^{\mathrm{th}}$ arrival element and the $\ell^{\mathrm{th}}$ departure element, and $1/\sqrt{\left|\bar{\mathcal{M}}^{[m]}\right|}$ guarantees $\sum_{\ell=1}^M |\tau_{\ell, m}|^2\leq1$, where the inequality holds true only if $\tau_{\ell, m} = 0, \forall{\ell}$, leading to $\sum_{\ell=1}^M |\tau_{\ell, m}|^2 =0 <1$. %, i.e., RIS elements are passive. We note that I-RIS is nearly-passive as it requires control signals to activate or deactivate its RF switches. %\avc{1. ``.'' then i.e., does not work, 2. the sentence after i.e. is not well written, it simply means sharing is useless, you want to say the I-RIS elements are passive} (i.e., there is no gain from power sharing at the $m^{\mathrm{th}}$ arrival element.)
Then, we use $\mathbf{T}^{\mathrm{i}}$ to denote the I-RIS configuration as:
\begin{align}
    \mathbf{T}^{\mathrm{i}}=\mathrm{blkdiag}\left\{\boldsymbol{\tau}^{\mathrm{i}[1]},\boldsymbol{\tau}^{\mathrm{i}[2]}, \ldots, \boldsymbol{\tau}^{\mathrm{i}[\frac{M}{cd}]}\right\},
\end{align}
where $\boldsymbol{\tau}^{\mathrm{i}[u]}, 1\leq u \leq \frac{M}{cd}$ follows \eqref{eq:tau_general_vector}.
\begin{figure*}
\begin{align}
\label{eq:tau_general_vector}
    \boldsymbol{\tau}^{\mathrm{i}[u]} = \begin{bmatrix}
\tau^{\mathrm{i}[u]}_{1,1} & \tau^{\mathrm{i}[u]}_{1,2} & \ldots & \tau^{\mathrm{i}[u]}_{1,cd}\\
\vdots & \vdots & \ldots & \vdots
\\
\tau^{\mathrm{i}[u]}_{cd,1} & \tau^{\mathrm{i}[u]}_{cd,2} & \ldots & \tau^{\mathrm{i}[u]}_{cd, cd}
\end{bmatrix} = \begin{bmatrix}
\tau_{(u-1)cd+1,(u-1)cd+1} & \tau_{(u-1)cd+1,(u-1)cd+2} & \ldots & \tau_{(u-1)cd+1,ucd}\\
\vdots & \vdots & \ldots & \vdots
\\
\tau_{ucd,(u-1)cd+1} & \tau_{ucd,(u-1)cd+2} & \ldots & \tau_{ucd,ucd}
\end{bmatrix}.
\end{align}
\hrule
\end{figure*}
We consider $\boldsymbol{\tau}^{\mathrm{i}[u]}=\hat{\boldsymbol{\tau}}^{\mathrm{i}[u]}+\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}$. For each $\tau^{\mathrm{i}[u]}_{u_1,u_2}, 1 \leq u_1, u_2 \leq cd$, if it is the only non-zero element in the $u_1^{\mathrm{th}}$ row and $u_2^{\mathrm{th}}$ column of $\boldsymbol{\tau}^{\mathrm{i}[u]}$, we include $\tau^{\mathrm{i}[u]}_{u_1,u_2}$ in $\hat{\boldsymbol{\tau}}^{\mathrm{i}[u]}$ by following~\eqref{eq:hat_tau}; otherwise, we save $\tau^{\mathrm{i}[u]}_{u_1,u_2}$ in $\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}$ as~\eqref{eq:tilde_tau}. We show \eqref{eq:tau_general_vector},~\eqref{eq:hat_tau}, and~\eqref{eq:tilde_tau} at the top of the next page.  
\begin{figure*}
\begin{minipage}[t]{0.50\linewidth}
\begin{equation}
\label{eq:hat_tau}
\hat{\tau}^{\mathrm{i}[u]}_{u_1,u_2}=\left\{ \begin{array}{ll} \tau^{\mathrm{i}[u]}_{u_1,u_2}, & \sum_{q=1}^{cd}\left(\tau^{\mathrm{i}[u]}_{u_1,q} + \tau^{\mathrm{i}[u]}_{q,u_2} \right) = 2\tau^{\mathrm{i}[u]}_{u_1,u_2}, \\
0, & \text{otherwise},
\end{array} \right.
\end{equation}
\end{minipage}
 % Adjust the spacing between equations
\begin{minipage}[t]{0.50\linewidth}
\begin{equation}
\label{eq:tilde_tau}
\tilde{\tau}^{\mathrm{i}[u]}_{u_1,u_2}=\left\{ \begin{array}{ll} \tau^{\mathrm{i}[u]}_{u_1,u_2}, & \sum_{q=1}^{cd}\left(\tau^{\mathrm{i}[u]}_{u_1,q} + \tau^{\mathrm{i}[u]}_{q,u_2}\right) \neq 2\tau^{\mathrm{i}[u]}_{u_1,u_2}, \\
0, & \text{otherwise},
\end{array} \right.
\end{equation}
\end{minipage}
\hrule
\end{figure*}Then, based on Fig.~\ref{Fig:channel_model_new_RIS}(d), to ensure I-RIS is passive, we normalize $\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}$, i.e., replace $\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}$ with $\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}/||\Tilde{\boldsymbol{\tau}}^{\mathrm{i}[u]}||_{\mathrm{F}}$. Finally, the $m^{\mathrm{th}}$ departure element mixes the incident signals of all elements in $\mathcal{M}^{[m]}$ and reflects a combination of them toward the receivers.

\textbf{Received signal:} ${\sf Rx}_{k}, 1\leq k \leq K,$ receives the reflected signals from the RIS, which is given by:
\begin{align}
\label{eq_ch5:received_sig_a_RIS}
    y_{k}=\sum_{j=1}^K \Big[\textbf{g}^{k}\mathbf{T}\textbf{h}^{j}\Big]x_j+n_{k},
\end{align}
where $\mathbf{T} \in \left\{\mathbf{T}^{\mathrm{s}}, \mathbf{T}^{\mathrm{i}}\right\}$, $x_j$ is the transmitted signal from ${\sf Tx}_j$, and $n_{k} \thicksim \mathcal{CN}(0,\sigma^2)$ denotes noise at ${\sf Rx}_{k}$. Here, $\mathbb{E}\left\{\textbf{x}^{H}\textbf{x}\right\}=\mathrm{diag}([P_1, P_2,\ldots,P_K])$, where $\textbf{x}=[x_1,x_2,\ldots,x_K] \in \mathbb{C}^{1\times K}$, and $P_j$ is the transmit power from ${\sf Tx}_j$.  Then, we use \eqref{eq_ch5:received_sig_a_RIS} to express the signal-to-interference-plus-noise ratio (SINR) at ${\sf Rx}_{k}$ as follows:
\begin{align}
\label{eq_ch5:SINR_update_a_RIS}
    \text{SINR}_{k}=\frac{P_{k}\Big|\textbf{g}^{k}\mathbf{T}\textbf{h}^{k}\Big|^2}{\sigma^2+\sum_{j=1, j\neq k}^{K }P_j\Big|\textbf{g}^{k}\mathbf{T}\textbf{h}^{j}\Big|^2}.
\end{align} 


==> Sections/Sect3_Beamforming_design.tex <==
We aim to optimize RIS elements to maximize the sum-rate; thus, we formulate our optimization problem as:
\begin{align}
\label{eq:opt_prob_std_RIS_feb_27_2023}
    &\underset{\mathbf{T}}{\max}\underbrace{\sum_{\gidx=1}^{K} \log(1+\text{SINR}_{\gidx})}_{\overset{\triangle}=~-w(\mathbf{T})}\equiv \underset{\mathbf{T}}{\min}~w(\mathbf{T})\\ \nonumber
    &\text{s.t.} ~~\mathbf{T} \in \{\mathbf{T}^{\mathrm{s}}, \mathbf{T}^{\mathrm{i}}\},~~  s_m,s_{\ell m}\in\{0,1\},~~1\leq \ell,m\leq M,
\end{align}
which is non-convex due to the binary constraints and the non-convex objective function. To optimize~\eqref{eq:opt_prob_std_RIS_feb_27_2023}, we first focus on S-RIS where $\mathbf{T}=\mathbf{T}^{\mathrm{s}}$ and propose two methods to solve the problem: (1) we use the %\avc{write out the full name again} 
semi-definite binary optimization (SBO) method, which converts~\eqref{eq:opt_prob_std_RIS_feb_27_2023} to a semi-definite relaxation (SDR) problem and then solves the equivalent convex problem; (2) we utilize the sigmoid filled function (SFF), which is a heuristic method based on filled function that directly targets \eqref{eq:opt_prob_std_RIS_feb_27_2023} to obtain an approximation of the global optimum solution. We provide further details below. 

\textbf{SBO method:} In this case, to address the non-convexity of the binary constraints, we use slack variable $\textbf{S}$ and rewrite the binary constraint as follows:
\begin{align}
\label{eq:Diag_S_feb_27_2023}
    \mathrm{Diag}(\textbf{S})=\boldsymbol{\tau}^{\mathrm{s}}, 
\end{align}
\begin{align}
\label{eq:S=ss_feb_27_2023}
    \textbf{S}=\boldsymbol{\tau}^{\mathrm{s}}{\boldsymbol{\tau}^{\mathrm{s}}}^{\top},
\end{align}
\begin{align}
\label{eq:01_values_feb_27_2023}
    0 \leq s_m \leq 1,~\text{and}~0 \leq S_{\ell m} \leq 1,~~ \text{for}~ 1\leq \ell,m \leq M,
\end{align}
where $S_{\ell m}$ is an element located at the $\ell^{\mathrm{th}}$ row and the $m^{\mathrm{th}}$ column of $\textbf{S}$. Here, \eqref{eq:S=ss_feb_27_2023} is non-convex; therefore, we substitute it with the following conditions~\cite{guo2018new,hu2021robust}.
\begin{align}
\label{eq:Y_matrix_feb_27_2023}
    \textbf{Y}=\begin{bmatrix}
        \textbf{S}& \boldsymbol{\tau}^{\mathrm{s}}\\
        {\boldsymbol{\tau}^{\mathrm{s}}}^{\top}& 1\\
    \end{bmatrix}\succeq \mathbf{0},~~\text{and} ~~ \text{Rank}(\textbf{Y})=1.
\end{align}

Since $\textbf{Y}$ includes binary elements, the rank of $\textbf{Y}$ is equal to one for any binary feasible solution. Next, we define $\textbf{G}^{[\gidx j]}\overset{\triangle}=\textbf{g}^{[\gidx]} \mathrm{diag}(\textbf{h}^{[j]})$ and $\bar{\textbf{G}}^{[\gidx j]}\overset{\triangle}=\textbf{G}^{[\gidx j]}{\textbf{G}^{[\gidx j]}}^{\textrm{H}}$ and use \eqref{eq:Diag_S_feb_27_2023}, \eqref{eq:01_values_feb_27_2023}, and \eqref{eq:Y_matrix_feb_27_2023} to rewrite~\eqref{eq:opt_prob_std_RIS_feb_27_2023} as an SDR problem as follows:
\begin{align}
\label{eq:finalswitch_SNR_feb_27_2023}
    &\underset{\boldsymbol{\tau}^{\mathrm{s}},\textbf{S} }{\min}~-\sum_{\gidx=1}^K\log\left(1+\frac{P_{\gidx}~\mathrm{tr}\left(\textbf{S}\bar{\textbf{G}}^{[\gidx \gidx ]}\right)}{\sigma^2+\sum_{j=1,j\neq \gidx}^K P_j~\mathrm{tr}\left(\textbf{S}\bar{\textbf{G}}^{[\gidx j]}\right) }\right)\\ \nonumber
    &\text{s.t.} ~~ \mathrm{Diag}(\textbf{S})=\boldsymbol{\tau}^{\mathrm{s}}, \\ \nonumber 
    & ~~~~~~\textbf{Y}\succeq \mathbf{0}, \\ \nonumber 
    & ~~~~~~0 \leq s_m \leq 1,~~0 \leq S_{\ell m} \leq 1,~~ \text{for}~ 1\leq \ell,m \leq M.
\end{align}

Then, we use the feature of a logarithmic function and rewrite~\eqref{eq:finalswitch_SNR_feb_27_2023} as:
\begin{align}
\label{eq:finalswitch_SINR_Dbi_Nbi_feb_27_2023}
    &\underset{\boldsymbol{\tau}^{\mathrm{s}},\textbf{S} }{\min}~N-D\\ \nonumber
    &\text{s.t.} ~~ \mathrm{Diag}(\textbf{S})=\boldsymbol{\tau}^{\mathrm{s}}, \\ \nonumber 
    & ~~~~~~\textbf{Y}\succeq \mathbf{0}, \\ \nonumber 
    & ~~~~~~0 \leq s_m \leq 1,~~0 \leq S_{\ell m} \leq 1,~~ \text{for}~ 1\leq \ell,m \leq M,
\end{align}
where
\begin{align}
    \label{eq:SINR_noise_Nbi_feb_27_2023}
    N=-\sum_{\gidx=1}^K\log\left(\sigma^2+\sum_{j=1}^K P_{j}~\mathrm{tr}\left(\textbf{S}\bar{\textbf{G}}^{[\gidx j]}\right)\right),
\end{align}
and
\begin{align}
    \label{eq:SINR_noise_Dbi_feb_27_2023}
    D=-\sum_{\gidx=1}^K\log\left(\sigma^2+\sum_{j=1, j\neq \gidx}^K P_j~\mathrm{tr}\left(\textbf{S}\bar{\textbf{G}}^{[\gidx j]}\right)\right).
\end{align}

Based on \eqref{eq:SINR_noise_Nbi_feb_27_2023} and \eqref{eq:SINR_noise_Dbi_feb_27_2023}, $N$ and $D$ are convex with respect to $\textbf{S}$; thus,~\eqref{eq:finalswitch_SINR_Dbi_Nbi_feb_27_2023} falls under the difference of convex (DC) optimization problem. To solve this problem, we use the SCA method, which is an iterative approach that runs for $I_{\mathrm{tr}}$ times. To do so, we apply the first-order Taylor approximation to $D$ and obtain a lower bound on that as follows:
\begin{align}
\label{eq:lower_bound_Dbi_formula_feb_27_2023}
    D(\textbf{S})\geq D\left(\textbf{S}^t\right)+\nabla^{\top}_{\textbf{S}}\left(D\left(\textbf{S}^t\right)\right)\left(\textbf{S}-\textbf{S}^t\right),
\end{align}
where $\textbf{S}^t$ is the value of $\textbf{S}$ in the $t^{\mathrm{th}}$ iteration and 
\begin{align}
\label{eq:lower_bound_Dbi_feb_27_2023}
    \nabla^{\top}_{\textbf{S}}\left(D\left(\textbf{S}^t\right)\right)=-\frac{1}{\mathrm{ln}~2}\sum_{\gidx=1}^K\frac{\sum_{j=1, j\neq \gidx}^K P_j\bar{\textbf{G}}^{[\gidx j]}}{\sigma^2+\sum_{j=1, j\neq \gidx}^K P_j~\mathrm{tr}\left(\textbf{S}^t\bar{\textbf{G}}^{[\gidx j]}\right)}.
\end{align} 

By applying \eqref{eq:lower_bound_Dbi_formula_feb_27_2023} to \eqref{eq:finalswitch_SINR_Dbi_Nbi_feb_27_2023}, we obtain a convex SDR problem and solve it using CVX Toolbox in MATLAB~\cite{grant2011matlab}.

\textbf{SFF method:} Heuristic optimization methods (e.g., genetic algorithm and filled function) are popular for optimizing non-convex problems. Unlike the SBO method, a heuristic method directly tackles the non-convex problem in~\eqref{eq:opt_prob_std_RIS_feb_27_2023} without needing approximations for a convex equivalent. This avoids the performance degradation associated with the approximations used in the SBO method. Hence, we utilize the SFF method based on sigmoid filled function as our second optimization method in this paper to solve~\eqref{eq:opt_prob_std_RIS_feb_27_2023}. This method includes two steps: local and global search. Prior to explaining the details, we need to define: (i) $\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})\overset{\triangle}=w(\textbf{T}^{\mathrm{s}})$, and (ii) $\left[\boldsymbol{\tau}^{\mathrm{s}}\right]_n\in \{0,1\}^{M \times 1}$ as the $n^{\mathrm{th}}$ neighbor of $\boldsymbol{\tau}^{\mathrm{s}}$, where $||\left[\boldsymbol{\tau}^{\mathrm{s}}\right]_n-\boldsymbol{\tau}^{\mathrm{s}}||^2=1$ and $1\leq n\leq M$. Here, the SFF method first runs the local search with respect to $\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})$ to obtain the local minimum solution for~\eqref{eq:opt_prob_std_RIS_feb_27_2023}. To do so, we start from initial configuration $\boldsymbol{\tau}^{\mathrm{s}}$ and search among its neighbors to find $\boldsymbol{\tau}^{\mathrm{s}*}$ as a new solution that provides $\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})<\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})$ among all neighbors of $\boldsymbol{\tau}^{\mathrm{s}}$. We note that $\boldsymbol{\tau}^{\mathrm{s}}$ has $M$ neighbors. If $\boldsymbol{\tau}^{\mathrm{s}*}\neq \boldsymbol{\tau}^{\mathrm{s}}$, we set $\boldsymbol{\tau}^{\mathrm{s}}=\boldsymbol{\tau}^{\mathrm{s}*}$, and redo the above process. We define $i^{\text{loc}}$ to indicate the number of iterations that we use the local search process. The search ends if $i^{\text{loc}}$ reaches its maximum value (i.e., $i^{\text{loc}}_{\max}$) or there is no further improvement by running the search (i.e., $\boldsymbol{\tau}^{\mathrm{s}*}=\boldsymbol{\tau}^{\mathrm{s}}$). The details are demonstrated in Algorithm~\ref{algo:Local}. 
\begin{algorithm}
  \caption{Local Search}
  \begin{multicols}{2}
  
  \hspace*{\algorithmicindent} \textbf{Input:} $\boldsymbol{\tau}^{\mathrm{s}}$, $i_{\max}^{\text{loc}}$; \\ 
  \hspace*{\algorithmicindent} \textbf{Output:} $\boldsymbol{\tau}^{\mathrm{s}*}$;
  \begin{algorithmic}[1]
  \label{algo:Local}
  \STATE $i^{\text{loc}}=0$; $\boldsymbol{\tau}^{\mathrm{s}*}=\boldsymbol{\tau}^{\mathrm{s}}$;
  \FOR{ all $ \left[\boldsymbol{\tau}^{\mathrm{s}}\right]_n$ such that $||\left[\boldsymbol{\tau}^{\mathrm{s}}\right]_n-\boldsymbol{\tau}^{\mathrm{s}}||^2=1$}{
  \IF{$\bar{w}(\boldsymbol{\tau}^{\mathrm{s}}_n)< \bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})$}
  \STATE $\boldsymbol{\tau}^{\mathrm{s}*}=\left[\boldsymbol{\tau}^{\mathrm{s}}\right]_n$;
  \ENDIF
  }
  \ENDFOR
  \STATE $i^{\text{loc}} \leftarrow i^{\text{loc}}+1$;
  \IF{$\boldsymbol{\tau}^{\mathrm{s}*}\neq \boldsymbol{\tau}^{\mathrm{s}}$ and $i^{\text{loc}}\leq i_{\max}^{\text{loc}}$}
  \STATE $\boldsymbol{\tau}^{\mathrm{s}}=\boldsymbol{\tau}^{\mathrm{s}*}$;
  \STATE Go to line 2;
  \ELSE
  \STATE $\boldsymbol{\tau}^{\mathrm{s}*}$ is the local minimum solution. 
  \ENDIF
\end{algorithmic}
\end{multicols}
\vspace{-3mm}
\end{algorithm}



The issue with local search is that $\boldsymbol{\tau}^{\mathrm{s}*}$ depends on the initial choice of $\boldsymbol{\tau}^{\mathrm{s}}$. Thus, we use global search based on sigmoid filled function to move from $\boldsymbol{\tau}^{\mathrm{s}*}$ to another better solution. Here, we use our filled function, $W_r(\boldsymbol{\tau}^{\mathrm{s}},\boldsymbol{\tau}^{\mathrm{s}*})$, and define an auxiliary optimization problem as below:
\begin{align}
\label{eq:aux_opt}
    &\underset{\boldsymbol{\tau}^{\mathrm{s}}}{\min}~W_r(\boldsymbol{\tau}^{\mathrm{s}},\boldsymbol{\tau}^{\mathrm{s}*}) \nonumber \\
    &\text{s.t.} \quad \boldsymbol{\tau}^{\mathrm{s}},\boldsymbol{\tau}^{\mathrm{s}*}\in \{0,1\}^{M \times 1},
\end{align}
where $r$ denotes the heuristic optimization parameter, $\boldsymbol{\tau}^{\mathrm{s}*}$ is the current local minimum solution,
\begin{align}
\label{eq:filled_func}
    &W_r(\boldsymbol{\tau}^{\mathrm{s}},\boldsymbol{\tau}^{\mathrm{s}*})\nonumber\\
    &~~~~=(1+\frac{1}{1+\eta||\boldsymbol{\tau}^{\mathrm{s}}-\boldsymbol{\tau}^{\mathrm{s}*}||^2})q_r(\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})),
\end{align}
\begin{align}
\label{eq:parameters_filled_func}
&q_r(\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*}))\\ \nonumber
&=
\left\{ \begin{array}{ll}
\vspace{1mm} \bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})+r , & \bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})\leq -r, \\
\frac{1}{1+e^{\frac{-6}{r}(\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})+r/2)}}, & -r<\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})< 0,\\
1, & \bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})\geq 0,
\end{array} \right.
\end{align}
and
\begin{align}
    & \eta=
\left\{ \begin{array}{ll}
\vspace{1mm} 0, & \bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})\leq -r, \\
1, & \text{otherwise}.
\end{array} \right.
\end{align}

In this part, we use $i$ and $\boldsymbol{\tau}^{\mathrm{s}}_i$ to denote the $i^{\mathrm{th}}$ iteration of global search and the solution in the $i^{\mathrm{th}}$ iteration, respectively. Here, we start from an initial random solution,  $\boldsymbol{\tau}^{\mathrm{s}}_0$, and then apply Algorithm~\ref{algo:Local} to~\eqref{eq:opt_prob_std_RIS_feb_27_2023} to get $\boldsymbol{\tau}^{\mathrm{s}*}_0$. After finding $\boldsymbol{\tau}^{\mathrm{s}*}_0$, we run local search starting from $\boldsymbol{\tau}^{\mathrm{s}*}_0$ with respect to~\eqref{eq:aux_opt} to attain $\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_0$. Next, we assume $\boldsymbol{\tau}^{\mathrm{s}}_1=\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_0$. If $\bar{w}(\boldsymbol{\tau}^{\mathrm{s}}_1)<\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*}_0)$, we consider $\boldsymbol{\tau}^{\mathrm{s}}_1$ as a new solution and redo the above procedure. Else, we apply other neighbors of $\boldsymbol{\tau}^{\mathrm{s}*}_0$ to~\eqref{eq:aux_opt} to obtain a new $\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_0$ and repeat the above procedure. If neither $\boldsymbol{\tau}^{\mathrm{s}*}_0$ nor its neighbors can lead to a new solution, we reduce $r$ (e.g., $r=r/10$) to find a new filled function, and thus new $\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_0$ and then repeat the above search. Moreover, we use $\gamma \in \mathbb{N}$ to indicate that after $\gamma$ times of finding
the local minimizer of~\eqref{eq:aux_opt}, we
run local search for~\eqref{eq:opt_prob_std_RIS_feb_27_2023}. The search stops if $r< \epsilon, \epsilon\ll 1$ or $i^{\text{filled}}$, the number of times that we use the filled function, reaches its maximum value, $i^{\text{filled}}_{\max}$. In this case, we say that the current solution is an approximation of the global minimum solution.
%%-----------------%%



% It is important to note that the local search uses finite steps to find the local minimizer since there are $N^M$ possible solutions that are finite. 

\begin{algorithm}
  \caption{Global Search}
  \begin{multicols}{2}
  \hspace*{\algorithmicindent} \textbf{Input:} $\boldsymbol{\tau}^{\mathrm{s}}_0, r, \gamma, \epsilon, i_{\max}^{\text{loc}}, i_{\max}^{\text{filled}}$; 
  \hspace*{\algorithmicindent}\hspace{-0.4mm} \textbf{Output:} $\boldsymbol{\tau}^{\mathrm{s}**}$;
  \begin{algorithmic}[1]
  \label{algo:global}
  \STATE $i=0$; $r_0=r$; $\bar{\gamma}=\gamma$;
  \STATE $i^{\text{filled}}=0$;
  \STATE $\boldsymbol{\tau}^{\mathrm{s}**}=\boldsymbol{\tau}^{\mathrm{s}}_0$;
  \IF{$i+1\geq \bar{\gamma}$}
  \STATE $\bar{\gamma}\leftarrow\bar{\gamma}+\gamma$;
  \STATE Apply Algorithm~\ref{algo:Local} to $\boldsymbol{\tau}^{\mathrm{s}}_{i}$ and \eqref{eq:opt_prob_std_RIS_feb_27_2023} to get $\boldsymbol{\tau}^{\mathrm{s}*}_{i}$;
  \ELSE
  \STATE  $\boldsymbol{\tau}^{\mathrm{s}*}_{i}=\boldsymbol{\tau}^{\mathrm{s}}_{i}$;
  \ENDIF
  
  \IF{$i=0$ or $\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*}_{i})<\bar{w}(\boldsymbol{\tau}^{\mathrm{s}**})$ }
      \STATE $\boldsymbol{\tau}^{\mathrm{s}**}=\boldsymbol{\tau}^{\mathrm{s}*}_{i}$; $r=r_0$; 
      \STATE $m=1$;
      \STATE Apply Algorithm~\ref{algo:Local} to $\boldsymbol{\tau}^{\mathrm{s}*}_{i}$ and \eqref{eq:aux_opt} to obtain $\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_{i}$;
      \STATE $i^{\text{filled}} \leftarrow i^{\text{filled}}+1$
      \IF{$m=1$}
      \STATE $i\leftarrow i+1$;
      \STATE $\boldsymbol{\tau}^{\mathrm{s}}_{i}=\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_{i-1}$;
      \ELSE
      \STATE $\boldsymbol{\tau}^{\mathrm{s}}_{i}=\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_{i}$;
      \ENDIF
      \STATE Go to line 4;
  \ENDIF
  \IF{$m \leq M$}
      \STATE $\boldsymbol{\tau}^{\mathrm{s}*}_{i}=$ the $m^{\mathrm{th}}$ neighbor of $\boldsymbol{\tau}^{\mathrm{s}*}_{i-1}$;
      \STATE $m\leftarrow m+1$;
      \STATE Go to line 12;
  \ELSE
      \IF{$r<\epsilon$ or $i^{\text{filled}}>i_{\max}^{\text{filled}}$ }
           \STATE $\boldsymbol{\tau}^{\mathrm{s}**}$ is the global minimum solution.
          \ELSE
          \STATE $r \leftarrow \frac{r}{10}$;
          \STATE $i \leftarrow i-1$;
          \STATE Go to line 11;   
      \ENDIF
  \ENDIF
    \end{algorithmic}
    \end{multicols}
    \vspace{-3mm}
\end{algorithm}

In Section~\ref{Section:Num_results}, we will show that the SFF method outperforms the SBO method using S-RIS. 

In the second scenario based on \newwRIS, we need to update~\eqref{eq:opt_prob_std_RIS_feb_27_2023} using $\textbf{T}=\textbf{T}^{\mathrm{i}}$. Here, we use the SFF method by following Algorithms~\ref{algo:Local} and \ref{algo:global} since the filled function-based optimization methods solve a general non-convex problem as long as selecting a possible configuration from a discrete set is the only constraint~\cite{ng2005discrete}. On the contrary, the SBO method can not be directly applied to \newRIS due to the additional non-convexity that arises from dependence of $\bar{\mathcal{M}}^{[m]}$ on the current solution. This necessitates an additional approximation, which further degrades its performance. As a result, in the next section, we only utilize the SFF method for optimizing the I-RIS elements.




==> Sections/Sect3_Beamforming_design_USV_v0.tex <==
In this work, our goal is to apply a passive beamfroming through RIS elements to maximize sum-rate. Therefore, we formulate our optimization problem as below:
\begin{align}
\label{eq:opt_prob_std_RIS_feb_27_2023}
    &\underset{\mathbf{T}}{\max}\underbrace{\sum_{i=1}^{K} \log(1+\text{SINR}_i)}_{\overset{\triangle}=~-w(\mathbf{T})}\equiv \underset{\mathbf{T}}{\min}~w(\mathbf{T})\\ \nonumber
    &\text{s.t.} ~~\mathbf{T} \in \{\mathbf{T}^{s}, \mathbf{T}^g\},~~  s_m,s_{\ell m}\in\{0,1\},~~1\leq \ell,m\leq M.
\end{align}
The optimization problem in~\eqref{eq:opt_prob_std_RIS_feb_27_2023} is non-convex due to (i) the binary constraint, and (ii) the non-convex objective function. To optimize~\eqref{eq:opt_prob_std_RIS_feb_27_2023}, we first focus on the S-RIS where $\mathbf{T}=\mathbf{T}^{s}$ and propose two methods to solve the problem: (1) we use the SBO method, which converts~\eqref{eq:opt_prob_std_RIS_feb_27_2023} to a semi-definite convex problem and then solves the equivalent convex problem; (2) we utilize a heuristic method based on sigmoid filled function (i.e., the SFF method) to obtain an approximation of the global optimum solution. We provide further details below. 

\textbf{SBO method:} In this case, to address the non-convexity of the binary constraint, we use slack variable $\textbf{S}$ and rewrite the binary constraint as follows:
\begin{align}
\label{eq:Diag_S_feb_27_2023}
    \mathrm{Diag}(\textbf{S})=\boldsymbol{\tau}^{s}, 
\end{align}
\begin{align}
\label{eq:S=ss_feb_27_2023}
    \textbf{S}=\boldsymbol{\tau}^{s}{\boldsymbol{\tau}^{s}}^{\top},
\end{align}
\begin{align}
\label{eq:01_values_feb_27_2023}
    0 \leq s_m \leq 1,~\text{and}~0 \leq S_{\ell m} \leq 1,~~ \text{for}~ 1\leq \ell,m \leq M,
\end{align}
where $S_{\ell m}$ is an element located at the $\ell^{\mathrm{th}}$ row and the $m^{\mathrm{th}}$ column of $\textbf{S}$. Here, \eqref{eq:S=ss_feb_27_2023} is non-convex. In~\cite{guo2018new,hu2021robust}, the authors show that \eqref{eq:S=ss_feb_27_2023} can be substituted with the following conditions.
\begin{align}
\label{eq:Y_matrix_feb_27_2023}
    \textbf{Y}=\begin{bmatrix}
        \textbf{S}& \boldsymbol{\tau}^{s}\\
        {\boldsymbol{\tau}^{s}}^{\top}& 1\\
    \end{bmatrix}\succeq \mathbf{0},~~\text{and} ~~ \text{Rank}(\textbf{Y})=1,
\end{align}
where $\textbf{Y} \succeq \mathbf{0}$ means $\textbf{Y}$ is a positive semi-definite matrix. Since $\textbf{Y}$ includes binary elements, the rank of $\textbf{Y}$ is equal to one for any binary vector $\boldsymbol{\tau}^{s}$. Therefore, we define $\textbf{G}^{[ij]}\overset{\triangle}=\textbf{g}^{[i]} \mathrm{diag}(\textbf{h}^{[j]})$ and $\bar{\textbf{G}}^{[ij]}\overset{\triangle}=\textbf{G}^{[ij]}{\textbf{G}^{[ij]}}^{\textrm{H}}$ and use \eqref{eq:Diag_S_feb_27_2023}, \eqref{eq:01_values_feb_27_2023}, and \eqref{eq:Y_matrix_feb_27_2023} to rewrite~\eqref{eq:opt_prob_std_RIS_feb_27_2023} as a semi-definite relaxation (SDR) problem as follows:
\begin{align}
\label{eq:finalswitch_SNR_feb_27_2023}
    &\underset{\boldsymbol{\tau}^{s},\textbf{S} }{\min}~-\sum_{i=1}^K\log\left(1+\frac{P_i~\mathrm{tr}\left(\textbf{S}\bar{\textbf{G}}^{[ii]}\right)}{\sigma^2+\sum_{j=1,j\neq i}^K P_j~\mathrm{tr}\left(\textbf{S}\bar{\textbf{G}}^{[ij]}\right) }\right)\\ \nonumber
    &\text{s.t.} ~~ \mathrm{Diag}(\textbf{S})=\boldsymbol{\tau}^{s}, \\ \nonumber 
    & ~~~~~~\textbf{Y}\succeq \mathbf{0}, \\ \nonumber 
    & ~~~~~~0 \leq s_m \leq 1,~~0 \leq S_{\ell m} \leq 1,~~ \text{for}~ 1\leq \ell,m \leq M.
\end{align}

Then, we use the feature of a logarithmic function and rewrite~\eqref{eq:finalswitch_SNR_feb_27_2023} as below:
\begin{align}
\label{eq:finalswitch_SINR_Dbi_Nbi_feb_27_2023}
    &\underset{\boldsymbol{\tau}^{s},\textbf{S} }{\min}~N-D\\ \nonumber
    &\text{s.t.} ~~ \mathrm{Diag}(\textbf{S})=\boldsymbol{\tau}^{s}, \\ \nonumber 
    & ~~~~~~\textbf{Y}\succeq \mathbf{0}, \\ \nonumber 
    & ~~~~~~0 \leq s_m \leq 1,~~0 \leq S_{\ell m} \leq 1,~~ \text{for}~ 1\leq \ell,m \leq M,
\end{align}
where
\begin{align}
    \label{eq:SINR_noise_Nbi_feb_27_2023}
    N=-\sum_{i=1}^K\log\left(\sigma^2+\sum_{j=1}^K P_i~\mathrm{tr}\left(\textbf{S}\bar{\textbf{G}}^{[ij]}\right)\right),
\end{align}
and
\begin{align}
    \label{eq:SINR_noise_Dbi_feb_27_2023}
    D=-\sum_{i=1}^K\log\left(\sigma^2+\sum_{j=1, j\neq i}^K P_j~\mathrm{tr}\left(\textbf{S}\bar{\textbf{G}}^{[ij]}\right)\right).
\end{align}

Based on \eqref{eq:SINR_noise_Nbi_feb_27_2023} and \eqref{eq:SINR_noise_Dbi_feb_27_2023}, $N$ and $D$ are convex with respect to $\textbf{S}$; thus,~\eqref{eq:finalswitch_SINR_Dbi_Nbi_feb_27_2023} falls under the difference of convex (DC) optimization problem. To solve this problem, we use the SCA method, which is an iterative approach that runs for $I_{tr}$ times. To do so, we apply the first-order Taylor approximation to $D$ and obtain a lower bound on that as follows:
\begin{align}
\label{eq:lower_bound_Dbi_formula_feb_27_2023}
    D(\textbf{S})\geq D\left(\textbf{S}^t\right)+\nabla^{\top}_{\textbf{S}}\left(D\left(\textbf{S}^t\right)\right)\left(\textbf{S}-\textbf{S}^t\right),
\end{align}
where $\textbf{S}^t$ is the value of $\textbf{S}$ in the $t^{\mathrm{th}}$ iteration and 
\begin{align}
\label{eq:lower_bound_Dbi_feb_27_2023}
    \nabla^{\top}_{\textbf{S}}\left(D\left(\textbf{S}^t\right)\right)=-\frac{1}{\mathrm{ln}~2}\sum_{i=1}^K\frac{\sum_{j=1, j\neq i}^K P_j\bar{\textbf{G}}^{[ij]}}{\sigma^2+\sum_{j=1, j\neq i}^K P_j~\mathrm{tr}\left(\textbf{S}^t\bar{\textbf{G}}^{[ij]}\right)}.
\end{align} 

By applying \eqref{eq:lower_bound_Dbi_formula_feb_27_2023} to \eqref{eq:finalswitch_SINR_Dbi_Nbi_feb_27_2023}, we obtain a convex SDR problem that can be solved with the CVX Toolbox in MATLAB~\cite{grant2011matlab}.

\textbf{SFF method:} As the heuristic method is one type of the approaches to solve the non-convex problems, we utilize the SFF method based on sigmoid filled function to solve the problem in~\eqref{eq:opt_prob_std_RIS_feb_27_2023}. This method includes two steps as local and global search. Prior to explain the details, we need to define $\boldsymbol{\tau}^{s}_n\in \{0,1\}^{M \times 1}$ as a neighbor of $\boldsymbol{\tau}^{s}$, where $||\boldsymbol{\tau}^{s}_n-\boldsymbol{\tau}^{s}||^2=1$. Then, to run the local search with respect $w(\textbf{T}^s)=\bar{w}(\boldsymbol{\tau}^{s})$, we start from a random initial configuration, $\boldsymbol{\tau}^{s}_0$, and search among its neighbors to find $\boldsymbol{\tau}^{s*}_0$ as a new solution that provides the maximum gain among all neighbors of $\boldsymbol{\tau}^{s}_0$. If $\boldsymbol{\tau}^{s*}_0\neq \boldsymbol{\tau}^{s}_0$, we set $\boldsymbol{\tau}^{s}_0=\boldsymbol{\tau}^{s*}_0$, and redo the process; else, we declare $\boldsymbol{\tau}^{s*}_0$ as the optimal local solution. We define $i^{\text{loc}}$ to indicate the number of iterations that we use the local search process. The search ends if $i^{\text{loc}}$ reaches its maximum value (i.e., $i^{\text{loc}}_{\max}$) or there is no further improvement by running the search. The details are demonstrated in Algorithm~\ref{algo:Local}. 
\begin{algorithm}
  \caption{Local Search}
  \begin{multicols}{2}
  
  \hspace*{\algorithmicindent} \textbf{Input:} $\boldsymbol{\tau}^{s}_0$, $i_{\max}^{\text{loc}}$; \\ 
  \hspace*{\algorithmicindent} \textbf{Output:} $\boldsymbol{\tau}^{s*}_0$;
  \begin{algorithmic}[1]
  \label{algo:Local}
  \STATE $i^{\text{loc}}=0$; $\boldsymbol{\tau}^{s*}=\boldsymbol{\tau}^{s}_0$;
  \FOR{$\forall \boldsymbol{\tau}^{s}_n\hspace{-1mm}:\hspace{-1mm}||\boldsymbol{\tau}^{s}_n=\boldsymbol{\tau}^{s}_0||^2=1$}{
  \IF{$\bar{w}(\boldsymbol{\tau}^{s}_n)\leq \bar{w}(\boldsymbol{\tau}^{s}_0)$}
  \STATE $\boldsymbol{\tau}^{s*}_0=\boldsymbol{\tau}^{s}_n$;
  \ENDIF
  }
  \ENDFOR
  \STATE $i^{\text{loc}} \leftarrow i^{\text{loc}}+1$;
  \IF{$\boldsymbol{\tau}^{s*}_0\neq \boldsymbol{\tau}^{s}_0$ and $i^{\text{loc}}\leq i_{\max}^{\text{loc}}$}
  \STATE $\boldsymbol{\tau}^{s}_0=\boldsymbol{\tau}^{s*}_0$;
  \STATE Go to line 2;
  \ELSE
  \STATE The local minimum is equal to $\boldsymbol{\tau}^{s*}_0$ 
  \ENDIF
\end{algorithmic}
\end{multicols}
\end{algorithm}



The issue with local search is that $\boldsymbol{\tau}^{s*}_0$ depends on the initial choice of $\boldsymbol{\tau}^{s}_0$. Thus, we use global search based on sigmoid filled function to move from $\boldsymbol{\tau}^{s*}_0$ to another better solution. To do so, we first define our filled function as below:
\begin{align}
\label{eq:aux_opt}
    &\underset{\boldsymbol{\tau}^{s}}{\min}~W_r(\boldsymbol{\tau}^{s},\boldsymbol{\tau}^{s*}) \nonumber \\
    &\text{s.t.} \quad \boldsymbol{\tau}^{s},\boldsymbol{\tau}^{s*}\in \{0,1\}^{M \times 1},
\end{align}
where $r$ denotes the heuristic optimization parameter, $\boldsymbol{\tau}^{s*}$ is the current local minimum,
\begin{align}
\label{eq:filled_func}
    &W_r(\boldsymbol{\tau}^{s},\boldsymbol{\tau}^{s*})\nonumber\\
    &~~~~=(1+\frac{1}{1+\eta||\boldsymbol{\tau}^{s}-\boldsymbol{\tau}^{s*}||^2})q_r(\bar{w}(\boldsymbol{\tau}^{s})-\bar{w}(\boldsymbol{\tau}^{s*})),
\end{align}
\begin{align}
\label{eq:parameters_filled_func}
&q_r(\bar{w}(\boldsymbol{\tau}^{s})-\bar{w}(\boldsymbol{\tau}^{s*}))\\ \nonumber
&=
\left\{ \begin{array}{ll}
\vspace{1mm} \bar{w}(\boldsymbol{\tau}^{s})-\bar{w}(\boldsymbol{\tau}^{s*})+r , & \bar{w}(\boldsymbol{\tau}^{s})-\bar{w}(\boldsymbol{\tau}^{s*})\leq -r, \\
\frac{1}{1+e^{\frac{-6}{r}(\bar{w}(\boldsymbol{\tau}^{s})-\bar{w}(\boldsymbol{\tau}^{s*})+r/2)}}, & -r<\bar{w}(\boldsymbol{\tau}^{s})-\bar{w}(\boldsymbol{\tau}^{s*})< 0,\\
1, & \bar{w}(\boldsymbol{\tau}^{s})-\bar{w}(\boldsymbol{\tau}^{s*})\geq 0,
\end{array} \right.
\end{align}
and
\begin{align}
    & \eta=
\left\{ \begin{array}{ll}
\vspace{1mm} 0, & \bar{w}(\boldsymbol{\tau}^{s})-\bar{w}(\boldsymbol{\tau}^{s*})\leq -r, \\
1, & \text{otherwise}.
\end{array} \right.
\end{align}

After finding $\boldsymbol{\tau}^{s*}_0$ through Algorithm~\ref{algo:Local}, we run local search starting from $\boldsymbol{\tau}^{s*}_0$ with respect to~\eqref{eq:aux_opt} to attain $\bar{\boldsymbol{\tau}}^{s*}_0$. If $\bar{w}(\bar{\boldsymbol{\tau}}^{s*}_0)<\bar{w}(\boldsymbol{\tau}^{s*}_0)$, we consider $\boldsymbol{\tau}^{s}_0=\bar{\boldsymbol{\tau}}^{s*}_0$ and redo the above procedure. Otherwise, we reduce $r$ (e.g., $r=r/10$) and find a new filled function, and thus new $\bar{\boldsymbol{\tau}}^{s*}_0$ and then repeat the above search. Moreover, we define: (1) $\gamma \in \mathbb{N}$ to indicate after $\gamma$ times of finding
the local minimizer of~\eqref{eq:aux_opt}, we
run local search for~\eqref{eq:opt_prob_std_RIS_feb_27_2023}; (2) $i$ to denote the $i^{\mathrm{th}}$ solution. Then, we reduce $r$ if $r\geq \epsilon, \epsilon\ll 1$ and $i^{\text{filled}}$, the number of times that we use the filled function, does not reach its maximum value, $i^{\text{filled}}_{\max}$, and continue the search process. Otherwise, we say that the current optimal solution is an approximation of the global optimal solution.
%%-----------------%%



% It is important to note that the local search uses finite steps to find the local minimizer since there are $N^M$ possible solutions that are finite. 

\begin{algorithm}
  \caption{Global Search}
  \begin{multicols}{2}
  \hspace*{\algorithmicindent} \textbf{Input:} $\boldsymbol{\tau}^{s}_0, r, \gamma, \epsilon, i_{\max}^{\text{loc}}, i_{\max}^{\text{filled}}$; 
  \hspace*{\algorithmicindent}\hspace{-0.4mm} \textbf{Output:} $\boldsymbol{\tau}^{s**}$;
  \begin{algorithmic}[1]
  \label{algo:global}
  \STATE $i=0$; $r_0=r$; $\bar{\gamma}=\gamma$;
  \STATE $i^{\text{filled}}=0$;
  \STATE $\boldsymbol{\tau}^{s**}=\boldsymbol{\tau}^{s}_0$;
  \IF{$i+1\geq \bar{\gamma}$}
  \STATE $\bar{\gamma}\leftarrow\bar{\gamma}+\gamma$;
  \STATE Apply Algorithm~\ref{algo:Local} to $\boldsymbol{\tau}^{s}_{i}$ and \eqref{eq:opt_prob_std_RIS_feb_27_2023} to get $\boldsymbol{\tau}^{s*}_{i}$;
  \ELSE
  \STATE  $\boldsymbol{\tau}^{s*}_{i}=\boldsymbol{\tau}^{s}_{i}$;
  \ENDIF
  
  \IF{$i=0$ or $\bar{w}(\boldsymbol{\tau}^{s*}_{i})<\bar{w}(\boldsymbol{\tau}^{s**})$ }
      \STATE $\boldsymbol{\tau}^{s**}=\boldsymbol{\tau}^{s*}_{i}$; $r=r_0$; 
      \STATE $m=1$;
      \STATE Apply Algorithm~\ref{algo:Local} to $\boldsymbol{\tau}^{s*}_{i}$ and \eqref{eq:aux_opt} to obtain $\bar{\boldsymbol{\tau}}^{s*}_{i}$;
      \STATE $i^{\text{filled}} \leftarrow i^{\text{filled}}+1$
      \IF{$m=1$}
      \STATE $i\leftarrow i+1$;
      \STATE $\boldsymbol{\tau}^{s}_{i}=\bar{\boldsymbol{\tau}}^{s*}_{i-1}$;
      \ELSE
      \STATE $\boldsymbol{\tau}^{s}_{i}=\bar{\boldsymbol{\tau}}^{s*}_{i}$;
      \ENDIF
      \STATE Go to line 4;
  \ENDIF
  \IF{$m \leq M$}
      \STATE $\boldsymbol{\tau}^{s*}_{i}=$ the $m^{\mathrm{th}}$ neighbor of $\boldsymbol{\tau}^{s*}_{i-1}$;
      \STATE $m\leftarrow m+1$;
      \STATE Go to line 12;
  \ELSE
      \IF{$r<\epsilon$ or $i^{\text{filled}}>i_{\max}^{\text{filled}}$ }
           \STATE $\boldsymbol{\tau}^{s**}$ is the global minimizer.
          \ELSE
          \STATE $r \leftarrow \frac{r}{10}$;
          \STATE $i \leftarrow i-1$;
          \STATE Go to line 11;   
      \ENDIF
  \ENDIF
    \end{algorithmic}
    \end{multicols}
\end{algorithm}

In Section~\ref{Section:Num_results}, we will show that the SFF method outperforms the SBO method in terms of complexity and sum-rate. Therefore, we only apply the SFF method to optimize~\eqref{eq:opt_prob_std_RIS_feb_27_2023} based on the generalized RIS. On the other hand,~\cite{ng2005discrete} claims that the filled function-based optimization methods optimize a general nonlinear objective function as long as selecting a possible configuration from a discrete set is the only constraint, while the SBO method can not be directly applied to the G-RIS. As a result, we update~\eqref{eq:opt_prob_std_RIS_feb_27_2023} using $\textbf{T}^g$ and follow Algorithm~\ref{algo:Local} and~\ref{algo:global} to obtain the optimal solution.



==> Sections/Sect3_Beamforming_design_v1.tex <==
We aim to optimize RIS elements to maximize the sum-rate; thus, we formulate our optimization problem as:
\begin{align}
\label{eq:opt_prob_std_RIS_feb_27_2023}
    &\underset{\mathbf{T}}{\max}\underbrace{\sum_{\gidx=1}^{K} \log(1+\text{SINR}_{\gidx})}_{\overset{\triangle}=~-w(\mathbf{T})}\equiv \underset{\mathbf{T}}{\min}~w(\mathbf{T})\\ \nonumber
    &\text{s.t.} ~~\mathbf{T} \in \{\mathbf{T}^{\mathrm{s}}, \mathbf{T}^{\mathrm{i}}\},~~  s_m,s_{\ell, m}\in\{0,1\},~~1\leq \ell,m\leq M,
\end{align}
which is non-convex due to the binary constraints and the non-convex objective function. To optimize~\eqref{eq:opt_prob_std_RIS_feb_27_2023}, we first focus on S-RIS where $\mathbf{T}=\mathbf{T}^{\mathrm{s}}$ and propose two methods to solve the problem: (1) we use the %\avc{write out the full name again} 
semi-definite binary optimization (SBO) method, which converts~\eqref{eq:opt_prob_std_RIS_feb_27_2023} to a semi-definite relaxation (SDR) problem and then solves the equivalent convex problem; (2) we utilize the sigmoid filled function (SFF), which is a heuristic method based on filled function that directly targets \eqref{eq:opt_prob_std_RIS_feb_27_2023} to obtain an approximation of the global optimum solution. We provide further details below. 

\textbf{SBO method:} In this case, to address the non-convexity of the binary constraints, we use slack variable $\textbf{S}$ and rewrite the binary constraint as follows:
% \begin{align}
% \label{eq:Diag_S_feb_27_2023}
%     \mathrm{Diag}(\textbf{S})=\boldsymbol{\tau}^{\mathrm{s}}, 
% \end{align}
% \begin{align}
% \label{eq:S=ss_feb_27_2023}
%     \textbf{S}=\boldsymbol{\tau}^{\mathrm{s}}{\boldsymbol{\tau}^{\mathrm{s}}}^{\top},
% \end{align}


\begin{minipage}[ht]{0.5\linewidth}
\begin{equation}
\label{eq:Diag_S_feb_27_2023}
    \mathrm{Diag}(\textbf{S})=\boldsymbol{\tau}^{\mathrm{s}}, \quad \quad \quad
\end{equation}
\end{minipage}
 % Adjust the spacing between equations
\begin{minipage}[ht]{0.44\linewidth}
\begin{equation}
\label{eq:S=ss_feb_27_2023}
 \textbf{S}=\boldsymbol{\tau}^{\mathrm{s}}{\boldsymbol{\tau}^{\mathrm{s}}}^{\top},\quad \quad
\end{equation}
\end{minipage}



\begin{align}
\label{eq:01_values_feb_27_2023}
    0 \leq s_m \leq 1,~\text{and}~0 \leq S_{\ell, m} \leq 1,~~ \text{for}~ 1\leq \ell,m \leq M,
\end{align}
where $S_{\ell, m}$ is the element in the $\ell^{\mathrm{th}}$ row and $m^{\mathrm{th}}$ column of $\textbf{S}$. Here, \eqref{eq:S=ss_feb_27_2023} is non-convex; therefore, we substitute it with the following conditions~\cite{guo2018new,hu2021robust}.
\begin{align}
\label{eq:Y_matrix_feb_27_2023}
    \textbf{Y}=\begin{bmatrix}
        \textbf{S}& \boldsymbol{\tau}^{\mathrm{s}}\\
        {\boldsymbol{\tau}^{\mathrm{s}}}^{\top}& 1\\
    \end{bmatrix}\succeq \mathbf{0},~~\text{and} ~~ \text{Rank}(\textbf{Y})=1.
\end{align}

Since $\textbf{Y}$ includes binary elements, the rank of $\textbf{Y}$ is equal to one for any binary feasible solution. Next, we define $\textbf{G}^{[\gidx j]}\overset{\triangle}=\textbf{g}^{[\gidx]} \mathrm{diag}(\textbf{h}^{[j]})$ and $\bar{\textbf{G}}^{[\gidx j]}\overset{\triangle}=\textbf{G}^{[\gidx j]}{\textbf{G}^{[\gidx j]}}^{\textrm{H}}$ and use \eqref{eq:Diag_S_feb_27_2023}, \eqref{eq:01_values_feb_27_2023}, and \eqref{eq:Y_matrix_feb_27_2023} to rewrite~\eqref{eq:opt_prob_std_RIS_feb_27_2023} as an SDR problem as follows:
\begin{align}
\label{eq:finalswitch_SNR_feb_27_2023}
    &\underset{\boldsymbol{\tau}^{\mathrm{s}},\textbf{S} }{\min}~-\sum_{\gidx=1}^K\log\left(1+\frac{P_{\gidx}~\mathrm{tr}\left(\textbf{S}\bar{\textbf{G}}^{[\gidx \gidx ]}\right)}{\sigma^2+\sum_{j=1,j\neq \gidx}^K P_j~\mathrm{tr}\left(\textbf{S}\bar{\textbf{G}}^{[\gidx j]}\right) }\right)\\ \nonumber
    &\text{s.t.} ~~ \mathrm{Diag}(\textbf{S})=\boldsymbol{\tau}^{\mathrm{s}}, \quad \textbf{Y}\succeq \mathbf{0}, \\ \nonumber 
    & ~~~~~~0 \leq s_m \leq 1,~~0 \leq S_{\ell, m} \leq 1,~~ \text{for}~ 1\leq \ell,m \leq M.
\end{align}

Then, we use the feature of a logarithmic function and rewrite~\eqref{eq:finalswitch_SNR_feb_27_2023} as:
\begin{align}
\label{eq:finalswitch_SINR_Dbi_Nbi_feb_27_2023}
    &\underset{\boldsymbol{\tau}^{\mathrm{s}},\textbf{S} }{\min}~N-D\\ \nonumber
    &\text{s.t.} ~~ \mathrm{Diag}(\textbf{S})=\boldsymbol{\tau}^{\mathrm{s}}, \quad \textbf{Y}\succeq \mathbf{0}, \\ \nonumber 
    & ~~~~~~0 \leq s_m \leq 1,~~0 \leq S_{\ell, m} \leq 1,~~ \text{for}~ 1\leq \ell,m \leq M,
\end{align}
where
\begin{align}
    \label{eq:SINR_noise_Nbi_feb_27_2023}
    N=-\sum_{\gidx=1}^K\log\left(\sigma^2+\sum_{j=1}^K P_{j}~\mathrm{tr}\left(\textbf{S}\bar{\textbf{G}}^{[\gidx j]}\right)\right),
\end{align}
and
\begin{align}
    \label{eq:SINR_noise_Dbi_feb_27_2023}
    D=-\sum_{\gidx=1}^K\log\left(\sigma^2+\sum_{j=1, j\neq \gidx}^K P_j~\mathrm{tr}\left(\textbf{S}\bar{\textbf{G}}^{[\gidx j]}\right)\right).
\end{align}

Based on \eqref{eq:SINR_noise_Nbi_feb_27_2023} and \eqref{eq:SINR_noise_Dbi_feb_27_2023}, $N$ and $D$ are convex with respect to $\textbf{S}$; thus,~\eqref{eq:finalswitch_SINR_Dbi_Nbi_feb_27_2023} falls under the difference of convex (DC) optimization problem. To solve this problem, we use the SCA method, which is an iterative approach that runs for $I_{\mathrm{tr}}$ times. To do so, we apply the first-order Taylor approximation to $D$ and obtain a lower bound on that as follows:
\begin{align}
\label{eq:lower_bound_Dbi_formula_feb_27_2023}
    D(\textbf{S})\geq D\left(\textbf{S}^t\right)+\nabla^{\top}_{\textbf{S}}\left(D\left(\textbf{S}^t\right)\right)\left(\textbf{S}-\textbf{S}^t\right),
\end{align}
where $\textbf{S}^t$ is the value of $\textbf{S}$ in the $t^{\mathrm{th}}$ iteration and 
\begin{align}
\label{eq:lower_bound_Dbi_feb_27_2023}
    \nabla^{\top}_{\textbf{S}}\left(D\left(\textbf{S}^t\right)\right)=-\frac{1}{\mathrm{ln}~2}\sum_{\gidx=1}^K\frac{\sum_{j=1, j\neq \gidx}^K P_j\bar{\textbf{G}}^{[\gidx j]}}{\sigma^2+\sum_{j=1, j\neq \gidx}^K P_j~\mathrm{tr}\left(\textbf{S}^t\bar{\textbf{G}}^{[\gidx j]}\right)}.
\end{align} 

By applying \eqref{eq:lower_bound_Dbi_formula_feb_27_2023} to \eqref{eq:finalswitch_SINR_Dbi_Nbi_feb_27_2023}, we obtain a convex SDR problem and solve it using CVX Toolbox in MATLAB~\cite{grant2011matlab}.

\textbf{SFF method:} Heuristic optimization methods (e.g., genetic algorithm and filled function) are popular for optimizing non-convex problems. Unlike the SBO method, a heuristic method directly tackles the non-convex problem in~\eqref{eq:opt_prob_std_RIS_feb_27_2023} without needing approximations for a convex equivalent. This avoids the performance degradation associated with the approximations used in the SBO method. Hence, we utilize the SFF method based on sigmoid filled function~\cite{nassirpour2022power} as our second optimization method in this paper to solve~\eqref{eq:opt_prob_std_RIS_feb_27_2023}. This method includes two steps: local and global search. Prior to explaining the details, we need to define: (i) $\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})\overset{\triangle}=w(\textbf{T}^{\mathrm{s}})$, and (ii) $\left[\boldsymbol{\tau}^{\mathrm{s}}\right]_n\in \{0,1\}^{M \times 1}$ as the $n^{\mathrm{th}}$ neighbor of $\boldsymbol{\tau}^{\mathrm{s}}$, where $||\left[\boldsymbol{\tau}^{\mathrm{s}}\right]_n-\boldsymbol{\tau}^{\mathrm{s}}||^2=1$ and $1\leq n\leq M$. Here, the SFF method first runs the local search with respect to $\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})$ to obtain the local minimum solution for~\eqref{eq:opt_prob_std_RIS_feb_27_2023}. To do so, we start from initial configuration $\boldsymbol{\tau}^{\mathrm{s}}$ and search among its neighbors to find $\boldsymbol{\tau}^{\mathrm{s}*}$ as a new solution that provides $\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})<\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})$. We note that $\boldsymbol{\tau}^{\mathrm{s}}$ has $M$ neighbors. If $\boldsymbol{\tau}^{\mathrm{s}*}\neq \boldsymbol{\tau}^{\mathrm{s}}$, we set $\boldsymbol{\tau}^{\mathrm{s}}=\boldsymbol{\tau}^{\mathrm{s}*}$, and redo the above process. We define $i^{\text{loc}}$ to indicate the number of iterations that we use the local search process. The search ends if $i^{\text{loc}}$ reaches its maximum value (i.e., $i^{\text{loc}}_{\max}$) or there is no further improvement by running the search (i.e., $\boldsymbol{\tau}^{\mathrm{s}*}=\boldsymbol{\tau}^{\mathrm{s}}$). The details are demonstrated in Algorithm~\ref{algo:Local}. 
\begin{algorithm}
  \caption{Local Search}
  \begin{multicols}{2}
  
  \hspace*{\algorithmicindent} \textbf{Input:} $\boldsymbol{\tau}^{\mathrm{s}}$, $i_{\max}^{\text{loc}}$; \\ 
  \hspace*{\algorithmicindent} \textbf{Output:} $\boldsymbol{\tau}^{\mathrm{s}*}$;
  \begin{algorithmic}[1]
  \label{algo:Local}
  \STATE $i^{\text{loc}}=0$; $\boldsymbol{\tau}^{\mathrm{s}*}=\boldsymbol{\tau}^{\mathrm{s}}$;
  \FOR{ all $ \left[\boldsymbol{\tau}^{\mathrm{s}}\right]_n$ such that $||\left[\boldsymbol{\tau}^{\mathrm{s}}\right]_n-\boldsymbol{\tau}^{\mathrm{s}}||^2=1$}{
  \IF{$\bar{w}(\boldsymbol{\tau}^{\mathrm{s}}_n)< \bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})$}
  \STATE $\boldsymbol{\tau}^{\mathrm{s}*}=\left[\boldsymbol{\tau}^{\mathrm{s}}\right]_n$;
  \ENDIF
  }
  \ENDFOR
  \STATE $i^{\text{loc}} \leftarrow i^{\text{loc}}+1$;
  \IF{$\boldsymbol{\tau}^{\mathrm{s}*}\neq \boldsymbol{\tau}^{\mathrm{s}}$ and $i^{\text{loc}}\leq i_{\max}^{\text{loc}}$}
  \STATE $\boldsymbol{\tau}^{\mathrm{s}}=\boldsymbol{\tau}^{\mathrm{s}*}$;
  \STATE Go to line 2;
  \ELSE
  \STATE $\boldsymbol{\tau}^{\mathrm{s}*}$ is the local minimum solution. 
  \ENDIF
\end{algorithmic}
\end{multicols}
\vspace{-3mm}
\end{algorithm}



The output of local search (i.e., $\boldsymbol{\tau}^{\mathrm{s}*}$) depends on the initial choice of $\boldsymbol{\tau}^{\mathrm{s}}$. Thus, we use global search based on sigmoid filled function to move from $\boldsymbol{\tau}^{\mathrm{s}*}$ to another better solution. Here, we use our filled function, $W_r(\boldsymbol{\tau}^{\mathrm{s}},\boldsymbol{\tau}^{\mathrm{s}*})$, and define an auxiliary optimization problem as below:
\begin{align}
\label{eq:aux_opt}
    &\underset{\boldsymbol{\tau}^{\mathrm{s}}}{\min}~W_r(\boldsymbol{\tau}^{\mathrm{s}},\boldsymbol{\tau}^{\mathrm{s}*}) \nonumber \\
    &\text{s.t.} \quad \boldsymbol{\tau}^{\mathrm{s}},\boldsymbol{\tau}^{\mathrm{s}*}\in \{0,1\}^{M \times 1},
\end{align}
where $r$ denotes the heuristic optimization parameter, $\boldsymbol{\tau}^{\mathrm{s}*}$ is the current local minimum solution,
\begin{align}
\label{eq:filled_func}
    &W_r(\boldsymbol{\tau}^{\mathrm{s}},\boldsymbol{\tau}^{\mathrm{s}*})\nonumber\\
    &~~~~=(1+\frac{1}{1+\eta||\boldsymbol{\tau}^{\mathrm{s}}-\boldsymbol{\tau}^{\mathrm{s}*}||^2})q_r(\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})),
\end{align}
\begin{align}
\label{eq:parameters_filled_func}
&q_r(\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*}))\\ \nonumber
&=
\left\{ \begin{array}{ll}
\vspace{1mm} \bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})+r , & \bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})\leq -r, \\
\frac{1}{1+e^{\frac{-6}{r}(\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})+r/2)}}, & -r<\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})< 0,\\
1, & \bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})\geq 0,
\end{array} \right.
\end{align}
and
\begin{align}
    & \eta=
\left\{ \begin{array}{ll}
\vspace{1mm} 0, & \bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})\leq -r, \\
1, & \text{otherwise}.
\end{array} \right.
\end{align}

In this part, we use $i$ and $\boldsymbol{\tau}^{\mathrm{s}}_i$ to denote the $i^{\mathrm{th}}$ iteration of global search and the solution in the $i^{\mathrm{th}}$ iteration, respectively. Here, we start from an initial random solution,  $\boldsymbol{\tau}^{\mathrm{s}}_0$, and then apply Algorithm~\ref{algo:Local} to~\eqref{eq:opt_prob_std_RIS_feb_27_2023} to get $\boldsymbol{\tau}^{\mathrm{s}*}_0$. After finding $\boldsymbol{\tau}^{\mathrm{s}*}_0$, we run local search starting from $\boldsymbol{\tau}^{\mathrm{s}*}_0$ with respect to~\eqref{eq:aux_opt} to attain $\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_0$. Next, we assume $\boldsymbol{\tau}^{\mathrm{s}}_1=\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_0$. If $\bar{w}(\boldsymbol{\tau}^{\mathrm{s}}_1)<\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*}_0)$, we consider $\boldsymbol{\tau}^{\mathrm{s}}_1$ as a new solution and redo the above procedure. Else, we apply other neighbors of $\boldsymbol{\tau}^{\mathrm{s}*}_0$ to~\eqref{eq:aux_opt} to obtain a new $\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_0$ and repeat the above procedure. If neither $\boldsymbol{\tau}^{\mathrm{s}*}_0$ nor its neighbors can lead to a new solution, we reduce $r$ (e.g., $r=r/10$) to find a new filled function, and thus new $\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_0$ and then repeat the above search. Moreover, we use $\gamma \in \mathbb{N}$ to indicate that after $\gamma$ times of finding
the local minimizer of~\eqref{eq:aux_opt}, we
run local search for~\eqref{eq:opt_prob_std_RIS_feb_27_2023}. The search stops if $r< \epsilon, \epsilon\ll 1$ or $i^{\text{filled}}$, the number of times that we use the filled function, reaches its maximum value, $i^{\text{filled}}_{\max}$. In this case, we say that the current solution is an approximation of the global minimum solution.
%%-----------------%%



% It is important to note that the local search uses finite steps to find the local minimizer since there are $N^M$ possible solutions that are finite. 

\begin{algorithm}
  \caption{Global Search}
  \begin{multicols}{2}
  \hspace*{\algorithmicindent} \textbf{Input:} $\boldsymbol{\tau}^{\mathrm{s}}_0, r, \gamma, \epsilon, i_{\max}^{\text{loc}}, i_{\max}^{\text{filled}}$; 
  \hspace*{\algorithmicindent}\hspace{-0.4mm} \textbf{Output:} $\boldsymbol{\tau}^{\mathrm{s}**}$;
  \begin{algorithmic}[1]
  \label{algo:global}
  \STATE $i=0$; $r_0=r$; $\bar{\gamma}=\gamma$;
  \STATE $i^{\text{filled}}=0$;
  \STATE $\boldsymbol{\tau}^{\mathrm{s}**}=\boldsymbol{\tau}^{\mathrm{s}}_0$;
  \IF{$i+1\geq \bar{\gamma}$}
  \STATE $\bar{\gamma}\leftarrow\bar{\gamma}+\gamma$;
  \STATE Apply Algorithm~\ref{algo:Local} to $\boldsymbol{\tau}^{\mathrm{s}}_{i}$ and \eqref{eq:opt_prob_std_RIS_feb_27_2023} to get $\boldsymbol{\tau}^{\mathrm{s}*}_{i}$;
  \ELSE
  \STATE  $\boldsymbol{\tau}^{\mathrm{s}*}_{i}=\boldsymbol{\tau}^{\mathrm{s}}_{i}$;
  \ENDIF
  
  \IF{$i=0$ or $\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*}_{i})<\bar{w}(\boldsymbol{\tau}^{\mathrm{s}**})$ }
      \STATE $\boldsymbol{\tau}^{\mathrm{s}**}=\boldsymbol{\tau}^{\mathrm{s}*}_{i}$; $r=r_0$; 
      \STATE $m=1$;
      \STATE Apply Algorithm~\ref{algo:Local} to $\boldsymbol{\tau}^{\mathrm{s}*}_{i}$ and \eqref{eq:aux_opt} to obtain $\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_{i}$;
      \STATE $i^{\text{filled}} \leftarrow i^{\text{filled}}+1$
      \IF{$m=1$}
      \STATE $i\leftarrow i+1$;
      \STATE $\boldsymbol{\tau}^{\mathrm{s}}_{i}=\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_{i-1}$;
      \ELSE
      \STATE $\boldsymbol{\tau}^{\mathrm{s}}_{i}=\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_{i}$;
      \ENDIF
      \STATE Go to line 4;
  \ENDIF
  \IF{$m \leq M$}
      \STATE $\boldsymbol{\tau}^{\mathrm{s}*}_{i}=$ the $m^{\mathrm{th}}$ neighbor of $\boldsymbol{\tau}^{\mathrm{s}*}_{i-1}$;
      \STATE $m\leftarrow m+1$;
      \STATE Go to line 12;
  \ELSE
      \IF{$r<\epsilon$ or $i^{\text{filled}}>i_{\max}^{\text{filled}}$ }
           \STATE $\boldsymbol{\tau}^{\mathrm{s}**}$ is the global minimum solution.
          \ELSE
          \STATE $r \leftarrow \frac{r}{10}$;
          \STATE $i \leftarrow i-1$;
          \STATE Go to line 11;   
      \ENDIF
  \ENDIF
    \end{algorithmic}
    \end{multicols}
    \vspace{-3mm}
\end{algorithm}

In Section~\ref{Section:Num_results}, we will show that the SFF method outperforms the SBO method using S-RIS. 

In the second scenario based on \newwRIS, we need to update~\eqref{eq:opt_prob_std_RIS_feb_27_2023} using $\textbf{T}=\textbf{T}^{\mathrm{i}}$. Here, we use the SFF method by following Algorithms~\ref{algo:Local} and \ref{algo:global} since the filled function-based optimization methods solve a general non-convex integer programming problem as long as selecting a possible configuration from a discrete set is the only constraint~\cite{ng2005discrete}. On the contrary, the SBO method can not be directly applied to \newRIS due to the additional non-convexity that arises from dependence of $\bar{\mathcal{M}}^{[m]}$ on the current solution. This necessitates an additional approximation, which further degrades its performance. As a result, in the next section, we only utilize the SFF method for optimizing the I-RIS elements.




==> Sections/Sect3_Beamforming_design_v2.tex <==
We aim to optimize RIS elements to maximize the sum-rate; thus, we formulate our optimization problem as:
\begin{align}
\label{eq:opt_prob_std_RIS_feb_27_2023}
    &\underset{\mathbf{T}}{\max}\underbrace{\sum_{\gidx=1}^{K} \log(1+\text{SINR}_{\gidx})}_{\overset{\triangle}=~-w(\mathbf{T})}\equiv \underset{\mathbf{T}}{\min}~w(\mathbf{T})\\ \nonumber
    &\text{s.t.} ~~\mathbf{T} \in \{\mathbf{T}^{\mathrm{s}}, \mathbf{T}^{\mathrm{i}}\},~~  s_m,s_{\ell, m}\in\{0,1\},~~1\leq \ell,m\leq M,
\end{align}
which is non-convex due to the binary constraints and the non-convex objective function. To optimize~\eqref{eq:opt_prob_std_RIS_feb_27_2023}, we first focus on S-RIS where $\mathbf{T}=\mathbf{T}^{\mathrm{s}}$ and propose two methods to solve the problem: (1) we use the %\avc{write out the full name again} 
semi-definite binary optimization (SBO) method, which converts~\eqref{eq:opt_prob_std_RIS_feb_27_2023} to a semi-definite relaxation (SDR) problem and then solves the equivalent convex problem; (2) we utilize the sigmoid filled function (SFF), which is a heuristic method based on filled function that directly targets \eqref{eq:opt_prob_std_RIS_feb_27_2023} to obtain an approximation of the global optimum solution. We provide further details below. 

\textbf{SBO method:} In this case, to address the non-convexity of the binary constraints, we use slack variable $\textbf{S}$ and rewrite the binary constraint as follows:
% \begin{align}
% \label{eq:Diag_S_feb_27_2023}
%     \mathrm{Diag}(\textbf{S})=\boldsymbol{\tau}^{\mathrm{s}}, 
% \end{align}
% \begin{align}
% \label{eq:S=ss_feb_27_2023}
%     \textbf{S}=\boldsymbol{\tau}^{\mathrm{s}}{\boldsymbol{\tau}^{\mathrm{s}}}^{\top},
% \end{align}


\begin{minipage}[ht]{0.5\linewidth}
\begin{equation}
\label{eq:Diag_S_feb_27_2023}
    \mathrm{Diag}(\textbf{S})=\boldsymbol{\tau}^{\mathrm{s}}, \quad \quad \quad
\end{equation}
\end{minipage}
 % Adjust the spacing between equations
\begin{minipage}[ht]{0.44\linewidth}
\begin{equation}
\label{eq:S=ss_feb_27_2023}
 \textbf{S}=\boldsymbol{\tau}^{\mathrm{s}}{\boldsymbol{\tau}^{\mathrm{s}}}^{\top},\quad \quad
\end{equation}
\end{minipage}



\begin{align}
\label{eq:01_values_feb_27_2023}
    0 \leq s_m \leq 1,~\text{and}~0 \leq S_{\ell, m} \leq 1,~~ \text{for}~ 1\leq \ell,m \leq M,
\end{align}
where $S_{\ell, m}$ is the element in the $\ell^{\mathrm{th}}$ row and $m^{\mathrm{th}}$ column of $\textbf{S}$. Here, \eqref{eq:S=ss_feb_27_2023} is non-convex; therefore, we substitute it with the following conditions~\cite{guo2018new,hu2021robust}.
\begin{align}
\label{eq:Y_matrix_feb_27_2023}
    \textbf{Y}=\begin{bmatrix}
        \textbf{S}& \boldsymbol{\tau}^{\mathrm{s}}\\
        {\boldsymbol{\tau}^{\mathrm{s}}}^{\top}& 1\\
    \end{bmatrix}\succeq \mathbf{0},~~\text{and} ~~ \text{Rank}(\textbf{Y})=1.
\end{align}

Since $\textbf{Y}$ includes binary elements, the rank of $\textbf{Y}$ is equal to one for any binary feasible solution. Next, we define $\textbf{G}^{\gidx j}\overset{\triangle}=\textbf{g}^{[\gidx]} \mathrm{diag}(\textbf{h}^{j})$ and $\bar{\textbf{G}}^{\gidx j}\overset{\triangle}=\textbf{G}^{\gidx j}{\textbf{G}^{\gidx j}}^{\textrm{H}}$ and use \eqref{eq:Diag_S_feb_27_2023}, \eqref{eq:01_values_feb_27_2023}, and \eqref{eq:Y_matrix_feb_27_2023} to rewrite~\eqref{eq:opt_prob_std_RIS_feb_27_2023} as an SDR problem as follows:
\begin{align}
\label{eq:finalswitch_SNR_feb_27_2023}
    &\underset{\boldsymbol{\tau}^{\mathrm{s}},\textbf{S} }{\min}~-\sum_{\gidx=1}^K\log\left(1+\frac{P_{\gidx}~\mathrm{tr}\left(\textbf{S}\bar{\textbf{G}}^{\gidx \gidx }\right)}{\sigma^2+\sum_{j=1,j\neq \gidx}^K P_j~\mathrm{tr}\left(\textbf{S}\bar{\textbf{G}}^{\gidx j}\right) }\right)\\ \nonumber
    &\text{s.t.} ~~ \mathrm{Diag}(\textbf{S})=\boldsymbol{\tau}^{\mathrm{s}}, \quad \textbf{Y}\succeq \mathbf{0}, \\ \nonumber 
    & ~~~~~~0 \leq s_m \leq 1,~~0 \leq S_{\ell, m} \leq 1,~~ \text{for}~ 1\leq \ell,m \leq M.
\end{align}

Then, we use the feature of a logarithmic function and rewrite~\eqref{eq:finalswitch_SNR_feb_27_2023} as:
\begin{align}
\label{eq:finalswitch_SINR_Dbi_Nbi_feb_27_2023}
    &\underset{\boldsymbol{\tau}^{\mathrm{s}},\textbf{S} }{\min}~N-D\\ \nonumber
    &\text{s.t.} ~~ \mathrm{Diag}(\textbf{S})=\boldsymbol{\tau}^{\mathrm{s}}, \quad \textbf{Y}\succeq \mathbf{0}, \\ \nonumber 
    & ~~~~~~0 \leq s_m \leq 1,~~0 \leq S_{\ell, m} \leq 1,~~ \text{for}~ 1\leq \ell,m \leq M,
\end{align}
where
\begin{align}
    \label{eq:SINR_noise_Nbi_feb_27_2023}
    N=-\sum_{\gidx=1}^K\log\left(\sigma^2+\sum_{j=1}^K P_{j}~\mathrm{tr}\left(\textbf{S}\bar{\textbf{G}}^{\gidx j}\right)\right),
\end{align}
and
\begin{align}
    \label{eq:SINR_noise_Dbi_feb_27_2023}
    D=-\sum_{\gidx=1}^K\log\left(\sigma^2+\sum_{j=1, j\neq \gidx}^K P_j~\mathrm{tr}\left(\textbf{S}\bar{\textbf{G}}^{\gidx j}\right)\right).
\end{align}

Based on \eqref{eq:SINR_noise_Nbi_feb_27_2023} and \eqref{eq:SINR_noise_Dbi_feb_27_2023}, $N$ and $D$ are convex with respect to $\textbf{S}$; thus,~\eqref{eq:finalswitch_SINR_Dbi_Nbi_feb_27_2023} falls under the difference of convex (DC) optimization problem. To solve this problem, we use the SCA method, which is an iterative approach that runs for $I_{\mathrm{tr}}$ times. To do so, we apply the first-order Taylor approximation to $D$ and obtain a lower bound on that as follows:
\begin{align}
\label{eq:lower_bound_Dbi_formula_feb_27_2023}
    D(\textbf{S})\geq D\left(\textbf{S}^t\right)+\nabla^{\top}_{\textbf{S}}\left(D\left(\textbf{S}^t\right)\right)\left(\textbf{S}-\textbf{S}^t\right),
\end{align}
where $\textbf{S}^t$ is the value of $\textbf{S}$ in the $t^{\mathrm{th}}$ iteration and 
\begin{align}
\label{eq:lower_bound_Dbi_feb_27_2023}
    \nabla^{\top}_{\textbf{S}}\left(D\left(\textbf{S}^t\right)\right)=-\frac{1}{\mathrm{ln}~2}\sum_{\gidx=1}^K\frac{\sum_{j=1, j\neq \gidx}^K P_j\bar{\textbf{G}}^{\gidx j}}{\sigma^2+\sum_{j=1, j\neq \gidx}^K P_j~\mathrm{tr}\left(\textbf{S}^t\bar{\textbf{G}}^{\gidx j}\right)}.
\end{align} 

By applying \eqref{eq:lower_bound_Dbi_formula_feb_27_2023} to \eqref{eq:finalswitch_SINR_Dbi_Nbi_feb_27_2023}, we obtain a convex SDR problem and solve it using CVX Toolbox in MATLAB~\cite{grant2011matlab}.

\textbf{SFF method:} Heuristic optimization methods (e.g., genetic algorithm and filled function) are popular for optimizing non-convex problems. Unlike the SBO method, a heuristic method directly tackles the non-convex problem in~\eqref{eq:opt_prob_std_RIS_feb_27_2023} without needing approximations for a convex equivalent. This avoids the performance degradation associated with the approximations used in the SBO method. Hence, we utilize the SFF method based on sigmoid filled function~\cite{nassirpour2022power} as our second optimization method in this paper to solve~\eqref{eq:opt_prob_std_RIS_feb_27_2023}. This method includes two steps: local and global search. Prior to explaining the details, we need to define: (i) $\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})\overset{\triangle}=w(\textbf{T}^{\mathrm{s}})$, and (ii) $\left[\boldsymbol{\tau}^{\mathrm{s}}\right]_n\in \{0,1\}^{M \times 1}$ as the $n^{\mathrm{th}}$ neighbor of $\boldsymbol{\tau}^{\mathrm{s}}$, where $||\left[\boldsymbol{\tau}^{\mathrm{s}}\right]_n-\boldsymbol{\tau}^{\mathrm{s}}||^2=1$ and $1\leq n\leq M$. Here, the SFF method first runs the local search with respect to $\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})$ to obtain the local minimum solution for~\eqref{eq:opt_prob_std_RIS_feb_27_2023}. To do so, we start from initial configuration $\boldsymbol{\tau}^{\mathrm{s}}$ and search among its neighbors to find $\boldsymbol{\tau}^{\mathrm{s}*}$ as a new solution that provides $\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})<\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})$. We note that $\boldsymbol{\tau}^{\mathrm{s}}$ has $M$ neighbors. If $\boldsymbol{\tau}^{\mathrm{s}*}\neq \boldsymbol{\tau}^{\mathrm{s}}$, we set $\boldsymbol{\tau}^{\mathrm{s}}=\boldsymbol{\tau}^{\mathrm{s}*}$, and redo the above process. We define $i^{\text{loc}}$ to indicate the number of iterations that we use the local search process. The search ends if $i^{\text{loc}}$ reaches its maximum value (i.e., $i^{\text{loc}}_{\max}$) or there is no further improvement by running the search (i.e., $\boldsymbol{\tau}^{\mathrm{s}*}=\boldsymbol{\tau}^{\mathrm{s}}$). The details are demonstrated in Algorithm~\ref{algo:Local}. 
\begin{algorithm}
  \caption{Local Search}
  \begin{multicols}{2}
  
  \hspace*{\algorithmicindent} \textbf{Input:} $\boldsymbol{\tau}^{\mathrm{s}}$, $i_{\max}^{\text{loc}}$; \\ 
  \hspace*{\algorithmicindent} \textbf{Output:} $\boldsymbol{\tau}^{\mathrm{s}*}$;
  \begin{algorithmic}[1]
  \label{algo:Local}
  \STATE $i^{\text{loc}}=0$; $\boldsymbol{\tau}^{\mathrm{s}*}=\boldsymbol{\tau}^{\mathrm{s}}$;
  \FOR{ all $ \left[\boldsymbol{\tau}^{\mathrm{s}}\right]_n$ such that $||\left[\boldsymbol{\tau}^{\mathrm{s}}\right]_n-\boldsymbol{\tau}^{\mathrm{s}}||^2=1$}{
  \IF{$\bar{w}(\boldsymbol{\tau}^{\mathrm{s}}_n)< \bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})$}
  \STATE $\boldsymbol{\tau}^{\mathrm{s}*}=\left[\boldsymbol{\tau}^{\mathrm{s}}\right]_n$;
  \ENDIF
  }
  \ENDFOR
  \STATE $i^{\text{loc}} \leftarrow i^{\text{loc}}+1$;
  \IF{$\boldsymbol{\tau}^{\mathrm{s}*}\neq \boldsymbol{\tau}^{\mathrm{s}}$ and $i^{\text{loc}}\leq i_{\max}^{\text{loc}}$}
  \STATE $\boldsymbol{\tau}^{\mathrm{s}}=\boldsymbol{\tau}^{\mathrm{s}*}$;
  \STATE Go to line 2;
  \ELSE
  \STATE $\boldsymbol{\tau}^{\mathrm{s}*}$ is the local minimum solution. 
  \ENDIF
\end{algorithmic}
\end{multicols}
\vspace{-3mm}
\end{algorithm}



The output of local search (i.e., $\boldsymbol{\tau}^{\mathrm{s}*}$) depends on the initial choice of $\boldsymbol{\tau}^{\mathrm{s}}$. Thus, we use global search based on sigmoid filled function to move from $\boldsymbol{\tau}^{\mathrm{s}*}$ to another better solution. Here, we use our filled function, $W_r(\boldsymbol{\tau}^{\mathrm{s}},\boldsymbol{\tau}^{\mathrm{s}*})$, and define an auxiliary optimization problem as below:
\begin{align}
\label{eq:aux_opt}
    &\underset{\boldsymbol{\tau}^{\mathrm{s}}}{\min}~W_r(\boldsymbol{\tau}^{\mathrm{s}},\boldsymbol{\tau}^{\mathrm{s}*}) \nonumber \\
    &\text{s.t.} \quad \boldsymbol{\tau}^{\mathrm{s}},\boldsymbol{\tau}^{\mathrm{s}*}\in \{0,1\}^{M \times 1},
\end{align}
where $r$ denotes the heuristic optimization parameter, $\boldsymbol{\tau}^{\mathrm{s}*}$ is the current local minimum solution,
\begin{align}
\label{eq:filled_func}
    &W_r(\boldsymbol{\tau}^{\mathrm{s}},\boldsymbol{\tau}^{\mathrm{s}*})\nonumber\\
    &~~~~=(1+\frac{1}{1+\eta||\boldsymbol{\tau}^{\mathrm{s}}-\boldsymbol{\tau}^{\mathrm{s}*}||^2})q_r(\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})),
\end{align}
\begin{align}
\label{eq:parameters_filled_func}
&q_r(\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*}))\\ \nonumber
&=
\left\{ \begin{array}{ll}
\vspace{1mm} \bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})+r , & \bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})\leq -r, \\
\frac{1}{1+e^{\frac{-6}{r}(\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})+r/2)}}, & -r<\bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})< 0,\\
1, & \bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})\geq 0,
\end{array} \right.
\end{align}
and
\begin{align}
    & \eta=
\left\{ \begin{array}{ll}
\vspace{1mm} 0, & \bar{w}(\boldsymbol{\tau}^{\mathrm{s}})-\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*})\leq -r, \\
1, & \text{otherwise}.
\end{array} \right.
\end{align}

In this part, we use $i$ and $\boldsymbol{\tau}^{\mathrm{s}}_i$ to denote the $i^{\mathrm{th}}$ iteration of global search and the solution in the $i^{\mathrm{th}}$ iteration, respectively. Here, we start from an initial random solution,  $\boldsymbol{\tau}^{\mathrm{s}}_0$, and then apply Algorithm~\ref{algo:Local} to~\eqref{eq:opt_prob_std_RIS_feb_27_2023} to get $\boldsymbol{\tau}^{\mathrm{s}*}_0$. After finding $\boldsymbol{\tau}^{\mathrm{s}*}_0$, we run local search starting from $\boldsymbol{\tau}^{\mathrm{s}*}_0$ with respect to~\eqref{eq:aux_opt} to attain $\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_0$. Next, we assume $\boldsymbol{\tau}^{\mathrm{s}}_1=\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_0$. If $\bar{w}(\boldsymbol{\tau}^{\mathrm{s}}_1)<\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*}_0)$, we consider $\boldsymbol{\tau}^{\mathrm{s}}_1$ as a new solution and redo the above procedure. Else, we apply other neighbors of $\boldsymbol{\tau}^{\mathrm{s}*}_0$ to~\eqref{eq:aux_opt} to obtain a new $\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_0$ and repeat the above procedure. If neither $\boldsymbol{\tau}^{\mathrm{s}*}_0$ nor its neighbors can lead to a new solution, we reduce $r$ (e.g., $r=r/10$) to find a new filled function, and thus new $\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_0$ and then repeat the above search. Moreover, we use $\gamma \in \mathbb{N}$ to indicate that after $\gamma$ times of finding
the local minimizer of~\eqref{eq:aux_opt}, we
run local search for~\eqref{eq:opt_prob_std_RIS_feb_27_2023}. The search stops if $r< \epsilon, \epsilon\ll 1$ or $i^{\text{filled}}$, the number of times that we use the filled function, reaches its maximum value, $i^{\text{filled}}_{\max}$. In this case, we say that the current solution is an approximation of the global minimum solution.
%%-----------------%%



% It is important to note that the local search uses finite steps to find the local minimizer since there are $N^M$ possible solutions that are finite. 

\begin{algorithm}
  \caption{Global Search}
  \begin{multicols}{2}
  \hspace*{\algorithmicindent} \textbf{Input:} $\boldsymbol{\tau}^{\mathrm{s}}_0, r, \gamma, \epsilon, i_{\max}^{\text{loc}}, i_{\max}^{\text{filled}}$; 
  \hspace*{\algorithmicindent}\hspace{-0.4mm} \textbf{Output:} $\boldsymbol{\tau}^{\mathrm{s}**}$;
  \begin{algorithmic}[1]
  \label{algo:global}
  \STATE $i=0$; $r_0=r$; $\bar{\gamma}=\gamma$;
  \STATE $i^{\text{filled}}=0$;
  \STATE $\boldsymbol{\tau}^{\mathrm{s}**}=\boldsymbol{\tau}^{\mathrm{s}}_0$;
  \IF{$i+1\geq \bar{\gamma}$}
  \STATE $\bar{\gamma}\leftarrow\bar{\gamma}+\gamma$;
  \STATE Apply Algorithm~\ref{algo:Local} to $\boldsymbol{\tau}^{\mathrm{s}}_{i}$ and \eqref{eq:opt_prob_std_RIS_feb_27_2023} to get $\boldsymbol{\tau}^{\mathrm{s}*}_{i}$;
  \ELSE
  \STATE  $\boldsymbol{\tau}^{\mathrm{s}*}_{i}=\boldsymbol{\tau}^{\mathrm{s}}_{i}$;
  \ENDIF
  
  \IF{$i=0$ or $\bar{w}(\boldsymbol{\tau}^{\mathrm{s}*}_{i})<\bar{w}(\boldsymbol{\tau}^{\mathrm{s}**})$ }
      \STATE $\boldsymbol{\tau}^{\mathrm{s}**}=\boldsymbol{\tau}^{\mathrm{s}*}_{i}$; $r=r_0$; 
      \STATE $m=1$;
      \STATE Apply Algorithm~\ref{algo:Local} to $\boldsymbol{\tau}^{\mathrm{s}*}_{i}$ and \eqref{eq:aux_opt} to obtain $\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_{i}$;
      \STATE $i^{\text{filled}} \leftarrow i^{\text{filled}}+1$
      \IF{$m=1$}
      \STATE $i\leftarrow i+1$;
      \STATE $\boldsymbol{\tau}^{\mathrm{s}}_{i}=\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_{i-1}$;
      \ELSE
      \STATE $\boldsymbol{\tau}^{\mathrm{s}}_{i}=\bar{\boldsymbol{\tau}}^{\mathrm{s}*}_{i}$;
      \ENDIF
      \STATE Go to line 4;
  \ENDIF
  \IF{$m \leq M$}
      \STATE $\boldsymbol{\tau}^{\mathrm{s}*}_{i}=$ the $m^{\mathrm{th}}$ neighbor of $\boldsymbol{\tau}^{\mathrm{s}*}_{i-1}$;
      \STATE $m\leftarrow m+1$;
      \STATE Go to line 12;
  \ELSE
      \IF{$r<\epsilon$ or $i^{\text{filled}}>i_{\max}^{\text{filled}}$ }
           \STATE $\boldsymbol{\tau}^{\mathrm{s}**}$ is the global minimum solution.
          \ELSE
          \STATE $r \leftarrow \frac{r}{10}$;
          \STATE $i \leftarrow i-1$;
          \STATE Go to line 11;   
      \ENDIF
  \ENDIF
    \end{algorithmic}
    \end{multicols}
    \vspace{-3mm}
\end{algorithm}

In Section~\ref{Section:Num_results}, we will show that the SFF method outperforms the SBO method using S-RIS. 

In the second scenario based on \newwRIS, we need to update~\eqref{eq:opt_prob_std_RIS_feb_27_2023} using $\textbf{T}=\textbf{T}^{\mathrm{i}}$. Here, we use the SFF method by following Algorithms~\ref{algo:Local} and \ref{algo:global} since the filled function-based optimization methods solve a general non-convex integer programming problem as long as selecting a possible configuration from a discrete set is the only constraint~\cite{ng2005discrete}. On the contrary, the SBO method can not be directly applied to \newRIS due to the additional non-convexity that arises from dependence of $\bar{\mathcal{M}}^{[m]}$ on the current solution. This necessitates an additional approximation, which further degrades its performance. As a result, in the next section, we only utilize the SFF method for optimizing the I-RIS elements.




==> Sections/Sect4_Numerical_analysis.tex <==
In this section, we evaluate the effectiveness of our proposed RIS structures. We assume a multi-user RIS-assisted network with one RIS and $K$ transmitter-receiver pairs, where transmitters and RIS are fixed-location nodes and receivers are located randomly across an area with $100 \mathrm{m}\times 100\mathrm{m}$ dimensions. The simulation parameters are shown in Table~\ref{table:sim_param}.

\begin{table}[h]
\caption{Simulation parameters}
\fontsize{9pt}{12pt}\selectfont
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Parameters} & \textbf{Value} \\ 
\hline 
$\#$ of transmitter-receiver pairs & $K=4$\\ Location of transmitters $(\mathrm{10m})$ & $(5,0),(0,5),(10,5),(5,10)$\\
Location of RIS $(\mathrm{m})$& $(50,50)$\\
Transmit power $(\mathrm{dBm})$ & $P_i=40$\\
Noise power $(\mathrm{dBm})$  & $\sigma^2=-80$\\
Path loss exponent & $\alpha_1=2,\alpha_2=2.1,$\\
Signal loss at $1\mathrm{m}$ $(\mathrm{dB})$ & $C_0=-30$\\
Wavelength $(\mathrm{m})$& $\lambda=0.125$\\
Rician factor & $\kappa=2$\\
SFF parameters & $r=10, \gamma=10, \epsilon=0.01$\\
 & $i_{\max}^{\text{loc}}=M, i_{\max}^{\text{filled}}=8(M+1)$\\
SBO parameter & $I_{\mathrm{tr}}=5$\\
%[1ex]  % [1ex] adds vertical space
\hline
\end{tabular}
\label{table:sim_param}
\end{table}

\begin{figure}[ht]
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=5, width=0.8\linewidth, draft=false]{images/I_RIS_S_RIS_v2.png}
  \vspace{-2mm}
  \caption{Sum-rate against $\log(M)$ using S-RIS, I-RIS $(2,1)$, and I-RIS $(2,2)$.}\label{Fig:S_RIS_vs_I_RIS}
  \vspace{-5mm}
\end{figure}

\textbf{I-RIS vs. S-RIS:} In this part, we present a sum-rate comparison between S-RIS and I-RIS using the SFF method. Fig.~\ref{Fig:S_RIS_vs_I_RIS} shows sum-rate versus $\log(M)$ using S-RIS and two I-RIS cases with cell size $(2,1)$ and $(2,2)$ where $M \in \{4,8,16,32,64\}$. Based on Fig.~\ref{Fig:S_RIS_vs_I_RIS}, I-RIS enables multi-user scaling by offering a higher gain when $M$ is fixed. For instance, with $M=64$, S-RIS provides a sum-rate of $7.30$ bits/sec/Hz, while I-RIS $(2,1)$ and  I-RIS $(2,2)$ offer $9.88$ bits/sec/Hz, and $12.29$ bits/sec/Hz, which represent $35\%$ and $68\%$ improvement compared to S-RIS, respectively. This benefit comes from using more electronic circuits (power splitters and additional RF switches) to share the incident signal powers in I-RIS. We note that it is possible to create different versions of I-RIS by changing the cell size, and as the cell size increases, we get higher gains. 

Moreover, Fig.~\ref{Fig:S_RIS_vs_I_RIS} depicts that I-RIS requires fewer elements than S-RIS to provide the same sum-rate. For example, to achieve a sum-rate of $6$ bits/sec/Hz, we need $64$ elements with S-RIS, whereas we require $32$ and $16$ elements to get the same performance with I-RIS $(2,1)$ and  I-RIS $(2,2)$, respectively. This occurs since I-RIS needs fewer elements than S-RIS to obtain the same DoC. We use $M^{\prime}$ to denote the DoC, where $M^{\prime}=M\times c\times d$ with I-RIS, whereas in an S-RIS, we have $M^{\prime}=M$. Fig.~\ref{Fig:S_RIS_vs_I_RIS} depicts that S-RIS and I-RIS provide almost identical sum-rates if they have the same value of $M^{\prime}$.


\begin{comment}
    
\begin{table}[h]
\caption{Complexity of the SFF method using S-RIS and two cases based on I-RIS.}
\fontsize{9pt}{12pt}\selectfont
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 & $M^{\prime}=16$ & $M^{\prime}=32$&  $M^{\prime}=64$\\ 
\hline 
S-RIS  & $3.16\times 10^3$ & $1.27\times 10^4$  & $6.77 \times 10^4$\\
I-RIS ($2,1$) & $4.92 \times 10^3$ & $2.02\times 10^4$ & $9.10\times 10^4$  \\
I-RIS ($2,2$)  & $8.76\times 10^3$ & $3.17\times 10^4$ & $1.53\times 10^5$ \\
%[1ex]  % [1ex] adds vertical space
\hline
\end{tabular}
\label{table:complexity_SFF_standard_RIS_generalized_RIS}
\end{table}


\textbf{CSI resolution:}  Fig.~\ref{Fig:perfect_imperfect_comparison} compares the performance of I-RIS and S-RIS using the SFF method and under perfect and imperfect channels whose elements are distributed based on Rician-Rayleigh fading. As we expected, imperfect CSI results in gain reduction in both RIS structures since the optimal RIS configurations depend on channel realizations. It also depicts that, with imperfect CSI, I-RIS provides a higher sum-rate compared to S-RIS with the same number of RIS elements, and both RIS structures offer almost the same gains when they use the same DoC. As a result, the performance of the RIS-assisted network using imperfect CSI is not further degraded by I-RIS.
\begin{figure}[ht]
\centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=5, width=0.7\linewidth, draft=false]{images/perfect_imperfect_CSI.png}
  \vspace{-2mm}
  \caption{A sum-rate comparison between S-RIS and I-RIS $(2,1)$ %using the SFF method
  under perfect and imperfect CSI. 
  }\label{Fig:perfect_imperfect_comparison}
  %\vspace{-7mm}
\end{figure}
\end{comment}

\begin{figure}[ht]
\centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=5, width=0.85\linewidth, draft=false]{images/SW_vs_PS_I_RIS.eps}
  \vspace{-2mm}
  \caption{A comparison between a switch-based S-RIS, two cases of switch-based I-RIS, and a PS-based S-RIS using the SFF method. 
  }\label{Fig:sw_vs_PS_I_RIS}
  \vspace{-4mm}
\end{figure}
\textbf{Switch against phase shifter:} In Fig.~\ref{Fig:sw_vs_PS_I_RIS}, we compare the performance of our proposed switch-based RIS structures with an S-RIS using $2$-bit PSs. According to Fig.~\ref{Fig:sw_vs_PS_I_RIS}, our switch-based I-RIS $(2,2)$ has a higher gain due to its higher DoC ($M^{\prime}=M\times b$ with an S-RIS using $b$-bit PSs). Additionally, Fig.~\ref{Fig:sw_vs_PS_I_RIS} shows that if our switch-based I-RIS and the S-RIS with PSs have the same DoC (i.e., I-RIS $(2,1)$ and S-RIS with $2$-bit PSs), the latter provides a higher gain since it changes the phase of the incident signals, while the switch-based RIS can either block or reflect the incident signals.

\textbf{Performance of the optimization methods:} In this part, we evaluate the performance of our proposed optimization methods (the SFF and SBO methods) and the SR method in terms of sum-rate and complexity. Fig.~\ref{Fig:optimization_comparison} depicts sum-rate versus $\log(M)$ using S-RIS. It shows that the SFF method offers a higher sum-rate than the others since the SFF method directly targets the non-convex problem to
optimize the RIS elements, while the SBO method incorporates some approximations in the optimization process and solves an equivalent convex problem. Also, the SR method finds a local optimum solution, whereas the SFF method uses a filled function to move from one local optimum solution to another better one. Furthermore, the complexity of the SFF method is equal to $\mathcal{O}(2\log_{10}(r/\epsilon)M^5)$~\cite{nassirpour2022control}, which is lower than the complexity of  
the SBO method,
$\mathcal{O}(I_{\mathrm{tr}}(M+1)^3M^3)$~\cite{bomze2010interior}, and higher than the complexity of the SR method, which is $\mathcal{O}(M^4)$~\cite{wu2019beamforming}.
\begin{figure}[ht]
\vspace{-3mm}
\centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=5, width=0.85\linewidth, draft=false]{images/Fig_SFF_SB_SR_S_RIS_July_07_2023.eps}
  \vspace{-2mm}
  \caption{A Sum-rate comparison between the SFF, SBO, and SR methods. 
  }\label{Fig:optimization_comparison}
  %\vspace{-7mm}
\end{figure}





==> Sections/Sect4_Numerical_analysis_USV.tex <==
In this section, we assess the performance of our proposed RIS structures. The simulation parameters are shown in Table~\ref{table:sim_param}. We assume a maritime network where transmitters and RIS are fixed-location nodes and receivers are located randomly across an area with $100 \mathrm{m}\times 100\mathrm{m}$ dimensions.
\begin{table}[ht]
\caption{Simulation parameters}
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Parameters} & \textbf{Value} \\ 
\hline 
Number of transmitter-receiver pairs & $K=4$\\ Location of transmitters $(\mathrm{m})$ & $(50,0),(0,50),(100,50),(50,100)$\\
Location of RIS $(\mathrm{m})$& $(50,50)$\\
Transmit power from ${\sf Tx}_i$ $(\mathrm{dBm})$ & $P_i=40$\\
Noise power$(\mathrm{dBm})$  & $\sigma^2=-80$\\
Path loss exponent & $\alpha_1=2,\alpha_2=2.1,$\\
Signal loss at reference distance $(\mathrm{dB})$ & $C_0=-30$\\
Wavelength $(\mathrm{m})$& $\lambda=0.125$\\
Rician factor & $\kappa=2$\\
Perfect CSI parameter& $p=0$\\
Imperfect CSI parameter& $p=20\mathrm{dB}$\\
SFF parameters & $r=10, \gamma=10, \epsilon=0.01$\\
SBO parameter & $I_{tr}=10$\\
%[1ex]  % [1ex] adds vertical space
\hline
\end{tabular}
\label{table:sim_param}
\end{table}

\textbf{\newRIS vs. S-RIS:} In Fig.~\ref{Fig:std_vs_general}, we compare the sum-rate of the S-RIS to two \newRIS cases with cell size $(2,1)$ and $(2,2)$ under both perfect and imperfect CSI. Based on Fig.~\ref{Fig:std_vs_general}, the \newRIS enables multi-user scaling by offering a higher gain when $M$ is fixed. It also requires fewer RIS elements (i.e., compact RIS) than the S-RIS to provide the same sum-rate. These benefits come from using more electronic circuits (power splitters and additional RF switches) to share the incident signal powers. We note that it is possible to create different versions of the \newRIS by changing the cell size, and as the cell size increases (i.e., the number of cells decreases), we get higher gains. 

We use $M'$ to denote the number of control elements that require optimization in the scenarios using the \newRIS and S-RIS. In the \newwRIS, $M'$ is equal to $Mcd$, whereas in the S-RIS, it is equal to $M$. In this work, we define the number of evaluations needed to find
the solution as complexity. Table~\ref{table:complexity_SFF_standard_RIS_generalized_RIS} demonstrates that the complexity of the SFF method with the \newRIS and S-RIS under perfect CSI is in the same order if we optimize the same $M'$ control elements.
 
\begin{figure}[ht]
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=6, width=0.9\linewidth, draft=false]{images/std_vs_general.eps}
\vspace{-2mm}
\caption{\it Sum-rate versus $\log(M)$ relying on the SFF method using the S-RIS and the \newwRIS s with different cell sizes.}\label{Fig:std_vs_general}
\end{figure}


\begin{table}[h]
\caption{Complexity of the SFF method in a maritime network assisted by the S-RIS and two cases based on the \newwRIS.}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 & $M=4$ & $M=8$ & $M=16$ & $M=32$\\ 
\hline 
S-RIS & $198$ & $774$ & $3.16\times 10^3$ & $1.27\times 10^4$  \\
\newRIS ($2,1$) & $1.32\times 10^3$ & $4.92\times 10^3$ & $2.02\times 10^4$ & $9.10\times 10^4$ \\
\newRIS ($2,2$)  & $8.76\times 10^3$ & $3.17\times 10^4$ & $1.53\times 10^5$ & $7.27\times 10^5$ \\
%[1ex]  % [1ex] adds vertical space
\hline
\end{tabular}
\label{table:complexity_SFF_standard_RIS_generalized_RIS}
\end{table}

\textbf{Performance of the optimization methods:} In this part, we compare the performance of the SFF method with the SBO method in terms of sum-rate and complexity when we use the S-RIS. Further, we consider the brute-force (BF) search as a benchmark, which guarantees finding the global optimum solution. Fig.~\ref{Fig:SBO_SFF_BF_cmparison} depicts the sum-rate versus $\log(M)$ when $M \in \{4,8,16\}$ and perfect CSI is available. It shows that the SFF method provides sum-rates close to the BF search and outperforms the SBO method. It occurs since the SBO method incorporates some approximations in the optimization process and solves an equivalent convex problem, but the SFF method directly targets the non-convex problem to
optimize the RIS elements. Moreover, the complexity of the SFF method is equal to $\mathcal{O}(2\log_{10}(r/\epsilon)M^3)$~\cite{nassirpour2022control}, whereas the complexity of the BF search and the SBO method equal to $2^M-1$ and $\mathcal{O}(I_{tr}(M+1)^3)$~\cite{bomze2010interior}, respectively. As a result, the SFF method offers a lower complexity than the other two benchmarks. 
\begin{figure}[ht]
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=6, width=0.9\linewidth, draft=false]{images/std_SFF_vs_SBO.eps}
\vspace{-2mm}
\caption{\it A sum-rate comparison between the BF search, the SFF method, and the SBO method in a maritime network using the S-RIS and prefect CSI. }\label{Fig:SBO_SFF_BF_cmparison}
\end{figure}






==> Sections/Sect4_Numerical_analysis_v1.tex <==
In this section, we evaluate the effectiveness of our proposed RIS structures. We assume a multi-user RIS-assisted network with one RIS and $K$ transmitter-receiver pairs, where transmitters and RIS are fixed-location nodes and receivers are located randomly across an area with $100 \mathrm{m}\times 100\mathrm{m}$ dimensions. The simulation parameters are shown in Table~\ref{table:sim_param}.

\begin{table}[h]
\caption{Simulation parameters}
\fontsize{9pt}{12pt}\selectfont
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Parameters} & \textbf{Value} \\ 
\hline 
$\#$ of transmitter-receiver pairs & $K=4$\\ Location of transmitters $(\mathrm{10m})$ & $(5,0),(0,5),(10,5),(5,10)$\\
Location of RIS $(\mathrm{m})$& $(50,50)$\\
Transmit power $(\mathrm{dBm})$ & $P_j=40, 1 \leq j \leq K$\\
Noise power $(\mathrm{dBm})$  & $\sigma^2=-80$\\
Path loss exponent & $\alpha_1=2,\alpha_2=2.1,$\\
Signal loss at $1\mathrm{m}$ $(\mathrm{dB})$ & $C_0=-30$\\
Wavelength $(\mathrm{m})$& $\lambda=0.125$\\
Rician factor & $\kappa=2$\\
SFF parameters & $r=10, \gamma=10, \epsilon=0.01$\\
 & $i_{\max}^{\text{loc}}=M, i_{\max}^{\text{filled}}=8(M+1)$\\
SBO parameter & $I_{\mathrm{tr}}=5$\\
%[1ex]  % [1ex] adds vertical space
\hline
\end{tabular}
\label{table:sim_param}
\vspace{-6mm}
\end{table}

\begin{figure}[ht]
%\vspace{-5mm}
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=5, width=0.68\linewidth, draft=false]{images/SRIS_IRIS_updated_gh.png}
  \vspace{-4mm}
  \caption{Sum-rate against $\log(M)$ using S-RIS, I-RIS $(2,1)$, and I-RIS $(2,2)$.}\label{Fig:S_RIS_vs_I_RIS}
  \vspace{-2mm}
\end{figure}

\textbf{I-RIS vs. S-RIS:} In this part, we present a sum-rate comparison between S-RIS and I-RIS using the SFF method. Fig.~\ref{Fig:S_RIS_vs_I_RIS} shows sum-rate versus $\log(M)$ using S-RIS and two I-RIS cases with cell size $(2,1)$ and $(2,2)$ where $M \in \{4,8,16,32,64\}$. Based on Fig.~\ref{Fig:S_RIS_vs_I_RIS}, I-RIS enables multi-user scaling by offering a higher gain when $M$ is fixed. For instance, with $M=64$, I-RIS $(2,1)$ and  I-RIS $(2,2)$ offer $44\%$ and $81\%$ improvement compared to S-RIS, respectively. This benefit comes from using more electronic circuits (power splitters and additional RF switches) to share the incident signal powers in I-RIS. We note that it is possible to create different versions of I-RIS by changing the cell size, and as the cell size increases, we get a higher gain. 

Moreover, Fig.~\ref{Fig:S_RIS_vs_I_RIS} depicts that I-RIS requires fewer elements than S-RIS to provide the same sum-rate. For example, to achieve a sum-rate of $6$ bits/sec/Hz, we need $64$ elements with S-RIS, whereas we require $32$ and $16$ elements to get the same performance with I-RIS $(2,1)$ and  I-RIS $(2,2)$, respectively. This occurs since I-RIS needs fewer elements than S-RIS to obtain the same DoC. We use $M^{\prime}$ to denote the DoC, where $M^{\prime}=M\times c\times d$ with I-RIS, whereas in an S-RIS, we have $M^{\prime}=M$. Fig.~\ref{Fig:S_RIS_vs_I_RIS} shows that S-RIS and I-RIS provide almost identical sum-rates if they have the same value of $M^{\prime}$.


\begin{comment}
    
\begin{table}[h]
\caption{Complexity of the SFF method using S-RIS and two cases based on I-RIS.}
\fontsize{9pt}{12pt}\selectfont
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 & $M^{\prime}=16$ & $M^{\prime}=32$&  $M^{\prime}=64$\\ 
\hline 
S-RIS  & $3.16\times 10^3$ & $1.27\times 10^4$  & $6.77 \times 10^4$\\
I-RIS ($2,1$) & $4.92 \times 10^3$ & $2.02\times 10^4$ & $9.10\times 10^4$  \\
I-RIS ($2,2$)  & $8.76\times 10^3$ & $3.17\times 10^4$ & $1.53\times 10^5$ \\
%[1ex]  % [1ex] adds vertical space
\hline
\end{tabular}
\label{table:complexity_SFF_standard_RIS_generalized_RIS}
\end{table}


\textbf{CSI resolution:}  Fig.~\ref{Fig:perfect_imperfect_comparison} compares the performance of I-RIS and S-RIS using the SFF method and under perfect and imperfect channels whose elements are distributed based on Rician-Rayleigh fading. As we expected, imperfect CSI results in gain reduction in both RIS structures since the optimal RIS configurations depend on channel realizations. It also depicts that, with imperfect CSI, I-RIS provides a higher sum-rate compared to S-RIS with the same number of RIS elements, and both RIS structures offer almost the same gains when they use the same DoC. As a result, the performance of the RIS-assisted network using imperfect CSI is not further degraded by I-RIS.
\begin{figure}[ht]
\centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=5, width=0.7\linewidth, draft=false]{images/perfect_imperfect_CSI.png}
  \vspace{-2mm}
  \caption{A sum-rate comparison between S-RIS and I-RIS $(2,1)$ %using the SFF method
  under perfect and imperfect CSI. 
  }\label{Fig:perfect_imperfect_comparison}
  %\vspace{-7mm}
\end{figure}
\end{comment}

\begin{figure}[ht]
%\vspace{-4mm}
\centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=5, width=0.7\linewidth, draft=false]{images/Fig_SW_PS_updated_gh.eps}
  \vspace{-4mm}
  \caption{A comparison between a switch-based S-RIS, two cases of switch-based I-RIS, and a PS-based S-RIS using the SFF method. 
  }\label{Fig:sw_vs_PS_I_RIS}
  \vspace{-6mm}
\end{figure}
\textbf{Switch against phase shifter:} In Fig.~\ref{Fig:sw_vs_PS_I_RIS}, we compare the performance of our proposed switch-based RIS structures with an S-RIS using $2$-bit PSs. According to Fig.~\ref{Fig:sw_vs_PS_I_RIS}, our switch-based I-RIS $(2,2)$ has a higher gain due to its higher DoC ($M^{\prime}=M\times b$ with an S-RIS using $b$-bit PSs). Additionally, Fig.~\ref{Fig:sw_vs_PS_I_RIS} shows that if our switch-based I-RIS and the S-RIS with PSs have the same DoC (i.e., I-RIS $(2,1)$ and S-RIS with $2$-bit PSs), the latter provides a higher gain since it changes the phase of the incident signals, while the switch-based RIS can either block or reflect the incident signals.

\textbf{Performance of the optimization methods:} In this part, we evaluate the performance of our proposed optimization methods (the SFF and SBO methods) and the SR method in terms of sum-rate and complexity. Fig.~\ref{Fig:optimization_comparison} depicts sum-rate versus $\log(M)$ using S-RIS. It shows that the SFF method offers a higher sum-rate than the others since the SFF method directly targets the non-convex problem to
optimize the RIS elements, while the SBO method incorporates some approximations in the optimization process and solves an equivalent convex problem. Also, the SR method finds a local optimum solution, whereas the SFF method uses a filled function to move from one local optimum solution to another better one. Furthermore, the complexity of the SFF method is equal to $\mathcal{O}(2\log_{10}(r/\epsilon)M^5)$~\cite{nassirpour2022control}, which is lower than the complexity of  
the SBO method,
$\mathcal{O}(I_{\mathrm{tr}}(M+1)^3M^3)$~\cite{bomze2010interior}, and higher than the complexity of the SR method, which is $\mathcal{O}(M^4)$~\cite{wu2019beamforming}.
\begin{figure}[ht]
\vspace{-3mm}
\centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=5, width=0.7\linewidth, draft=false]{images/Fig_SFF_SBO_SR_updated_gh.eps}
  \vspace{-4mm}
  \caption{A Sum-rate comparison between the SFF, SBO, and SR methods. 
  }\label{Fig:optimization_comparison}
  \vspace{-4mm}
\end{figure}





==> Sections/Sect4_Numerical_analysis_v2.tex <==
In this section, we evaluate the effectiveness of our proposed RIS structures. We assume a multi-user RIS-assisted network with one RIS and $K$ transmitter-receiver pairs, where transmitters and RIS are fixed-location nodes and receivers are located randomly across an area with $100 \mathrm{m}\times 100\mathrm{m}$ dimensions. The simulation parameters are shown in Table~\ref{table:sim_param}.

\begin{table}[h]
\caption{Simulation parameters}
\fontsize{9pt}{12pt}\selectfont
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Parameters} & \textbf{Value} \\ 
\hline 
$\#$ of transmitter-receiver pairs & $K=4$\\ Location of transmitters $(\mathrm{10m})$ & $(5,0),(0,5),(10,5),(5,10)$\\
Location of RIS $(\mathrm{m})$& $(50,50)$\\
Transmit power $(\mathrm{dBm})$ & $P_j=40, 1 \leq j \leq K$\\
Noise power $(\mathrm{dBm})$  & $\sigma^2=-80$\\
Path loss exponent & $\alpha_1=2,\alpha_2=2.1,$\\
Signal loss at $1\mathrm{m}$ $(\mathrm{dB})$ & $C_0=-30$\\
Wavelength $(\mathrm{m})$& $\lambda=0.125$\\
Rician factor & $\kappa=2$\\
SFF parameters & $r=10, \gamma=10, \epsilon=0.01$\\
 & $i_{\max}^{\text{loc}}=M, i_{\max}^{\text{filled}}=8(M+1)$\\
SBO parameter & $I_{\mathrm{tr}}=5$\\
%[1ex]  % [1ex] adds vertical space
\hline
\end{tabular}
\label{table:sim_param}
\vspace{-6mm}
\end{table}

\begin{figure}[ht]
%\vspace{-5mm}
  \centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=5, width=0.68\linewidth, draft=false]{images/SRIS_IRIS_updated_gh.png}
  \vspace{-4mm}
  \caption{Sum-rate against $\log(M)$ using S-RIS, I-RIS $(2,1)$, and I-RIS $(2,2)$.}\label{Fig:S_RIS_vs_I_RIS}
  \vspace{-2mm}
\end{figure}

\textbf{I-RIS vs. S-RIS:} In this part, we present a sum-rate comparison between S-RIS and I-RIS using the SFF method. Fig.~\ref{Fig:S_RIS_vs_I_RIS} shows sum-rate versus $\log(M)$ using S-RIS and two I-RIS cases with cell size $(2,1)$ and $(2,2)$ where $M \in \{4,8,16,32,64\}$. Based on Fig.~\ref{Fig:S_RIS_vs_I_RIS}, I-RIS enables multi-user scaling by offering a higher gain when $M$ is fixed. For instance, with $M=64$, I-RIS $(2,1)$ and  I-RIS $(2,2)$ offer $44\%$ and $81\%$ improvement compared to S-RIS, respectively. This benefit comes from using more electronic circuits (power splitters and additional RF switches) to share the incident signal powers in I-RIS. We note that it is possible to create different versions of I-RIS by changing the cell size, and as the cell size increases, we get a higher gain. 

Moreover, Fig.~\ref{Fig:S_RIS_vs_I_RIS} depicts that I-RIS requires fewer elements than S-RIS to provide the same sum-rate. For example, to achieve a sum-rate of $6$ bits/sec/Hz, we need $64$ elements with S-RIS, whereas we require $32$ and $16$ elements to get the same performance with I-RIS $(2,1)$ and  I-RIS $(2,2)$, respectively. This occurs since I-RIS needs fewer elements than S-RIS to obtain the same DoC. We use $M^{\prime}$ to denote the DoC, where $M^{\prime}=M\times c\times d$ with I-RIS, whereas in an S-RIS, we have $M^{\prime}=M$. Fig.~\ref{Fig:S_RIS_vs_I_RIS} shows that S-RIS and I-RIS provide almost identical sum-rates if they have the same value of $M^{\prime}$.


\begin{comment}
    
\begin{table}[h]
\caption{Complexity of the SFF method using S-RIS and two cases based on I-RIS.}
\fontsize{9pt}{12pt}\selectfont
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 & $M^{\prime}=16$ & $M^{\prime}=32$&  $M^{\prime}=64$\\ 
\hline 
S-RIS  & $3.16\times 10^3$ & $1.27\times 10^4$  & $6.77 \times 10^4$\\
I-RIS ($2,1$) & $4.92 \times 10^3$ & $2.02\times 10^4$ & $9.10\times 10^4$  \\
I-RIS ($2,2$)  & $8.76\times 10^3$ & $3.17\times 10^4$ & $1.53\times 10^5$ \\
%[1ex]  % [1ex] adds vertical space
\hline
\end{tabular}
\label{table:complexity_SFF_standard_RIS_generalized_RIS}
\end{table}


\textbf{CSI resolution:}  Fig.~\ref{Fig:perfect_imperfect_comparison} compares the performance of I-RIS and S-RIS using the SFF method and under perfect and imperfect channels whose elements are distributed based on Rician-Rayleigh fading. As we expected, imperfect CSI results in gain reduction in both RIS structures since the optimal RIS configurations depend on channel realizations. It also depicts that, with imperfect CSI, I-RIS provides a higher sum-rate compared to S-RIS with the same number of RIS elements, and both RIS structures offer almost the same gains when they use the same DoC. As a result, the performance of the RIS-assisted network using imperfect CSI is not further degraded by I-RIS.
\begin{figure}[ht]
\centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=5, width=0.7\linewidth, draft=false]{images/perfect_imperfect_CSI.png}
  \vspace{-2mm}
  \caption{A sum-rate comparison between S-RIS and I-RIS $(2,1)$ %using the SFF method
  under perfect and imperfect CSI. 
  }\label{Fig:perfect_imperfect_comparison}
  %\vspace{-7mm}
\end{figure}
\end{comment}

\begin{figure}[ht]
%\vspace{-4mm}
\centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=5, width=0.7\linewidth, draft=false]{images/Fig_SW_PS_updated_gh.eps}
  \vspace{-4mm}
  \caption{A comparison between a switch-based S-RIS, two cases of switch-based I-RIS, and a PS-based S-RIS using the SFF method. 
  }\label{Fig:sw_vs_PS_I_RIS}
  \vspace{-6mm}
\end{figure}
\textbf{Switch against phase shifter:} In Fig.~\ref{Fig:sw_vs_PS_I_RIS}, we compare the performance of our proposed switch-based RIS structures with an S-RIS using $2$-bit PSs. According to Fig.~\ref{Fig:sw_vs_PS_I_RIS}, our switch-based I-RIS $(2,2)$ has a higher gain due to its higher DoC ($M^{\prime}=M\times b$ with an S-RIS using $b$-bit PSs). Additionally, Fig.~\ref{Fig:sw_vs_PS_I_RIS} shows that if our switch-based I-RIS and the S-RIS with PSs have the same DoC (i.e., I-RIS $(2,1)$ and S-RIS with $2$-bit PSs), the latter provides a higher gain since it changes the phase of the incident signals, while the switch-based RIS can either block or reflect the incident signals.

\textbf{Performance of the optimization methods:} In this part, we evaluate the performance of our proposed optimization methods (the SFF and SBO methods) and the SR method in terms of sum-rate and complexity. Fig.~\ref{Fig:optimization_comparison} depicts sum-rate versus $\log(M)$ using S-RIS. It shows that the SFF method offers a higher sum-rate than the others since the SFF method directly targets the non-convex problem to
optimize the RIS elements, while the SBO method incorporates some approximations in the optimization process and solves an equivalent convex problem. Also, the SR method finds a local optimum solution, whereas the SFF method uses a filled function to move from one local optimum solution to another better one. Furthermore, the complexity of the SFF method is equal to $\mathcal{O}(2\log_{10}(r/\epsilon)M^5)$~\cite{nassirpour2022control}, which is lower than the complexity of  
the SBO method,
$\mathcal{O}(I_{\mathrm{tr}}(M+1)^3M^3)$~\cite{bomze2010interior}, and higher than the complexity of the SR method, which is $\mathcal{O}(M^4)$~\cite{wu2019beamforming}.
\begin{figure}[ht]
\vspace{-3mm}
\centering
  \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=5, width=0.7\linewidth, draft=false]{images/Fig_SFF_SBO_SR_updated_gh.eps}
  \vspace{-4mm}
  \caption{A Sum-rate comparison between the SFF, SBO, and SR methods. 
  }\label{Fig:optimization_comparison}
  \vspace{-4mm}
\end{figure}





==> Sections/Sect5_Conclusion.tex <==
In this paper, we introduced a new compact RIS structure with interconnected elements, I-RIS, suited for space-limited nodes to assist multi-user networks. We used I-RIS to enable multi-user scaling and do so with fewer elements compared with proper designs. We considered binary RF switches as RIS elements to mitigate the practical issues related to phase shifters and showed that I-RIS outperforms an S-RIS using phase shifters. We proposed the SFF and SBO methods to obtain the optimal RIS configuration. Our findings showed that the SFF method provides a higher sum-rate than the SBO and SR methods, and its complexity is higher than the SR method and lower than the SBO method. In future works, we would like to use multiple I-RISs to improve the performance of multi-user networks under realistic channel models.

==> Sections/Sect5_Conclusion_v1.tex <==
In this paper, we introduced a new compact RIS structure with interconnected elements, I-RIS, suited for space-limited nodes to assist multi-user networks. We used I-RIS to enable multi-user scaling and do so with fewer elements compared with proper designs. We considered binary RF switches as RIS elements to mitigate the practical issues related to phase shifters and showed that I-RIS outperforms an S-RIS using phase shifters. We proposed the SFF and SBO methods to obtain the optimal RIS configuration. Our findings showed that the SFF method provides a higher sum-rate than the SBO and SR methods, and its complexity is higher than the SR method and lower than the SBO method. In future works, we would like to use multiple I-RISs to improve the performance of multi-user networks under realistic channel models.

==> Sections/Sect5_Conclusion_v2.tex <==
In this paper, we introduced a new compact RIS structure with interconnected elements, I-RIS, suited for space-limited nodes to assist multi-user networks. We used I-RIS to enable multi-user scaling and do so with fewer elements compared with proper designs. We considered binary RF switches as RIS elements to mitigate the practical issues related to phase shifters and showed that I-RIS outperforms an S-RIS using phase shifters. We proposed the SFF and SBO methods to obtain the optimal RIS configuration. Our findings showed that the SFF method provides a higher sum-rate than the SBO and SR methods, and its complexity is higher than the SR method and lower than the SBO method. In future works, we would like to use multiple I-RISs to improve the performance of multi-user networks under realistic channel models.
